GNNBENCH: Fair and Productive Benchmarking for Single-GPU GNN System

We hypothesize that the absence of a standardized benchmark has allowed several fundamental pitfalls in GNN System design and evaluation that the community has overlooked. In this work, we propose GNNBench, a plug-and-play benchmarking platform focused on system innovation. GNNBench presents a new protocol to exchange their captive tensor data, supports custom classes in System APIs, and allows automatic integration of the same system module to many deep learning frameworks, such as PyTorch and TensorFlow. To demonstrate the importance of such a benchmark framework, we integrated several GNN systems. Our results show that integration with GNNBench helped us identify several measurement issues that deserve attention from the community.

==> tex/SM.tex <==

\subsection{{\myname-SM}: Graph Preparation and Exchange} \label{sec.engg}

% Moreover, Numpy array has become the standard way to exchange the data between different Python module using zero-copy mechanism.  Therefore, {\graphpy-SM} is implemented on C++ but exports the prepared graph to users using Numpy arrays. Fig.~\ref{fig-engg} presents an overview, and Table~\ref{table-api} presents the APIs for graph creation, and data access using CSR and COO format.  

% \begin{figure}[h]
%   \includegraphics[scale= 0.48]{result/APIs-crop.pdf}
%   \caption{{\graphpy} Data Engineering Framework.}
%   \label{fig-engg}
% \end{figure}


% \td not sure what the next sentence means
% Many data science use-cases are as simple as performing graph topology analysis, such as BFS in the graph, as evident by the huge adoption of NetworkX. Even the DL requires some of those tasks. E.g. when preparing the dataset for DL, many works, such as GraphSage~\cite{graphsage17} do sampling or community analysis to downsize the graph. Further, it also performs connected component analysis and does union of a few components to get the representative dataset to avoid bias etc.
% Therefore, providing data-engineering support by {\graphpy} is not just limited to faster graph preparation from raw data, but requires good support of traditional as well as ad hoc graph analysis. 

%Graph creation step is very different than the kernels involved in DL training,  as the former involves many mundane tasks, such as file handling to parse graph data, and parallel processing to convert them to a desired format such as CSR/CSC. Further, 
%As we mentioned in the \cref{sec.science}, Plugin architecture of DL frameworks limits the way we can exchange data between Python and C++, which made passing the graph data from Workflow to Kernel a custom step for each prior work. 

The independent nature of {\myname-System} allows it to offer native Python binding capabilities. Hence, by modeling a graph as a class object, any custom graph storage can now be passed to its APIs using the same object, hence achieving a stable API. It is much better than using tensors to model graphs that needed workarounds and unstable APIs. 

Apart from customizing the graph storage format, one more variation in graph storage can be observed based on the edge properties.
%\noindent \textbf{Challenges.}
%\noindent \textbf{Gap between C/C++ and Python.}
To illustrate, edges are unweighted and undirected in GCN and GIN  but contain edge ID and are directed in the case of GAT.
%as each edge stores a trainable weight whose access is required through edge ID indirection.
%GAT requires introducing the edge ID abstraction for each edge where the edge ID points the offset in an attention score array to read (forward computation) and modify (backward computation that uses reverse graph) the attention score. 
Furthermore, graph edge requires an edge type being stored as well apart from the edge ID for the knowledge graph auto-completion GNNs~\cite{rgcn2018}. 
%Similarly, sparse tensors require the support of bipartite graphs and edge ID.
Not to mention, the ad hoc data science use-case may require the support of arbitrary multi-field properties, e.g., In LANL network dataset~\cite{turcotte17}, each edge has 9 fields and requires 32 bytes. 
%Similarly, a vertex can have properties, including its string-based identifier, type in the heterogeneous graph, timestamp, etc.

The research question here is whether we can pass graph storage with diverse edge properties to {\myname-System} for various use cases using stable APIs.
Moreover, the next opportunity to develop a productive GNN framework is to allow passing prepared graph to {\myname-System} directly and not forcing it to do the mundane tasks of file handling, data parsing, and parallel processing. 
Hence, another independent module handling graph creation is desired, and it can also be used for other graph data science use cases. 


%challenge here lies in abstracting the graph storage and passing it to {\graphpy-GNN} (or to any third party library) in a way that does not require new implementation of {\graphpy-SM} whenever graph property changes. At the same time, offer expert system researchers sufficient space to innovate in format design and kernel computation. 
% Hence, we again focus on interface design to exchange the data, apart from how to design {\graphpy-SM}.
%\noindent \textbf{Diverse Graph Storage Need.}


%Similarly, many prior graph systems, such as Galois~\cite{nguyen2013lightweight}, Ligra~\cite{shun2013ligra}, etc. cannot support graphs with arbitrary properties, even if we decide to write their Python binding.
%Hence, we can claim that \textit{graph system + Python binding is not equivalent to {\graphpy-SM}}, as the former  forces compilation for each edge property. 

%


%\subsection{Challenges and Prior Works} \label{sec.multi}


% \noindent \textbf{Opportunities.}
% We clearly see a \textit{gap} in the current graph data-science eco-system, which can allow passing graph objects stored in optimized data layout (e.g. CSR/CSC) to any third party C/C++ back-end as well as accessible in Python. Rather, graph object in prior works are captive in nature, i.e., does not allow it to be shared with third-party modules, and supports limited properties, as we explain next. The captive nature also makes the Kernel module a heavy-weight as it will have large code-base for file handling and graph preparation, or one has to rely on an ad hoc  way as in GNNAdvisor.

% It is hard to come up with a static property structure that can satisfy all the use-case of data science.




% Even if one writes python binding for such systems, we will be limited to either a single field property, or force the user to develop a plugin.
% any time we encounter a new set of properties followed by compilation Further, it now requires new python binding for each different set of properties and then compiling and deploying it. Such exercise is fine for system researchers, but we cannot expect the same from data scientists.
% or allow the final representation to be written to disk that can be used by GNNs later by loading them. 
% We focus on the former, as it allows the data scientist to further develop ad hoc techniques such as sampling or community identification to downsize the graph~\cite{graphsage17}.
% this additional python binding task introduces an important challenge to support graphs with arbitrary properties in the Python. This is due to the 



% \td not quite sure whether it relies on NetworkX or not, because DGL can build it own dgl graph, DGL can also build the graph from existing Networkx graph Alternately, it relies on NetworkX~\cite{networkx08}. 
%As we mentioned, this limits the scalability and size that we can operate on. 


%So, there is a need to develop a high-performance graph data engineering framework that can take care of all such tasks.

%the input to be available at once as edge list format of vertex IDs.
%and do not include the ML operations, which is popular in recent years. 
%Although NeuGraph, DGL and AliGraph does provide the python APIs but it assumes that the users already had the graph representation structure. 


%NetworkX \cite{hagberg2008exploring} is a python graph data science package that can create the graph representation and performs graph topology analytic tasks. NetworkX builds the graph representation data structure based on the edge list which contains information about the source node, destination node, and the optional edge weight. After building the graph representation data structure, many future graph analytics scientific computations can be performed, such as calculating the degree of the nodes, the number of nodes in the graph, or even perform a BFS algorithm on the graph data structure.
 
%However, NetworkX can only create the graph data structure from the python edge list, which makes that the network is not flexible to other raw data formats, such as CSV, text, Jason, and binary data. This format requirement restricts the usage of NetworkX and the data scientist needs to perform some graph data engineering to convert the raw data to the format which is satisfied with NextworkX if they want to use the network. Another disadvantage of NetworkX is that it was proposed in 2008, a time that the machine learning algorithms are not popular and widely used. This situation makes that NetworkX only includes traditional topology graph analytics features but not contain any machine learning related features or computations. 
 
 

%To implement the data engineering aspect of {\graphpy}, an important challenge needed to be handled. Many new-generation of graph DL algorithms need to use the dynamic graph edge information, which is not supported by previous works. \td Examples.



\subsubsection{Edge Property Specification: Numpy Dtype}
%\noindent \textbf

{\myname} relies on \textit{Numpy dtype} for edge property specification in the interfaces. 
%and each additional edge property can easily be modeled by defining the dtype. 
Hence, like a NumPy array object, a graph object can also allow the passing of diverse edge properties as shown in Listing~\ref{list-dtype}.
The Numpy dtype is a data type object which looks like a C-structure in Python but keeps many other details like the size of the array elements. Each element can be a native type, such as \textit{float} for a Numpy array of single floating points, or it can be a multi-field (e.g. edge weight, edge ID, edge type, etc.), each with a fixed size data type. 
%allow data scientists to define any arbitrary edge properties in Python, while {\graphpy-SM} dynamically supports those properties without any changes or compilation.
It should be noted that the dtype mechanism has become a de-facto standard for tensor specification in Python, though DL frameworks only allow a few dtype. \textit{{\myname} offers the exchange of graph objects among different modules by using the same de-facto standard of dtype resulting in stable APIs.}


%The {\graphpy-GNN} then can do any additional pre-processing to generate a custom graph storage. 
%Therefore how the interfaces should be designed to allow passing such diverse graphs to {\graphpy-GNNs} so that each can keep its own custom storage with the single notion of graph object to unify the model layer definition and training without redefining everything from scratch for changes to graph storage or format? 




Numpy dtype can specify many properties, and hence C++ ideally needs a new \textit{class} definition to support their compilation. 
%Differences between Python (interpreter-based language) and C++ (compiler-based language) environments introduce an important challenge to support graphs with arbitrary properties. 
For example, we can use 
%GraphOne~\cite{kumar2017graphone}, which uses 
template meta-programming to define edge properties using a C++ \textit{struct}, and can write a Python binding for the same. However, each custom property requires a new  definition in C++, and new Python binding, followed by \textit{compiling} it for use in Python.
% However, we realize that the job of {\graphpy-SM} is just to prepare the graph and not to provide graph analysis, which may require the definition of real classes to access property fields in a C++ way. 
However, dtype is nothing but information about how an array element should be interpreted in Python, including the size and type of each element in the array. 
%Hence, it is very easy to go to a specific element to read or write to it, if back-end can store the dtype information, including the size of each field. 
% Also, it is very easy to parse the input files and perform the tokenization to support reading a good set of raw input files and preparing the graph representation from it.
Hence, {\myname-SM} uses void pointers, element size, and other information to support dtype, along with a convention that edge dtype should always specify the source vertex first, destination vertex next, then the edge properties. Hence, by knowing the size of the edge properties, we can easily prepare a graph in {\myname-SM} without defining the actual C++ structure for the same.

\subsubsection{Graph Preparation, Exchange, and Ownership.} 
Table~\ref{table-api} lists graph storage related APIs. Listing ~\ref{list-dtype} shows an example of how {\myname-SM} prepares graph representation from the user-defined edge structure using Python dtype, and passes the prepared graph to {\myname-System}. The {\myname-SM} uses multiple cores and can generate the optional edge ID. The parsing APIs \textit{$add\_edges\_from\_*$()} accept delimiters and flags to support different types of input files.
For complex input data format, we require that users directly parse using the Python IO library, and send the back-end a Numpy array of edges in batches or at once using \textit{add$\_$edges()} API. Python has very good APIs for file handling and tokenization. 



\begin{table}[t]
\caption{\small {\myname} Python APIs for Graph Storage Handling} % title of Table
\vspace{-6pt}
\centering \small % used for centering table
%\setlength{\tabcolsep}{1mm}
\begin{tabular}{|l| l l } % centered columns (4 columns)
    \hline %inserts a single line
     \textbf{{\myname-SM} Initialization APIs} \\
    \hline
%    graph \hspace{1mm} init() \\
%   \hline
 %   $vclass$  init$\_$vclass(vertex$\_$count, vclass$\_$name, flag)\\
%   \hline
    $G$ \hspace{2mm} init$\_$graph(vcount, flag, edge$\_$dtype, graph$\_$name) \\
%    \hspace{22mm} e$\_$dtype, graph$\_$name)\\
    \hline
    \textbf{Graph Preparation APIs of {\myname-SM} on $G$} \\
    \hline %inserts double horizontal lines
    int \hspace{1mm} add$\_$edges$\_$from$\_$file(file$\_$name, delimiter, flag)\\
    int \hspace{1mm} add$\_$edges$\_$from$\_$dir(dir$\_$name, delimiter, flag) \\
    int \hspace{1mm} add$\_$edges(np$\_$array, count) \Comment{\blue{Can be called many times}}\\
    \hline %inserts a single line
    \textbf{Some APIs of {\myname-SM} on $G$}\\
    \hline
    {np$\_$arr1, np$\_$arr2, np$\_$arr3, np$\_$arr4} \hspace{1mm} get$\_$csr(csr$\_$dtype) \\
    %\hline
    %{Numpy$\_$array, Numpy$\_$array} \hspace{1mm} get$\_$csc(graph, dtype) \\
    %\hline
%    np$\_$array \hspace{16mm} get$\_$coo(edge$\_$dtype)\\
    \hline
    % \hspace{6mm} \textbf{ Vertex Related APIs of $vclass$} \\
    % \hline
    % int \hspace{5mm} string$\_$to$\_$vid(vertex$\_$name) \\
    % string \hspace{1mm} vid$\_$to$\_$string(vid) \\
    % \hline
    \textbf{Some Graph APIs of {\myname-System}} \\
    \hline
    g  \hspace{12mm} wrap$\_$graph(np$\_$arr1, np$\_$arr2, np$\_$arr3, np$\_$arr4) \\
    status \hspace{6mm} save$\_$graph(g, path) \\
    g \hspace{12mm} load$\_$graph(path) \\
    vcount \hspace{5mm} get$\_$vcount() \\
    ecount \hspace{5mm} get$\_$ecount() \\
     \hline
\end{tabular}
\label{table-api} % is used to refer this table in the text
% \vspace{-12pt}
\end{table}


%In Line 5, we defined the Numpy dtype for edges that contain two properties, which are present in the dataset. In Line 6, we use the API \textit{init$\_$graph()} to create the \textit{graph} object using this dtype. Preparing graphs from raw data files is performed when the user calls  \textit{add-edges-from-file()} or \textit{add-edges-from-dir()} API (Line 7). \textit{First} step inside this API is to convert the file content to the edge list/COO format. 
% We dedicated a fixed size of the buffer to gather such edges. \textit{Second} step is to convert the gathered edges to CSR format in the background using multiple cores. To support different types of files, we allow the specification of \textit{delimiter} in such APIs.

%The conversion of the edges to CSR/CSC still happens in {\graphpy-SM} using many cores.
%The edge structure format can be replaced by other Numpy dtype based on the dataset. For example, the ‘float’ data can be replaced by another ‘int’, or it can contain more properties of any fixed size fields. 
% At Line 8, we add the edges from the files present in the input directory, which includes the raw data in the text format using space as a delimiter. The comma can be used as a delimiter for CSV files.

% To overlap these two processes, we trigger the conversion to CSR even before it is full. In that sense, these two processes are continuous.   

% Raw graph data can be in any format, including plain text files or CSV, or separated by any other delimiter. To handle these cases, the APIs accept the delimiter to handle the text or CSV files. 
%At this moment we only support text, CSV, and JSON files, with support for XML files underway. Also, the parsing can be done in Python and stored temporarily using a Numpy array, and {\graphpy-SM} provides \textit{add-np-edges()}. This API can be called many times, each time providing new edges, thereby simplifying the parsing job and not occupying huge memory.




%Python code highlighting
\begin{lstlisting}[language=Python, caption= {\small Illustration of graph creation in Python using {\myname-SM} and passing it to a {\myname-System}. Edges have one property.}, label={list-dtype}]
import Numpy as np
import gnnbench_sm as gp
import gnnbench_kernel as gpk
def prep_graph():
 edge_dt=np.dtype([('src', np.int32), ('dst', np.int32), ('eid', np.int32)]
 csr_dt=np.dtype([('dst', np.int32), ('eid', np.int32)]) #dtype for csr
 G = gp.init_graph(|V|,edge_dt,"reddit", gp.eDir)
 G.add_edges_from_dir('./InputDir/', ' ', gp.eEid)
 g = gpk.wrap_graph(G.get_csr(csr_dt))
\end{lstlisting}

%\vspace{-6pt}

% V = init_vclass(vcount, "vclass1", 0)
%csr_offset, csr_neighbor, csc_offset, csc_neighbor 
%kernel_graph = gpk.wrap_graph(csr_offset, csr_neighbor, csc_offset, csc_neighbor);


{\myname-SM} exports the graph in CSR/CSC in the form of four zero-copy NumPy arrays using \textit{get$\_$csr()} API (At Line 9). The first Numpy array contains the \textit{offset} of size $|V+1|$, while the second array contains N(v) of the vertices along with the embedded edge properties as specified using dtype. The rest of the two arrays are for CSC format. In the case of an undirected graph, both groups of NumPy arrays share the same underlying memory. The four arrays are sufficient to pass any CSC/CSR variants taking care of the direction, edge IDs, or any multi-field property, etc. 

These arrays can be passed to the $wrap\_graph$() API of the \myname-GNN (Line 9) to initialize its internal graph wrapping these arrays or may further pre-process the graph to derive a new format and return the kernel-graph object(g) which is used by other {\myname-System} APIs. 
%The {\graphpy-GNN} can simply store the underlying memory pointers as offset and neighbor arrays inside the  kernel-graph object to offer vanilla CSR/CSC; or may decide to further pre-process the graph to derive a new format, and return the corresponding kernel-graph object. 
%based on parameters being passed through $dict\_param$, a python dictionary data-type, 
Thus, the kernel-graph object is owned by {\myname-System}. The module can save it to disk ($save\_graph()$ API in Table~\ref{table-api}), or load it from there ($load\_graph()$ API in Table~\ref{table-api}) without affecting {\myname-SM} or its other consumers (\cref{sec.overview}). 
%To demonstrate, and to gain confidence that systems researchers can provide a custom graph storage, a graduate student implemented SNB graph format~\cite{gstore}, and demonstrated many GNN models using the same set of Kernel APIs of Table~\ref{table-kernel}. It is 2-D partitioned graph, with custom storage. 
%This is in contrast to DGL, whose monolithic {Kernel} module handles graph preparation, and offers data-access APIs on the prepared graph through the same kernel.
%which has many repercussions(\cref{sec.dgl}).
%including issues in supporting diverse graph storage.


%from COO format, to CSR/CSC format with an edge ID as its fixed edge property, and offers various data-access APIs from this  graph in Python. If a system researcher wants to customize the graph storage for better Kernel performance, it would be challenging to support its existing Python data-access APIs, which assume that the underlying graph is CSR/CSC. Also, spending effort on supporting these APIs is not useful when the aim is just the kernel optimization through better storage format but will leave the whole DGL code in a broken state due to its monolithic nature. Hence, the lightweight Kernel module in the plug-and-play eco-system of {\graphpy} provides enough space for innovations without the need to spend efforts on graph preparation or in supporting the APIs that are not applicable for deep learning purposes.



%So far, we have only discussed passing CSR/CSC NumPy arrays to $wrap\_graph$(); another variant of this API also accepts COO format, where the COO data can come from $get\_coo()$ API of {\graphpy-SM}. Also, they can instruct {\graphpy-SM} to not create graphs in the CSR/CSC format by passing appropriate value in the \textit{flag} in \textit{init$\_$graph()} API.
%However, if users are only interested in COO format for some reason, they can use \textit{get$\_$coo()} directly. However, COO data is available only if the user has chosen to persist the data, as we don't keep all the COO data in memory. 
% This argument is accept in init$\_$graph() API (not shown for brevity). 
%A {\graphpy-GNN} is free to do anything that it wants with the COO data, and {$wrap\_graph$()} must return a kernel-graph object. 


% %After we create the graph representation, future graph operations such as graph topology analysis, or GNN operations can use them and are discussed in \cref{sec.dl}. 
% {\graphpy-SM} provides direct access to the graph representation using the Numpy arrays.
% The \textit{get$\_$csr()} API returns the internal CSR representation using a pair of two arrays, as per Figure~\ref{fig-format}(d). The first Numpy array contains the \textit{offset} of size $|V+1|$, while the second array contains the neighbor information of the vertices along with the embedded edge weights.  The rest of the two arrays are for CSC format. In the case of an undirected graph, both are the same. Thus, a data scientist can directly use the Numpy arrays for any ad hoc analysis either in Python or can use any other Python package that accepts Numpy arrays. 

% so that data scientists can write ad hoc analyses themselves, or can be used by other modules if {\graphpy} does not provide those functionalities out-of-box, such as GNN operations can use the use them, and are discussed in \cref{sec.dl}. 


%We have provided graph analysis module written in C++ that accepts these Numpy arrays, and supports BFS, PageRank, WCC, SSSP etc. out-of-the-box to show that is is possible to use these arrays directly inside a specialized {\graphpy-GNN} module.
%Similarly, CSC representation can also be accessed in the Numpy arrays. 

 
% \begin{figure}
% \includegraphics[scale= 0.4]{result/dtype-crop.pdf}
% \caption{example about how to use dtype for graph creation}
% \label{fig:dtype}
% \end{figure}

% \begin{algorithm}[h]
% 	\caption{\small Illustration of graph creation in Python}
% 	{\small
% 		\label{algo-dtype}
% 		\begin{algorithmic}[1]
% 		    \State {import Numpy as np}
% 		    \State {import {\graphpy} as gp}
% 			\State {\blue{\# Create graph with correct dtype}}
% 			\State {edge$\_$dt= np.dtype([('src', np.int32), ('dst', np.int32), (‘wt', np.float)]}
% 			\State {G = gp.init$\_$graph(gp.eDdir, edge$\_$dt) \blue{ \# Directed graph}}
% 			\State {G.add$\_$edges$\_$from$\_$dir(“./input$\_$dir/”, “ ”) \blue{\# space is delimiter}}
% 			\State {{\blue{\# export the graph as Numpy array with correct dtype}}}
% 			\State {csr$\_$dt= np.dtype([('dst', np.int32), (‘wt', np.float)])}
% 			\State {np$\_$csr$\_$array= G.get$\_$csr(csr$\_$dt)}
% 		\end{algorithmic}
% 	}
% \end{algorithm} 




%As we mentioned above, some newly proposed Graph DL algorithms use edge information to perform machine learning tasks. As we mentioned above, some newly proposed Graph DL algorithms use edge information to perform machine learning tasks. Therefore, the graph representation structure needs to store the edge feature information.


%Because there is not a well-defined format for edge information. In other words, different users may prefer to use different data structures and data types to store edge information. By combing these data types and data structure, there may exist thousands of different ways of edge information storage structure users can adopt. The existing graph analytics can not store these edge information or can only store an edge in as the edge information (DGL).  E.g. [x,y] only support plain graphs that have no option to store edge ID or edge properties. GraphOne, is based on template meta-programming. By definition, it must define the vertex and edge-properties in C++ before compiling and deploying it. 
 
% This means when users want to define a vertex/edge properties by themselves, they need to find the source code, define a new vertex/edge property structure, enable Python binding on this,  and re-compile to deploy it. The above pipeline procedure is not a good experience for data scientists or machine learning engineers.
 
% Our works support the dtype, which means we do not need to touch the source code. Instead, users just need to write the user-defined vertex/edge property structure and put it in the Python dtype code and the whole library can support this arbitrary edge structure.  




% \vspace{1mm}
% \noindent \textbf{Parallel Parsing.}
% % There is one difference between the two cases. 
% API add$\_$edges$\_$from$\_$dir() can use multiple cores to do the parsing work in parallel for each file, and create binary edges out of it.
% It should be noted that parsing is a very slow task, and hence parallel parsing  as shown in Fig.~\ref{fig-parallel_pa} results in faster graph creation. Here, each thread handles one file and batches them in an edge log buffer. The internal CSR converter code picks those multiple edge log buffers and converts them to CSR format using multiple threads. 
% % Thus, parsing and conversion both work concurrently utilizing multiple threads. 





% \begin{figure}[t]
%   \includegraphics[scale= 0.5]{result/high_per.pdf}
%   \vspace{-6pt}
%   \caption{{\graphpy} Parallel Parsing to produce binary edges. The CSR conversion code works concurrently to this process and operates on all the edge log buffers.}
%   \label{fig-parallel_pa}
% %   \vspace{-6pt}
% \end{figure}

% \subsubsection{Supporting Bipartite and Multiple Graphs}
% %\noindent \textbf{Supporting Bipartite and Multiple Graphs.}
% Supporting sparse tensors as in weight pruned fully connected layer requires support for a bipartite graph, which is a graph-like relationship between two different vertex ID spaces. To support that, the API  $init\_graph$() accepts two $vclass$ objects representing the two vertex ID spaces. In the case of homogeneous graphs, we only need to create one $vclass$ object.
% The data access APIs for bipartite graph still works in the same way. The different vertex count is well reflected in the offset Numpy arrays, hence {\graphpy-GNN} module uses it to derive this information about the bipartite graph. Thus the rest of the APIs remain the same for supporting bipartite graphs. 

 

% Moreover, a sparse model may be composed of many sparse layers, thus we need to support multiple independent bipartite graphs. This is achieved easily by calling init$\_$graph() many times, passing the correct vclass objects and other arguments. Thus, each returned $graph$ object represents one graph. 



% \vspace{1mm}
% \noindent \textbf{Vertex ID Space.}
% When the vertex  identifiers are in string format, the \textit{vclass} converts them to numerical IDs.
% % which is created using \textit{create-vclass()} API. 
% We provide $string\_to\_vid$() API to be used in Python. 
% %Internally, it is managed using Intel thread building block library's hash. If user requires the conversion of vertex ID to string, $vid\_to\_string$() API can be called.
% In many cases, the graph is already in the numerical ID, and hence we do not need to do the conversion. 
% %In this case, $init\_vclass()$ can directly be informed of the same using the \textit{flag}. In this case, exact number of vertex count needs to be passed using \textit{vertex$\_$count} argument. 
% We also support arbitrary vertex properties, but for brevity we treat the vertex string name as the only property in this paper. 

% \subsubsection{Data Access and Graph Analysis}
%{\graphpy-SM} offers NumPy arrays for CSR/CSC, and can be used for data access in Python directly, if needed, for any ad hoc graph analysis in Python. 

% \noindent \textbf{Graph Analysis.}
% For high-performance graph analysis, another module has been written that provides all built-in graph analysis, such as BFS, PageRank, Connected Components, etc. out-of-the-box to show that it is possible to use these arrays by other modules. 
% %inside a specialized {\graphpy-GNN} module, 
% which can be helpful in ad hoc data science applications as in GraphSage~\cite{graphsage17}. However, we do not evaluate it as it is outside the scope of the paper.
% %The module also offers GAS Framework.





==> tex/background2.tex <==

\section{Background on GNN Computation} \label{sec.background}
%We now present background on graph representation, deep learning computation. 
%We also take this opportunity to present related works on graph neural networks (GNNs), model sparsity, and traditional graph data science use-cases.

%\subsection{Graph Representation} \label{sec.background.graph}

\noindent \textbf{Graph Storage Formats.}
A graph is represented as G = (V, E, W), where V and E refer to the vertex and the edge set respectively, while W refers to the optional edge weight or property that can be  of arbitrary size including multiple fields. 
Fig.~\ref{fig-format} shows an example of a weighted graph and its corresponding representations. 
The \textit{compressed sparse row} (CSR) format stores all the neighbors ($N(v)$) of the vertex sequentially and uses the offset array to link the vertex and the first edge of its corresponding N(v). The reverse graph in the case of a directed graph is also needed to be stored; in this case, CSR stores out-neighbors while \textit{compressed sparse column} (CSC) format stores the in-neighbors of each vertex. The \textit{degree} of a vertex is the length of N(v).


%\emph {Edge list}/coordinate list (COO) format stores the graph data as an array of edges, and stores every edge and its corresponding weight sequentially as shown in Fig.~\ref{fig-format}(b). 
% The COO format can be easily updated, as the new incoming edge can be directly appended to the list. However, getting all the neighbors of a vertex include an O(E) search. 
%Hence, we need to search the whole list to get the neighbor information for the specific vertex. 
% The dense matrix representation of graph is called the  \textit{adjacency matrix}. It is a $|V| *|V|$ matrix, and the elements of the matrix represent whether the pair of vertices are connected or not, and store the weights or 1 (for unweighted graph). 
% % Although the searching procedure for neighbor information is very efficient, 
% %to \emph{O(V)}, 
% However, it cannot handle the sparsity of the graph efficiently as there are more zeros than the non-zero entries in the adjacency matrix. 

%In this paper, we discuss about the need to store \textit{edge ID} to be used by both the CSR and CSC format to access the same copy of edge-level tensors. 
 
%
% \begin{wrapfigure}{r}{9.0cm}
% 	%\begin{figure}[t]
% 	\centering
% 	\vspace{-4mm}
% 	\includegraphics[scale=0.5]{result/graph_combine.pdf}
% 	\caption{Stream analytics on network monitoring data need , and may get benefited by their concurrent execution. } 
% 	%		{\name} proposes a different grouping of phases to enable data movement using adjacency list format instead of using edge list format. In addition, {\name} also introduces asynchrony and concurrent execution of each phase to enable concurrent execution of diverse set of graph analytics within one or many sets of {\cvertex s}.}
% 	\label{fig-lanl}
% 	\vspace{-6mm}
% \end{wrapfigure}
%


%\subsection{GNN Computation} \label{sec.background.dl}

%Deep learning (DL) frameworks, such as TensorFlow \cite{abadi2016tensorflow}, Pytorch \cite{paszke2019pytorch}, Theano \cite{al2016theano}, Keras \cite{gulli2017deep}, etc. create a \textit{computation graph} or \textit{directed acyclic graph} (DAG). 
%The core functionality of each layer is implemented  in high-performance languages like C/C++, CUDA etc., and are called \textit{kernels}. 
%They are invoked automatically by the computation graph during training.

%In the \textit{forward} procedure, it calls a sequence of \textit{kernels}  from the input layer to the output layer to derive the prediction value, which is compared with the ground truth label to calculate the loss.
% and plug the loss into the backward procedure. 
%Then, in the \textit{backward} procedure, the loss is used to calculate the gradient by calling a sequence of kernels from the output layer to the input layer. It uses the chain-rule of gradient back-propagation to update the model parameter from it.

\noindent \textbf{State Tensor and Edge ID.}
DL training has forward and backward computations, as discussed in \cref{sec.intro}. 
The intermediate features and the model parameters are called \textit{tensors}.  Many tensors that are used and produced in the forward computation and are using by backward, called \textit{state}. 
For GNN, the trainable tensors are at vertex-level ($X$ and $Y$); and at edge-level ($W_e$ as attention score in GAT and GaAN). 
Both of these types of tensors ($W_{e}$, $X$ and $Y$) are used as \textit{states}, as shown in Fig.~\ref{fig-format}(a). 
Since, backward computation happens on the inverse graph (CSR), as opposed to using CSC during forward computation; the CSR and CSC  must share the same copy of the state tensors. This is handled by the vertex ID indirection for vertex-level tensors ($X$, $Y$), which is already present in the graph storage. However, for edge-level tensors ($W_{e}$), graph storage needs to introduce \textit{edge ID indirection} (Fig.~\ref{fig-format}(c) and (d)) for many GNN models. 


\noindent \textbf{GNN System and Stable API.}
The system code is referred to as the \textit{GNN system} and its Python APIs as \textit{system API}, while the model code, usually written in Python, is referred to as is.
The system API is called \textit{stable} if its signature does not require changes when a parameter, such as a graph object simply changes its format. 

\noindent \textbf{Autograd} refers to a class that contains forward() and backward() as its member function. 
%When this class is instantiated during the forward computation, 
The DL framework automatically invokes the backward() during the training using its \textit{computation graph} which is generated by the DL framework.


%and can be a vector as in case of multi-head attention. 
%In GAS forward, $W_e$ is calculated using a series of gSDDMM kernel, that takes various reduce operations of sum, min, max, etc in forward computation. Its one input tensor is a vertex-level, while the second input tensor can be either vertex-level or edge-level tensor. $W_e$ is used as edge weights (scalar or vector) in the gSpMM to calculate vertex-level tensor Y. In GCN, $W_{e}$ is absent in (unweighted) gSpMM. In its another variant, gSpMM only accepts an edge-level tensor to calcuate the output Y, and accepts various reduce operations.


%For completeness, some gSDDMM kernel during backward does not need an inverse graph.


% These graph deep learning works use the adjacency matrix A to represent the graph structure, and the matrix F represents the vertex features and performs matrix computations to perform the classification tasks. However, since most graph structures are sparse, the matrix operations in graph deep learning will mainly become sparse tensor operations. 
%which becomes hard to achieve good memory or computation performance. 


% {\color{red}
% \subsubsection{GNN System Component.}
% The infrastructure of GNN computation infrastructure consists of 3 components of different levels of granularities. The first coarse-grained component is module, which contains the model information of the GNN, such as the number of convolutional layers and the activation function between different convolutional layers if needed. The second component is the convolutional layer, which includes a sequence of different operators to perform the computation. The third fine-grained component is the operator, which uses GAS kernel functions or traditional sparse kernel to perform the forward and backward computations.
% }


%\subsubsection{Traditional Graph Analysis}
%Graph analytics systems~\cite{kyrola2012graphchi,roy2013x,nguyen2013lightweight,liu2017graphene,powerlyra2015eurosys,gstore, zheng2015flashgraph,mosiacEuroSys17, roy2015chaos, han2013turbograph, kumar2017falcon, zhu2015gridgraph,hong2012green, wu2015g, ai2017squeezing, zhu2016gemini,liu2015enterprise} have supported traditional graph topology analysis, while many of them supported unsupervised learning as well. 
%These systems were the ones that popularized the GAS programming.
%Kindly note that NetworkX~\cite{networkx08}, a purely Python package continues to be popular among data-scientists due to the ease of Python environment despite being very slow compared to them.
% These works pre-process the raw input data to create the graph representation and then perform the graph topology analysis. None of them, are able to support arbitrary edge properties. They allow at max one additional field for edge weights.

%\subsubsection{GNN}  \label{sec.gnn-background}
% Graph convolution network~\cite{gcn17iclr}(GCN), graph attention network~\cite{gat18iclr}(GAT), GIN~\cite{xu2019powerful}, GGNN~\cite{gatedgraph2017}, GaAN~\cite{zhang18} etc. are collectively called \textit{graph neural networks} (GNN) that specialize deep learning on graph data.
%The DL frameworks do not yet support sparse operations efficiently. Sensing the gap, a number of GNN frameworks were proposed recently, such as DGL~\cite{dgl2019}, NeuGraph~\cite{neugraph19atc}, AliGraph~\cite{yang2019aligraph}, Pytorch-Geomertric~\cite{pytorchg2019}, etc.
%GNNs ~\cite{gcn17iclr,gat18iclr, xu2019powerful,gatedgraph2017} are frameworks for representation learning on sparse data or graphs. 
%The forward computation uses a series of sSpMM and gSDDMM kernels. 



% \begin{figure}[t]
%   \includegraphics[scale= 0.64]{result/gnn-crop.pdf}
%  \vspace{-12pt}
%   \caption{\small GNN Forward and backward mode: X and Y are intermediate features, and $W_e$ is the model parameter of the layer, e.g. attention score in case of GAT. X, Y and $W_e$ tensors are \textit{state}, as it is used in forward and backward both. $A$ and $A^T$ are graph and its inverse respectively.}
%   \label{fig-forward}
% %   \vspace{-12pt}
% \end{figure}




%on the need for edge ID, edge-level tensors, various versions of gSpMM and gSDDMM  are also state tensors, therefore to access the correct edge features of an edge, we need to store the edge ID in both the CSR and CSC format.


%Because of the aggregation difference, different types of GNN models have different system-level implementation requirements.  

% \textbf{gSpMMve}
% This type of GNN models uses the weighted sum to aggregate the vertex-level neighbor feature. It first fetches the edge-level tensor to get the weight score and then uses it and the neighbor's feature to do the aggregation, 


% \textbf{GSMMe}

% \textbf{gSDDMMvv}

% \textbf{gSDDMMve}





%{\td   both sampling and no accuracy\cite{song2022rethinking}}
%{\td both sampling and multiple GPUs \cite{lin2020pagraph}}

% %\vspace{1mm}
% \noindent 
% \textbf{Sparse Kernels.}
% Prior works~\cite{gilmer2017neural,battaglia2018relational,dgl2019} have identified two important sparse kernels, that can be abstracted by the gather apply scatter (GAS) operations:
% %that various GNN kernels can easily be modeled using one or more of weighted and unweighted 
% generalized sparse matrix dense matrix multiplication (gSpMM); and generalized sampled dense dense matrix multiplication (gSDDMM).



% For the sake of brevity, we use the term kernel rather than GAS framework in many places for GNN operations.

% Traditional graph data analysis works mainly focus on analyzing the graph topology, such as the degree information, BFS, PageRank, Connected Components, Community Analysis etc. These works~\cite{227800, kumar2016g,nguyen2013lightweight,low2012distributed, zheng2015flashgraph} also provide the APIs, that are modeled after GAS framework. 




==> tex/dsl.tex <==

%\textbf{Automatic System Integration through DSL.}
\section{Automatic System Integration through DSL}
Listings~\ref{list-spmm} and \ref{list-pybind} discussed earlier represent the system integration code of {\myname} with a DL framework. Both the listings and related code are generated automatically from  the kernel signature using our simple domain-specific language (DSL). 
{\myname} just uses a file written in  DSL as the input, which is almost the same as a function signature in C++, except that it must use our array$\_$t to denote the tensor. 
%Our auto-generator code implements this DSL, and generates various files to be used in {\graphpy-GNN} as well as in {\graphpy-Workflow}. 
Listing ~\ref{dsl} shows an example of the DSL specification for one kernel.
%The generator generates the boilerplate code for the {\graphpy-Workflow} completely as shown earlier in Listing~\ref{list-spmm} for CPU version. 
The generated code is slightly different for GPU listing where tensor allocation happens in GPUs and is not shown here for brevity. The code also generates the skeleton code for autograd that is needed to make the kernel call in any layer, so that backward computation of the kernel  can be called automatically. However, DSL does not know details about backward computation logic, and hence it is the job of the researcher to fill the generated skeleton. 

%Python code highlighting
\begin{lstlisting}[language=Python, caption= {\small DSL example for gSpMMv system API. We generate the boilerplate code of Listing \ref{list-spmm} and \ref{list-pybind}, and the stub calling CUDA kernel. We also generate autograd skeleton (not shown).}, label={dsl}]
#System API specification in DSL file
status gSpMMv(graph_t& g, array_t<float>& input, array_t<float>& output, int reduceFn, int Forward); 
#Generated stub for calling actual C++/CUDA kernel 
status invoke_gSpMMv_impl(graph_t& g, array_t<float>& input, array_t<float>& output, int reduceFn, int Forward); 
\end{lstlisting}
\vspace{-6pt}


%the auto-generator generates the Listing \ref{list-spmm}.
%For {\graphpy-GNN}, the auto-generator generates a common CPU and GPU version of the APIs with the Python binding as shown in Listing~\ref{list-spmm}. 
%The difference between CPU and GPU version arise inside $\_gspmm()$ function.
Thus, a system researcher is only responsible for actual system API implementation. 
It should be noted that a new signature is needed when we may want to fuse different APIs together whose signature is then very different from the one listed in Table~\ref{table-api}, but not when customizing graph storage. Further, if any change in the signature of the API is required, the DSL helps with generating new system integration code, and thus {\myname} speeds up the prototyping.

%Hence, any custom kernel specification is automatically integrated into the DL framework, giving the impression that APIs are natively part of it.
% \noindent \textbf{Need of a New Baseline.} 



\subsection{Alternative Designs and Discussions} \label{sec.discuss}
%DGL implements Workflow in Python and Kernel in C++/CUDA. 
%DGL differs from the earlier method as the solution relies on the {Kernel} module to implement its own tensor library, which is made inter-operable with the DLPack tensor using \textit{full} DLPack protocol's ``consume'' step. 

\noindent %$\bullet$
\textbf{Tensor Exchange.}
DGL implements the ``consume'' protocol, as DGL and DLPack tensors are open-sourced under the same organization in GitHub, hence they know the protocol well. However, they developed an elaborate tensor library (visible in Python) for the same as per the ``consume'' requirement. 
%and converts DLPack tensor to their tensor data structure (visible in Python) following the "consume" protocol of DLPack using Python APIs. 
On the other hand, \textit{DLPack Sharing} protocol does not need any tensor library. Instead, {\myname-System} uses an internal data structure (e.g., $array\_t$) that is not visible in Python. Hence, anybody can design it, as it merely needs to keep the pointer, shape, and size. 
It should be noted that we studied many code bases, and hence best practices are incorporated from them, such as allocating output tensors in Python and not inside the {\myname-System} (Listing~\ref{list-spmm}).

%The proposed simple solution seems very attractive compared to options where solutions are based on workarounds and hit and trial due to missing documentation and restricted interfaces. 
%which we formalized by generating a system integration code to achieve productivity. 
%The proposed mechanism is powerful enough to solve all of the interface problems that we discussed in \cref{sec.obs} and \cref{sec.usecase}. 


%Data preparation and passing it to the kernel can be challenging when storage needs are different. 
%Designing an intelligent interface can simplify kernel prototyping efforts. Prior works have not focused on this step of data science.

% % On the other hand, {\graphpy-SM} makes graph available in CSR/CSC using zero-copy NumPy arrays using dtype for edge properties. 
% Numpy package is very standard and is part of almost every scientific Python package to specify matrix elements, and exchange the matrix data. Further, dtype has also been implemented by the tensor data structure. 
% E.g., passing image data to PyTorch's convolution layer, we use tensor data-structure and dtype.
% Hence, by designing {\graphpy-SM}, we demonstrate that graph (or sparse matrix) can also be specified and exchanged the same way as dense matrices.
% %Further, the utilities that offer Python binding, such as Pybind11 provides out-of-the-box support for Numpy arrays. Hence, our module is as standard and usable as the NumPy package is.

% In a nutshell, {\graphpy-SM} is a very lightweight and highly customized graph storage. It enables data sharing with other modules using Numpy arrays. We believe, this captures sufficient requirements for ad hoc and specific graph data science use-cases that we discuss in this paper. 

\noindent %$\bullet$
\textbf{Graph Edge Property Specification and Exchange.}
GNN systems, such as DGL follows \textit{ad hoc methods} and private methods to prepare graph.
%do not provide the capability to create graph representation from the raw data, such as the CSV, and text files. They support graph in captive form, i.e. for its internal use-cases only, and does not make them available to other modules. E.g., DGL 
It expects the user to parse the dataset and also store the reverse edges in an edge list array. It then \textit{always} creates {a directed graph with edge ID} from the doubled edge list array irrespective of whether edge ID is needed or not. 
%Further, actual data are seldom found in this format, and hence users need to perform file handling themselves.
GNNAdvisor manually parses the file in Python and relies on SciPy~\cite{2020SciPy-NMeth}, %SciPy can only provide unweighted graph support, and 
which cannot support edge ID creation. 
%and has not demonstrated attention-based GNNs. 
%NetworkX~\cite{networkx08}, a pure Python package, cannot provide high performance.
%is also similar except that it is difficult to introduce the parallel graph preparation due to its pure Python nature and hence cannot be used in the Kernel module directly. 
%Dynamic graph systems~\cite{macko2015llama,ediger2012stinger,kumar2017graphone,kumar2020graphone,dhulipala2019low} etc. can create graph efficiently using C/C++.E.g., GraphOne~\cite{kumar2017graphone} provides arbitrary multi-field edge property support using template meta-programming. But it requires that users write a plugin, including a \textit{struct} to capture the property and a few other functions, and then must \textit{compile} it. 
Most static graph systems~\cite{shun2013ligra,nguyen2013lightweight} are limited to supporting a one-field edge weight such as a floating point or none, that must be compiled separately generating two binaries but does not support edge ID natively.





==> tex/exp.tex <==
\begin{table}[t]
\footnotesize
\caption{\small Dataset details. * indicates labeled dataset, while the rest use 150 generated features and 7 predication classes.} % title of Table
\vspace{-6pt}
\centering % used for centering table
\begin{tabular}{l l r r r r} % centered columns (4 columns)
    \hline\hline %inserts double horizontal lines
    Graph & Vertex & Edge & Feature & Prediction\\ [0.5ex] % inserts table
    Dataset & Count & Count & Length & Class\\ 
    %heading
    \hline % inserts single horizontal line
    Cora(G0)* & 2,708 &  10,858 & 1,433 & 7\\ 
    Citeseer(G1)*  & 3,327 & 9,104 & 3,703 & 6\\
    Pubmed(G2)* & 19,717 &  88,648 & 500 & 3\\
    Amazon(G3) & 400,727 & 6,400,880 & 150 & 7\\ 
    %wiki-Talk	& 2,394,385	& 5,021,410 \\
    %Web-BerkStand & 685,230	& 7,600,595  \\ 
    %roadNet-CA	&1,971,279&	11,066,420\\
    As-Skitter(G4) & 1,696,415 & 22,190,596 & 150 & 7\\
    Cit-Patent(G5) & 3,774,768 & 33,037,894 & 150 & 7 \\ %16,518,948 \\  
    Stackoverflow(G6) & 2,601,977 &	95,806,532 & 150 & 7\\ %63,497,050\\
  %  Kron-21 & 2,097,152 & 67,108,864\\
    Hollywood(G7) & 1,069,127 & 112,613,308 & 150 & 7\\
    LiveJournal(G8) & 4,847,571 & 137,987,546 & 150 & 7 \\
    OGB-Prduct(G9)* & 2,449,029	& 123,718,280 & 100 & 47 \\
    Reddit(G10)* & 232,965 & 229,231,784 & 602 & 41 \\
    Orkut(G11)* & 3,072,627 & 234,370,166 & 150 & 7\\
    UK-2002(G12) & 18,520,486 & 596,227,524 & 150 & 7 \\
    Kron-25(G13) & 33,554,432 & 1,073,741,824 & 150 & 7 \\
 %   LANL & 31,142 & 115,949,436 \\
    % Kron-20 & 1,048,576 & 10,485,760\\
    % [1ex] % [1ex] adds vertical space
    \hline %inserts single line
\end{tabular}
\label{table-dataset} % is used to refer this table in the text
\end{table}
% {\graphpy} is implemented using C++/CUDA and Python, and will be open-sourced. {\graphpy} is fully integrated with Pytorch for many GNN and sparse layers case. Integration with Tensorflow is done for GCN case only to show that integration with any general-purpose DL framework is possible that exports their tensors as DLPack tensors.
% It contains roughly around 4000 lines of code for {\graphpy-DE},
% uses some code-base from an open-source graph system, but sufficient changes were needed to implement Dtype and parallel parsing. The size of generated critical boilerplate code is roughly 1000 lines, while kernel size is 2400 lines for reference CPU and GPU implementation for DL kernels.
% We also, added support for parallel graph parsing support. At the end of data ingestion, we prepared a pure CSR/CSC graph from the internals of adjacency list representation of GraphOne. The same CSR/CSC graph was exported as numpy arrays. It is complex to come up with an exact number of lines of code changes here, but we roughly added/modified more than 2000 lines of the code.

% The lines of code are listed in Table~\ref{table-code} for Pytorch. As we mentioned earlier, the boiler-plate code in Python, Pybind11 and kernel invocation are all auto-generated using the provided DSL script. When integrating with Tensorflow, {\name-Kernel} remains same.


% The code can be separated as 2 parts, c++ computation kernel code and python-based GNN binding code. Table 4 provides the code size in terms of the number of lines summary information.

% \begin{table}[h]
% \caption{Summary Information about code size.} % title of Table
% \vspace{-6pt}
% \centering % used for centering table
% \begin{tabular}{|l| r| } % centered columns (4 columns)
%     \hline\hline %inserts double horizontal lines
%     File & Code size\\ [0.5ex] % inserts table
%     %heading
%     \hline % inserts single horizontal line
%     % {\graphpy-DE}  & 5000 Lines \\
%     {\graphpy-Kernel} Boiler-plate Code & 649 Lines\\ 
%     {\graphpy-Kernel} Implementation & 2400 Lines \\ 
%     % {\graphpy-Kernel} Implementation (GPU) & 565 Lines \\ 
%     {\graphpy-Workflow} + DL Model layers & 593 Lines \\
%     % python GNN binding(with GAT, GCN) & 499 lines  \\ 
%     % DGL backend (without CUDA, GAT, GCN)& 2008 lines  \\
%     % [1ex] % [1ex] adds vertical space
%     \hline %inserts single line
% \end{tabular}
% \label{table-code} % is used to refer this table in the text
% \end{table}

\section{Evaluation} \label{sec.exp}
We show the impact of better high-level interfaces between the DL framework and GNN system, and GNN-specific kernel design while following the recommendations proposed in \cref{sec.obs}.
%baseline and interface design on 
We use memory consumption and speedup achieved due to framework overhead and requirement mismatch as main metrics to compare {\graphpy} to prior works.
%Our gSpMM kernels are implemented using vertex-level and feature-level~\cite{yang2018design} parallelism, which we believe forms a reference on top of which researchers try to optimize kernels. gSDDMM kernels use COO format and use edge-level parallelism.
%And,  
%Even with such a simple implementation, we indeed show that by in-depth analysis of different components for performance, framework overhead, memory consumption, as well as end-to-end accuracy of the model training,  
%uncover some useful insights for the progress of system research and can influence the course of the research direction.
The dataset for the experiments are listed in Table~\ref{table-dataset}. Only Cora, Pubmed, Citeseer, Reddit, and OGB-product datasets are labeled. The first three datasets are referred to as small. The experiments are run on  Nvidia A100 GPU, which has 40GB of memory.
%a single socket 4-core Intel CPU with up to 3.60GHz  machine, and DRAM of 16GB loaded with Ubuntu 18.04.
% i7-4790 


We focus on node classification using GCN, GIN, and GAT (with 1 and 3 heads implying edge feature length). In GCN and GAT, the intermediate feature length is 16, which implies that GAT-3 has 48 as the feature-length for each vertex. For GIN, the  intermediate vertex feature  length is 64. The feature lengths have been set based on the code of the original model paper. 
We test DGL~\cite{dgl2019}, PyG~\cite{pytorchg2019}, GNNAdvisor~\cite{wang2021gnnadvisor}, Huang et al~\cite{huang2021understanding},  GE-SpMM~\cite{gespmmsc2020}, and FeatGraph~\cite{featgraphsc20}. However, end-to-end training can only be performed in DGL, PyG, and GNNAdvisor (partial) due to various issues discussed earlier.


%\red{optimized overhead, better baseline} and usefulness in graph data science, for which we argued in the rest of the paper, including using in education and research, and writing new kernels for sparse layers that was not done in prior graph DL systems, as well prototyping kernels in SNB format. 

%We now explore whether a framework with better system design alone can provide performance gain when implementation is purely for reference purpose using vanilla CSR/CSC format devoid of any specific optimization. \red{Our kernel is implemented for referenced purpose instead of the kernel optimization as existing works. It uses the vertex level and feature level parallel and only reduce the overhead time. }



%We are specifically interested in measuring the framework overhead, and 
%We will also be showing the performance impact when any optimization techniques are not evaluated in a training loop for accuracy.



%Hence, we evaluate several data science use-cases, as well as benchmark the graph preparation time.




% Like prior works~\cite{dgl2019,featgraphsc20}, we run the performance experiments for 200 epochs for 10 times and average the result.


% E.g., Cora dataset is a citation network data set that has 2708 publications, treated as the nodes, and 5429 citation links, treated as the edges.
%Cora,  PubMed \cite{yang2020heterogeneous}, amazon \cite{leskovec2007dynamics}, and patient citation network \cite{leskovec2005graphs}, and LANL~\cite{turcotte17} are all real-world graphs. 
%Only LANL is a multi-field property graph, where each edge has 9 properties. %We use it for showing {\graphpy-DE} capability, while others may need to store edge ID for GAT.
% We also used graph500 generator~\cite{graph500} to generate Kron-20 graph, which is stored in 16 files. We use this dataset to show that parallel parsing of the file improves the graph preparation time. 


\subsection{GNN Training: Accuracy} \label{sec.exp-gnn}


%of {\graphpy} with DGL, Pytorch-Geometric (PyG), and GNNAdvisor to show that {\graphpy} is working.
% but not NetworkX as it is not designed to support DL operations. 
% {\graphpy} used the same three data set as (Cora, Citeseer and Pubmed (Kipf & Welling, 2017)). 





\noindent \textbf{PyTorch Integration.}
Fig.~\ref{exp-accuracy} shows the accuracy of {\graphpy}, DGL, and GNNAdvisor. 
We run each model for 1,000 epochs and printed training accuracy after each epoch to make sure that accuracy is captured correctly.  
%As we outlined earlier, many prior works such as GNAdvisor do not offer class A GNN, e.g., GAT.

Except for GNNAdvisor, the rest have almost similar accuracy for GCN with minor fluctuations. 
%These are due to random weight initialization that converges to the same number if run again. PyG shows lower accuracy for GIN. %Similar fluctuations are also observed in DGL. 
GNNAdvisor achieved significantly less accuracy than DGL and {\graphpy} for GCN. As we explained earlier it did not use bias in its GCN convolution layers, and the order of normalization by degree is wrong in the backward computation. Its paper also does not report accuracy. To see the contribution of bias on the accuracy, we commented bias in {\graphpy}, but the accuracy did not drop more than 5\%, e.g., in Cora, it achieved 78.3\% versus the original 83.4\%, while GNNAdvisor only achieved 69.5\%. 
%Hence, we suspect more bugs in GNNAdvisor.  
GNNAdvisor also could not train on Reddit and OGB-Product, it throws an invalid memory access error, which is also reported by prior work~\cite{fu2022tlpgnn}.
%and for GIN ``$CUBLAS\_STATUS\_NOT\_INITIALIZED$ when calling cublasCreate(handle)'' error. Unfortunately, the last error has nothing to do with cublas as it merely indicates that no memory is left for initializing cublas, a library provided by Nvidia. 
Indeed, GNNAdvisor has not evaluated any larger dataset. It has no GAT support.


\begin{figure}[t]
  \includegraphics[scale= 0.46]{exp/accu-crop.pdf}
  \vspace{-36pt}
  \caption{\small Accuracy comparison for many GNNs on the labeled dataset} %Missing results are due to out-of-memory conditions.}
  \label{exp-accuracy}
% \vspace{-12pt}
\end{figure}

% \begin{table}[t]
% \footnotesize
% \caption{Accuracy evaluation results for various datasets for 200 epochs. GAT-1 and GAT-3 represent single-head attention and 3-head attention mechanism in GAT. \td GIN and PyG results.} % title of Table
% \vspace{-6pt}
% \centering % used for centering table
% \setlength{\tabcolsep}{1.0mm}
% \begin{tabular}{|l| rrr|rrr|rrr|} % centered columns (4 columns)
%     \hline\hline %inserts double horizontal lines
%      & \multicolumn{3}{c|}{Cora} & \multicolumn{3}{c|}{Pubmed} & \multicolumn{3}{c|}{Citeseer}\\
%     \cline{2-10}
%         & DGL  & {\graphpy} & PyG & DGL  & {\graphpy} & PyG & DGL  & {\graphpy} & PyG \\
%     %heading
%     \hline % inserts single horizontal line
%     GCN & 83.10\%  &  83.40\% & 73.7\% & 76.50\%  &  76.52\% & 71.50\% & 65.40\%  &  65.10\%  & 50.30\%\\ % inserting body of the table
%     GAT-1 & 76.70\% & 76.90\% & 71.97\% &76.50\% & 75.12\% & 77.35\% & 60.30\% & 61.46\% & 54.20\%\\
%     GAT-3 & 77.70\%  & 78.10\% & 73.10\% & 75.40\%  & 75.44\% & 77.50 \% & 64.80\%  & 64.76\% & 57.10\%\\
%     GIN & 76.10\% & 74.10\% & 66.03\% & 74.23 \% & 74.50\% &35.73\% & 50.40 \% & 49.30 \% & 16.90\%\\
% %    [1ex] % [1ex] adds vertical space
%     \hline %inserts single line
% \end{tabular}
% \label{table-accuracy} % is used to refer this table in the text
% \end{table}



The results (Fig.~\ref{exp-accuracy}) clearly outline that {\graphpy} works end-to-end and prove that the proposed Half DLPack protocol works and has no side effects, even though we did not follow the ``consume'' protocol to handle the DLPack tensor.

 


%which has serious measurement implications as we discus next. 
%And, as we identified, the overhead dominates in such dataset, therefore we believe reference implementation of {\graphpy} is better suited as a baseline system that future researchers can use to show better system performance on larger datasets, or smaller overhead on smaller dataset. 
%For PyG, it materializes the scattered messages as part of GAS, which causes




% \begin{table}[h]
% \small
% \vspace{-6pt}
% \caption{\small {\graphpy}-TensorFlow vs {\graphpy}-PyTorch accuracy comparison for GCN.} % title of Table
% \vspace{-6pt}
% \centering % used for centering table
% \begin{tabular}{|l| r| r|} % centered columns (4 columns)
%     \hline\hline %inserts double horizontal lines
%     Graph Dataset & {\graphpy}-Tensorflow & {\graphpy}-Pytorch\\ [0.5ex] % inserts table
%     %heading
%     \hline % inserts single horizontal line
%     Cora & 83.18\% &  83.40\%\\ 
%     Citeseer & 65.32\% & 65.10\%  \\
%     PubMed & 76.47\% &  76.52\%\\
%     Reddit & 92.89\% &  92.96\%\\
%     OGB-Product & 69.76\%& 69.67\%\\
%     % Kron-20 & 1,048,576 & 10,485,760\\
%     % [1ex] % [1ex] adds vertical space
%     \hline %inserts single line
% \end{tabular}
% \vspace{-6pt}
% \label{table-graphpy-TFvsPT} % is used to refer this table in the text
% \end{table}

\noindent \textbf{TensorFlow Integration}. 
We also test GCN on TensorFlow to show that {\graphpy} can work with it. We achieved similar accuracy for GCN training for all the labeled datasets. 
%as shown in Table~\ref{table-graphpy-TFvsPT}. 
This suggests that integration with almost any DL framework is possible that offers a DLPack tensors conversion routine. 
For the rest of the comparison, we focus on PyTorch integration, as related works are also integrated into it.

% \begin{table*}[t]
% \caption{Graph DL training time (in \textit{Milliseconds}) based on different GNN models for 200 epochs. } % title of Table
% \centering % used for centering table
% \setlength{\tabcolsep}{1.3mm}
% \begin{tabular}{|l rrrrrr| rrrrrr|} % centered columns (4 columns)
%     \hline\hline %inserts double horizontal lines
%           & \multicolumn{6}{c|}{CPU} & \multicolumn{6}{c|}{GPU}\\
%     \hline
%           & \multicolumn{2}{c}{Cora} & \multicolumn{2}{c}{Pubmed} & \multicolumn{2}{c|}{Citeseer} & \multicolumn{2}{c}{Cora} & \multicolumn{2}{c}{Pubmed} & \multicolumn{2}{c|}{Citeseer}\\
%     \hline
%     Method & DGL  & {\graphpy} & DGL  & {\graphpy} & DGL  & {\graphpy} & DGL  & {\graphpy} & DGL  & {\graphpy} & DGL  & {\graphpy}\\ 
%     \hline % inserts single horizontal line
%     GCN        &    1819.14  & 959.74 &   4316.49  &  3060.49 &   3755.371    &  2108.99  &  900.00    &  1061.39  &   883.42    &  1119.79 &   882.51    &  969.49  \\ 
%     GAT-1 & 3716.29   &  1761.71 &  8221.17   &   6604.11 & 4612.36 &  2766.27 & 2526.51 &  2115.72     &   2341.94 &  2202.73 & 2321.38 &  1863.86 \\
%     GAT-3 &  4674.74  &  2633.27 &  16792.28   &  13896.02 &  6369.62 & 4704.58 &  2547.01 &  2945.06  &  2325.61 &  3138.60  &   2312.89 &  2352.84 \\
% % [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table-gnn} % is used to refer this table in the text
% \end{table*}




% \begin{table}[ht]
% \caption{Accuracy evaluation results for Cora dataset for 200 iterations.} % title of Table
% \centering % used for centering table
% \begin{tabular}{l c c c} % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines
% Method & DGL  & {\graphpy} \\ [0.7ex] % inserts table
% %heading
% \hline % inserts single horizontal line
% GCN & 79.91\%  &  77.62\% \\ % inserting body of the table
% GAT (single-head) & 74.65\% & 69.94\%  \\
% GAT (multi-heads) & 78.10\%  & 73.34\%  \\
% [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table-accuracy} % is used to refer this table in the text
% \end{table}

% \begin{table}[ht]
% \caption{Accuracy evaluation results for PubMed dataset for 200 iterations.} % title of Table
% \centering % used for centering table
% \begin{tabular}{l c c c} % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines
% Method & DGL  & {\graphpy} \\ [0.7ex] % inserts table
% %heading
% \hline % inserts single horizontal line
% GCN & 77.30\%  &  75.80\% \\ % inserting body of the table
% GAT (single-head) & 76.00\% & 75.18\%  \\
% GAT (multi-heads) & 75.50\%  & 76.02\%  \\
% [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table-accuracy-pubmed} % is used to refer this table in the text
% \end{table}

% \begin{table}[ht]
% \caption{Accuracy evaluation results for Citeseer dataset for 200 iterations.} % title of Table
% \centering % used for centering table
% \begin{tabular}{l c c c} % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines
% Method & DGL  & {\graphpy} \\ [0.7ex] % inserts table
% %heading
% \hline % inserts single horizontal line
% GCN & 65.00\%  &  60.16\% \\ % inserting body of the table
% GAT (single-head) & 59.70\% & 59.44\%  \\
% GAT (multi-heads) & 65.10\%  & 64.92\%  \\
% [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table-accuracy-citeseer} % is used to refer this table in the text
% \end{table}


%\subsection{GNN Training Performance} \label{sec.exp-gnn.time}
% To evaluate the average graph DL training time,  We compare our work {\graphpy} with DGL but not NetworkX as it is not designed to support DL operations.   
%We train the GCN, GIN, and GAT on datasets for 200 epochs and repeat the experiments 10 times, and average the result. 
%The average GNN training time is converted to milliseconds.
%We classify the results into smaller datasets and larger datasets. A smaller dataset is the one where kernel time is in sub-milliseconds and does not play any role in total training time.


\begin{figure}[b]
  \includegraphics[scale= 0.58]{exp/gpu_small_perf.pdf}
   \vspace{-24pt}
  \caption{\small GNN training speedup on top of DGL for smaller datasets.}
  \label{exp-gnn-gpu}
%\vspace{-8pt}
\end{figure}


\subsection{Smaller Dataset: Impact of Framework Overhead} \label{sec.exp.overhead}

Fig. \ref{exp-gnn-gpu} shows the graph DL training time evaluation result for GPU using 200 epochs. 
%\noindent \textbf{CPU.} 
{\graphpy} achieves 1.54$\times$ and 1.35$\times$ average speedup over DGL and PyG respectively for the three datasets. It would be tempting to attribute this performance advancement to GNN-specific kernel design. However, less framework overhead is the root cause.

%\noindent \textbf{Methodology.} 
We used the methodology discussed in \cref{sec.obs} to measure the overhead, but we categorize it as the start-up cost (first epoch) and runtime cost (rest 199 epochs).
Table~\ref{table-exp-overhead} shows them for Pubmed and Reddit. Reddit dataset is included to show that the overhead time is much less than the total training time to \textit{prove that the proposed methodology is valid}.
%and \red{\textit{represents a new methodology to find the framework overhead.}}
%In comparsion to other methodologies, that is used by prior 
%and hence the overhead plays an insignificant role in larger datasets. 

%and is plotted in Fig.~\ref{exp-overhead-time} for GCN. Clearly, the training time is the same as the framework overhead.  


% \begin{figure}[htb]
%   \includegraphics[scale= 0.47]{exp/overhead.pdf}
%   \vspace{-24pt}
%   \caption{\small GCN training on Smaller Dataset: Framework overhead decides the total training (in Seconds for 200 epochs). %Clearly, system optimization works should not evaluate exclusively on smaller datasets to conclude performance gain.
%   }
%   \label{exp-overhead-time}
%  %\vspace{-6pt}
% \end{figure}



%E.g. in DGL, the total kernel time (for 200 epochs) is 0.18 seconds, while difference between
%This is evident from measurements on Reddit.
%Measuring only the overhead directly is not possible, as we do not know the source of overhead yet. 




\begin{table}[t]
\footnotesize
%\vspace{-6pt}
\caption{\small Framework overhead in Seconds for GCN(Lower is better) on Pubmed. Overhead on Reddit is also shown for comparison.} % title of Table
\vspace{-6pt}
\centering % used for centering table
\begin{tabular}{|l| ccc|c|c|} 
    \hline\hline 
    Graph & Startup & Runtime & Total & Training\\% & gSpMM \\
    Dataset & Cost & Cost & Overhead & Time \\%& Time \\ % inserts table
    %heading
    \hline % inserts single horizontal line
    DGL & 0.786 & 0.684 & 1.470 &1.480 \\%&  0.000228\\
    PyG & 0.567 & 0.684 & 1.251 & 1.261 \\%& \td\\
    {\graphpy} & 0.646 & 0.272 & 0.918 & 0.929 \\%& 0.000382\\
    \hline
    GNNAdvisor & 0.470 & 0.244 & 0.714 & 0.722\\%& \td\\
    {\graphpy-no-bias} & 0.648 & 0.207 & 0.855 & 0.865 \\%& 0.000382\\
    \hline
    Reddit-DGL & 0.851 &  0.551 & 1.402 &  25.839 \\%& 0.031 \\ 
    %Reddit-{\graphpy} & 0.662 & 0.371 & 1.033 & 11.191 \\%& 0.017\\ 
    % % & 76.47 &  76.52 & & \\
    \hline %inserts single line
\end{tabular}
%\vspace{-6pt}
\label{table-exp-overhead} % is used to refer this table in the text
\end{table}


The overhead is significant for Pubmed, a smaller dataset.
Kindly note that the training loop, GNN module, and the model layer (written in Python) are almost identical in DGL and {\graphpy}. The divergence starts from the mechanism to call system APIs, and the CPU code before invoking the CUDA kernel.
The minimalist approach of {\graphpy}, where we can directly invoke the custom system API with a DLPack capsule, and invoke the right CUDA kernel directly has less overhead. In comparison, DGL first converts the DL framework tensor to DGL's tensor, then uses a generic interface for gSpMM, followed by some heavyweight CPU code including GPU memory allocation to bridge the requirement mismatch.  
%Hence, it is the huge start-up cost, and run-time overhead that is responsible for DGL's poor performance
%, as DGL's GCN kernel (0.228 milliseconds) is faster than the {\graphpy's} GCN kernel (0.382 milliseconds) for Pubmed. 
%For Reddit, {\graphpy's} GCN kernel (17 milliseconds) is faster than DGL (31 milliseconds), which improves our performance, while the contribution from overhead is very less. 

\noindent
\textbf{Alternate Approach to Minimize Framework Overhead.} 
GNNAdvisor does not use bias in its GCN, so we compare it with a version of {\graphpy} where bias was commented, and ignored the wrong kernel order in GNNAdvisor.
This comparison presents a new insight as its layer implementation is in C++. We can clearly see that moving code from Python to C++ leads to less start-up cost because PyTorch spends hardly any time preparing the computation graph, however, that does not reduce the run-time overhead. 
%But the absence of an elaborate computation graph implies more C++ code execution in the backward computation that leads to poor runtime cost for GNNAdvisor. 
Though it is slightly faster than {\graphpy} for smaller data sets due to reduced start-up cost, we would not recommend writing layers in C++. 
%based on our experience as it plays no role for larger data sets. 
%\red{Why we do not recommend people to move code from Python to C++?\td
1) Moving code from Python to C++ cannot improve performance in large datasets. 
2) GNNAdvisor did not follow the correct approach to writing layers. It merges layer kernels together into one complex operator in C++. However, this fused operator forces us to manually invoke the backward computation of every kernel, such as the linear layer. 
3) Our experience shows that writing model layers in C++ correctly is complex and instructions are not clear. When we used the smart pointer approach and wrote layers in C++ it took us almost 6 months to implement GCN (see appendix). 
%Both approaches could be avoided easily by writing layers in Python.

% For GCN, GNNAdvisor is only 16.5\% faster (use {\graphpy} as baseline) compared to the reported 2.4$\times$ (approximate) speedup (use DGL as baseline) for Pubmed. 
% \textit{This speedup is still because of low start-up cost as listed in Table~\ref{table-exp-overhead}, confirming our earlier observation}.


%This implies that for smaller datasets, the overhead is significant which determines the training time and not the kernel execution time; while for larger datasets, kernel time plays deciding role.
{\textit{An overhead of around a second is not a major issue, but showing performance gains based on smaller datasets alone is not acceptable either. Because of this finding, we do not focus on small datasets and use large datasets for evaluation.}}

%Profiling DGL did not give any specific hints on from where the overhead might be coming.
%For PyG, the startup cost is lower, but the run-time cost is similar to DGL.


%Rather, DGL is impacted by framework overhead. and minor changes in the graph storage, as both its captive graph storage always generates directed graph with edge IDs (asking user to provide edges in both directions). However for GCN and GIN kernels, undirected graph with no edge ID is sufficient. Hence, DGL pollutes hardware caches with more graph data, while {\graphpy} just relies on undirected graph without egde IDs. 
%To confirm this observation, we re-run {\graphpy} using direction and edge ID graph storage, and observe performance drop by \td \% for GCN. 
%Clearly, support of {Dtype} in {\graphpy}, and outsourcing graph preparation to {\graphpy-DE} makes the Kernel interfaces free from any captive nature of graph, or any other interface limitations so that the Kernel can get better performance.

%could be many things, as they are built over different systems, where DGL performs its own memory management for generating output tensors, while {\graphpy} leaves tensor memory management to DL framework. However, our proposed optimizations of kernel fusing in GCN, plays an important role.  

%For GAT, edge IDs are stored along with neighbor information in {\graphpy}, while DGL separates them into two arrays. Also, DGL performs gSDDMM using COO format, while we use CSC format in CPU. Hence, {\graphpy} brings less data to hardware caches than DGL.
%that gains due to edge ID reordering.




\subsection{Large Dataset:  Requirement Mismatch} \label{sec.exp-gnn.time}

Requirement mismatch removal has memory and performance implications both as discussed next. 
%We train various models for 200 epochs in an end-to-end setup.
%We discuss them next. For non-labeled datasets, we generate random features of length 150, and set the prediction class as 7 in all the end-to-end training.

%\noindent \textbf{}
\subsubsection{Memory Consumption.}
%Since we were not able to run a few GNN models on DGL due to excessive memory usage, we show the memory consumption in 
%Interestingly, PyG could not train any GNN model on the Reddit and  datasets. 
%GNNAdvisor also failed to run GCN on Reddit. DGL fails to run on GAT-3 because of \textit{out of memory} condition(OOM) that is listed in Table~\ref{table-exp-memory}. %Therefore, Fig.~\ref{exp-accuracy} does not plot results on Reddit dataset.  
Fig.~\ref{exp-mem} shows that {\graphpy} reduces memory consumption on average by 6.92$\times$ on GCN, 3.4$\times$ on GIN, and 1.96$\times$ on GAT-1 models in comparison to DGL.
E.g., on Reddit (G10), {\graphpy} (DGL) consumes only 2.1GB (23.2GB), 4.0GB (23.7GB), 13.3GB (30.3GB), and 30.9GB(OOM) on GCN, GIN, GAT-1, and GAT-3 respectively, 
%while DGL  consumes 23.2GB, 23.7GB, 32.3GB, and out of memory. 
%Hence, {\graphpy} achieves over 10$\times$ memory saving on GCN for Reddit.
%{\graphpy} is even able to run GAT-3 on the Reddit dataset consuming around 32GB of memory, while DGL cannot. 
The requirement mismatch in the case of DGL's reliance on CuSparse gSpMMve API requires allocating memory for the dummy edge-level tensor in GCN and GIN, and for intermediate results in GAT. 
(1) Results reveal that GCN and GIN memory consumption is also proportional to $|E|$ in DGL due to the mismatch, while {\graphpy} closely follows $|V|$.
(2) For GAT-3, DGL has its own implementation as CuSparse has no support for the vector edge feature. However, it consumes more memory and runs out of memory on Reddit. 
This is an important  result indicating that its monolithic backend may have other avenues of additional memory consumption.
We exclude results for G3--G8 in Fig.~\ref{exp-mem} as the focus is to study the out-of-memory behavior, though we observe a similar pattern for those datasets.

%It is unfortunate that we could not run the DGL integrated system of FeatGraph and Ge-SpMM to observe if this memory overhead is due to their kernel or the framework.

%specifically, the memory needed for additional transpose, eShuffle (for GAT only), and dummy edge-level tensor (for GCN/GIN only). 
%This makes DGL consumes over 10$\times$ memory than {\graphpy} while training GCN on the Reddit dataset which has only slightly more than 230 thousand vertices.  

%Most of the kernels of the DGL are written by it as CuSparse does not support vector edge features or gSpMMeid. 

\begin{figure}[t]
  \includegraphics[scale= 0.48]{exp/exp-memory.pdf}
  \vspace{-12pt}
  \caption{\small Memory consumption comparison on various models. OOM refers to an out-of-memory condition. (Lower is better).}
  \label{exp-mem}
% \vspace{-12pt}
\end{figure}


%It achieves over 90\% accuracy on GCN and GAT. 
%hence we may not be able to run DGL on entry and mid-level GPUs that have less memory, such as Nvidia GTX 1080 Ti, Titan V. Because of such issue many prior works used smaller datasets only.

PyG ran out of memory on Reddit and OGB-Product even on GCN, so we did not plot it.
PyG scatters the vertex features to edges generating |E|*feature-dimension memory requirement, before computing the vertex-level tensor in its gSpMM. This scatter phase consumes a huge amount of memory for larger datasets, which is the reason for OOM and has been identified by prior works~\cite{chen2020fusegnn,huang2021understanding}.
\textit{Another important takeaway is that {\graphpy} can train GCN on a billion-edge graph (G13: Kron-25), a first on a GPU}, consuming 29.8 GB only, while DGL cannot even run a graph with around half a billion-edge (G12: UK-2002) when using the same feature-count (150) and prediction classes (7).


%Results indicate that {\graphpy} allows the training of various GNN models on larger datasets that cannot be trained by current systems on a single GPU. Hence {\graphpy} saves memory consumption and computing resources. 

%\textit{These results (Fig.~\ref{exp-accuracy} and \ref{exp-mem}) clearly identify the need to evaluate the accuracy and memory consumption in a training loop, before we should report any performance gain.} 
%as adding bias in GNNAdvisor will reduce its performance gain reported in its paper.
%It should be noted that the CuSparse feature matrix argument is expected in column-major for SpMM, while the supplied feature tensor from PyTorch is row-major. Therefore DGL has to plug this gap, which it does through two transposes on tensors, as mentioned in the DGL codebase. For GAT, cuSparse does not support access of edge-level tensors through edge ID, so DGL has to shuffle such tensors first before sending it to cuSparse. The additional code in DGL allocates and consumes additional memory.  



% \begin{table}[t]
% \footnotesize
% %\vspace{-6pt}
% \caption{\small Memory Consumption (in MB). Lower is better.} % title of Table
% \vspace{-6pt}
% \centering % used for centering table
% \begin{tabular}{|l| r|r |r|r|r|r|} 
%     \hline\hline 
%     Graph  & \multicolumn{3}{|c|}{GCN} & \multicolumn{3}{c|}{GAT-1}\\ [0.5ex] % inserts table
%     %heading
%     \hline 
%     Dataset & DGL & PyG & {\graphpy} & DGL & PyG & {\graphpy}\\
%     \cline{2-7}
% %    Cora & 1,719 & 1,349 & 1,381 & 1,719 &1,375& 1,383\\ 
% %    PubMed & 1,767 & 1,395& 1,423 &1809& 1,503& 1,429\\
% %    Citeseer& 1,697&1,381&  1,415 & 1,759 &1,409& 1,417\\ 
%     Reddit & 23,237&OOM& 2153 & 30,395 & OOM & 13,345\\
%     OGB & 24,681&OOM& 4,901 & 36,139 & OOM & 12,647 \\
%     \hline
%     & \multicolumn{3}{|c|}{GIN} & \multicolumn{3}{c|}{GAT-1}\\ [0.5ex] 
%     % & 76.47 &  76.52 & & \\
%     \hline %inserts single line
% \end{tabular}
% \vspace{-6pt}
% \label{table-exp-memory} % is used to refer this table in the text
% \end{table}

%Fig.~\ref{exp-gnn-gpu} shows speedup on end-to-end GNN training performance using DGL as the base. 

\begin{figure}[t]
  \includegraphics[scale= 0.49]{exp/gpu_large_perf.pdf}
  \vspace{-24pt}
  \caption{\small {\graphpy} speedup over DGL for GNN training time (200 epochs) in GPU for larger datasets. A speedup of 4 means that DGL has OOM not {\graphpy}. (higher is better)}
  \label{exp-gnn-gpu-large}
%\vspace{-8pt}
\end{figure}

\subsubsection{End-to-End Performance.}
Fig.~\ref{exp-gnn-gpu-large} shows that {\graphpy} performs much better than DGL for all datasets while training various GNN models. % for 200 epochs.
For Reddit, {\graphpy} achieves around 2.30$\times$ speedup for GCN, and 1.36$\times$ for both GIN and GAT-1 over DGL, while for GAT-3 DGL resulted in OOM. 
The performance improvement is purely based on designing kernels as per GNN use cases.
Specifically, for GAT, the newly designed gSpMMveid kernel removes the  need for a separate eShuffle. 
For GCN and GIN, 
DGL's gSpMMv uses CuSparse's gSpMMve API which forces DGL to use a dummy edge-level tensor as the latter does not provide the gSpMMv. %the transpose of vertex-level tensors. 
{\graphpy} directly implements gSpMMv, and fuses it with normalization by the degree in the right order in the forward direction.
These kernels alone improve the training performance despite {\graphpy} having no advantage over other kernels such as linear operation, ReLU, etc.





\subsection{{\graphpy-Kernel} Performance}
We use kernel run-time to understand the impact of GNN-specific kernels alone and also focus on other systems which we could not run end-to-end (\cref{sec.obs}, \cref{sec.dgl}). We use Reddit and OGB-Product-- two widely used large labeled datasets. 
%This setting explicitly avoids the framework overhead for others (except DGL), e.g., GE-SpMM will not show the memory and performance overhead due to normalization by degree being performed by DGL.  {\graphpy} has the usual overhead to {\graphpy}. 

\noindent \textbf{gpk$\_$gSpMMveid.}
 Fig.~\ref{exp-gpu-gspmmve} plots the time taken to implement the gSpMMveid kernel, which is a combination of gSMMve (implemented by prior works) and eShuffle (implemented by us to estimate the cost). We plot for feature lengths 16 and 32 both as GE-SpMM has not optimized for feature-length 16. GNNAdvisor is not plotted as it has not been implemented.
(a) The results clearly show the eShuffle cost introduced by DGL over CuSparse is significant, and we captured this overhead really well. 
(b) The gSpMMveid is natively implemented by only {\graphpy}  and outperforms all the prior works. 
(c) Even a workload-balanced kernel design by Huang et al is slower than {\graphpy} due to the requirement mismatch overhead that cost almost equal to gSpMMve.

\begin{figure}[b]
  \includegraphics[scale= 0.60]{exp/exp-spmmve.pdf}
  \vspace{-24pt}
  \caption{\small gSpMMve kernel time comparison for 16 and 32 feature length. GNNAdvisor does not implement it. (Lower is better)}
  \label{exp-gpu-gspmmve}
%\vspace{-8pt}
\end{figure}



%including the removal of transpose.

% if the reduce operation is \textit{sum}, while for \textit{min} reduce operation it uses its own kernel implementation. 
% In {\graphpy}, we have written all the versions ourselves but did not do any specific optimization.
% For gSDDMM, both the systems uses edge-level parallelism on GPUs using COO format. 
% Since, {\graphpy-Kernel} is not optimized specifically, the speedup over DGL was not expected. 

\noindent \textbf{gpk$\_$gSpMMv.}
A similar analysis for gSpMMv is presented in Fig.~\ref{exp-gpu-gspmmv}. It should be noted that many works have focused on GCN, and have even good workload balancing. 
Despite this, {\graphpy} performed better than DGL, CuSparse, and GNNAdvisor. It is better than GE-SpMM which is the only other system that natively but silently offers gSpMMv, and performed equivalent to Huang et al which is a workload balanced solution. 
We analyze the results next.

(a) DGL still has lower performance because it directly uses gSpMMve of CuSparse. It introduces some overhead on top of it as it allocates memory workspace in the critical path that the new gSpMMve API of CuSparse needs as input. 
(b) GNNAdvisor has a poor gSpMMv implementation despite using neighbor grouping to balance the workload. That is because it uses shared memory for caching (introduced by GE-SpMM) but performs an additional write to it and uses an additional memory barrier during initialization (not needed). Rather it mostly performs slower than CuSparse and GE-SpMM. 
(c) Neighbor grouping was simultaneously proposed by Huang et al for gSpMMve which is used by their forward-only GCN (gSpMMv is not implemented). It performs better than others but cannot outperform {\graphpy} despite the latter having a workload imbalance.
%This is due to its focus on evaluating smaller datasets only, where double write to GPU shared memory 
We believe it could have performed better if gSpMMv was natively implemented and hence is the victim of requirement mismatch.
%Kindly note that neighbor grouping requires a graph pre-processing whose cost is not shown.


\begin{figure}[t]
  \includegraphics[scale= 0.60]{exp/exp-spmmv.pdf}
 \vspace{-6pt}
  \caption{\small gSpMMv GPU kernel time for larger datasets.}
  \label{exp-gpu-gspmmv}
%\vspace{-8pt}
\end{figure}


Measuring individual kernel performance, however, does not show some other advantages. E.g., {\graphpy} can perform in-place normalization by degrees that do not require additional memory compared to all prior works except GNNAdvisor which wrongly performs this step. E.g., DGL uses Pytorch API in Python to do out-of-place normalization, resulting in additional memory consumption. 

\textit{The results in this sub-section clearly prove our initial observation:} 
(a) even a good technique (neighbor grouping in GNNAdvisor) when not evaluated on larger datasets can cause performance regression compared to the same system against which it claimed to perform better;
(b) kernels implemented specifically for GNN use cases provide better performance compared to the optimized systems that follow earlier conventions of generality. 


% \begin{table}[h]
% \small
% %\vspace{-6pt}
% \caption{\small Kernel Time (in Millisecond) with vertex-level feature length = 16.\textbf{* indicates that CuSparse gSpMMv involves a dummy edge-level tensor for the computation.}} % title of Table
% \vspace{-6pt}
% \centering % used for centering table
% \begin{tabular}{|l| r|r |r|r|} 
%     \hline\hline 
%     GNN  & \multicolumn{2}{|c|}{gSpMMv(GCN)} & \multicolumn{2}{c|}{gSpMMve(GAT)}\\ [0.5ex] % inserts table
%     %heading
%     \cline{2-5}
%     Kernel & Reddit & Ogb-Product & Reddit & Ogb-product\\
%     \hline % inserts a single horizontal line
%    GNNAdvisor & 45.18 & 34.47 & N.A. &N.A.\\
%    GE-SpMM & 22.18 & 18.30 & 42.04 & 25.12 \\
%     DGL & 29.29 & 26.42 &37.04& 36.22\\
%     % DGL & & & 39.19 & 32.30\\ Correct one
%     % DGL Norm & 0.682 &0.647 &  & \\ Correct one
%     {\graphpy} & 11.045 & 9.26 & 30.52 & 19.31 \\
%     \hline
%     CuSparse& 14.07$^*$ & 22.04$^*$ & 14.07 &22.04\\
%     eShuffle time & N.A. & N.A. &13.31 & 7.31\\
% %    Huang et al & N.A. & N.A. & 12.34& 10.35\\
%     % & 76.47 &  76.52 & & \\
%     % norm time & 0.33 & 0.57 & 0 & 0
%  %Correct one
% % GraphPY fuse GCN & 11.096 & 9.321 & 0 & 0$
% %    \hline %inserts single line
%     \hline
% \end{tabular}
% %\vspace{-6pt}
% \label{table-kernel-time} % is used to refer this table in the text
% \end{table}








%To confirm this result, we also evaluated GCN on a larger dataset of reddit. {\graphpy} achieved 2.3$\times$ speedup compared to DGL. 
% {\graphpy} is better than PyG as we expect CSR/CSC to perform better than COO format of PyG for kernel implementation due to its interface limitations (\cref{sec.science.challenges}). Unfortunately, none of the results except Reddit can be explained due to just better kernel performance, as we 
% explain next after measuring memory overhead. 


%\noindent \textbf{Lower Framework Overhead.}
%To find the exact reason behind the speedup, and to better understand the performance comparison on smaller datasets, we measure the gSpMM kernel time for GCN on two datasets of Pubmed and Reddit in the GPU, along with framework overhead. 
%Measuring framework overhead is not simple, hence we measure the time taken by CPU, i.e., the time taken by everything except the time spent in the GPU kernel. 




%Profiling DGL did not give any specific hints on from where the overhead might be coming.
%For PyG, the startup cost is lower, but the run-time cost is similar to DGL.


%Rather, DGL is impacted by framework overhead. and minor changes in the graph storage, as both its captive graph storage always generates directed graph with edge IDs (asking user to provide edges in both directions). However for GCN and GIN kernels, undirected graph with no edge ID is sufficient. Hence, DGL pollutes hardware caches with more graph data, while {\graphpy} just relies on undirected graph without egde IDs. 
%To confirm this observation, we re-run {\graphpy} using direction and edge ID graph storage, and observe performance drop by \td \% for GCN. 
%Clearly, support of {Dtype} in {\graphpy}, and outsourcing graph preparation to {\graphpy-DE} makes the Kernel interfaces free from any captive nature of graph, or any other interface limitations so that the Kernel can get better performance.

%could be many things, as they are built over different systems, where DGL performs its own memory management for generating output tensors, while {\graphpy} leaves tensor memory management to DL framework. However, our proposed optimizations of kernel fusing in GCN, plays an important role.  

%For GAT, edge IDs are stored along with neighbor information in {\graphpy}, while DGL separates them into two arrays. Also, DGL performs gSDDMM using COO format, while we use CSC format in CPU. Hence, {\graphpy} brings less data to hardware caches than DGL.
%that gains due to edge ID reordering.



% \noindent \textbf{GPU.} 
% {\graphpy} achieves 1.68$\times$ and 1.39$\times$ average speedup over DGL and PyG respectively. 
% % It should be noted that our implementation is for proof of concept only, with two optimizations. However, 
% For PyG, it was again the usage of COO that causes slowdown. For DGL, apart from graph format differences, the performance improvement in {\graphpy} is also because of better parallelism using GPU warp that is made up of 32 single instruction multiple threads (SIMT). We think that using warp for processing one N(v) instead of single thread (used by DGL) has become a mainstream strategy~\cite{liu2015enterprise}, as GPU is known for its SIMT capability, and should be part of implementation. Since, DGL does not use it, it performs even slower than PyG by 20\%.
% %Apart from that, the two optimizations (\cref{sec.optimization}) improve the performance further.
% % So, it is clear that there are event better opportunities to optimize the performance, and hence {\graphpy} will reduce the effort in prototyping new solutions. 

% \noindent \textbf{Actual Advancement by Other Works.}
% %As we outlined earlier, DGL have already identified the framework overhead, though its impact was not very clear.
% DGL framework overhead is interesting because many works that have not used DGL for their kernel prototype have used it as baseline to show their impressive performance gain, mostly focusing on smaller dataset only.
% %and hence a new baseline will put those result in perspective as we explore here, and needed for better progress of research. 
% So, we revisited other works to benchmark them again using {\graphpy} as a new baseline. 


%while {\graphpy} is better for run-time overhead.  %as better kernel does not play any role.
%They have not implemented GAT. 
%However, since DGL kernel is faster than our reference kernel, we expect the actual gain to be even smaller.

%GE-SpMM~\cite{gespmmsc2020} has not implemented the training loop.
%Similarly, 
%We were unable to run FeatGraph as its integration to DGL seems still in progress, as we tried many DGL github branches as suggested by their authors. However, they emphasized that FeatGraph's performance will be similar to DGL. Huang et al~\cite{huang2021understanding} have not implemented the training loop, while they have not used the edge ID indirection which is needed for GAT. Implementation of a training loop, and measuring accuracy would have revealed the issue, and hence the work could have been evaluated more objectively. We believe {\graphpy} is the right platform for such tasks. P3~\cite{p3gandhi2021} and NeuGraph~\cite{neugraph19atc} are not open-sourced. Request to open-source P3 did not elicit any response from its author.



%while they have done many optimization in the data science part, by writing

%though we are still not sure if this comparison is correct due to issues with accuracy.  
%Secondly, it crashes for slightly larger dataset as it uses more resources for computation. 

% \begin{figure}[h]
%   \includegraphics[scale= 0.44]{exp/featgraph_crop.pdf}
%   \vspace{-16pt}
%   \caption{GNN training time comparison in GPU between featgraph and {\graphpy}.}
%   \label{exp-featgraph}
% % \vspace{-12pt}
% \end{figure}






% \noindent \textbf{Impact of Edge ID reordering.} 
% To demonstrate that {\graphpy} is capable of supporting the optimization, we implemented the edge ID reordering, where CSC format will be allocated sequential edge IDs. Thus, except CSR data access, edges are always sequential including COO formats. 
% Fig.~\ref{exp-order} shows that the gSDDMM GAS kernel improves by 1.74$\times$ to 7.11$\times$, while gSpMMW kernel improves by only 1.05$\times$ to 1.43$\times$. The better result for gSDDMM is because it writes the tensor at edge-level, and hence random write is converted to sequential version, which imporves even further when graph size is larger, such as Patent citation. While gSpMMW only reads the edge-level tensors, and thus has lower impact on performance.
% When testing end to end, these improvements translated to around 10\% improvement in GAT. \td.

% \begin{figure}[h]
%   \includegraphics[scale= 0.64]{exp/reorder-crop.pdf}
%   \vspace{-6pt}
%   \caption{Impact of Edge ID reordering on GAS kernels (GPU).}
%   \label{exp-order}
%  \vspace{-12pt}
% \end{figure}



% \begin{table*}[t]
% \caption{Graph DL training time (in \textit{Milliseconds}) for Cora dataset based on different graph DL models for 200 iterations. } % title of Table
% \centering % used for centering table
% % \setlength{\tabcolsep}{0.4mm}
% \begin{tabular}{l cccccc} % centered columns (4 columns)
%     \hline\hline %inserts double horizontal lines
%           & \multicolumn{2}{c}{Cora} & \multicolumn{2}{c}{Pubmed} & \multicolumn{2}{c}{Citeseer}\\
%     \hline
%     Method & DGL  & {GP} & DGL  & {GP} & DGL  & {GP} \\ 
%     \hline % inserts single horizontal line
%     GCN   &  900.00    &  1061.39  &   883.42    &  1119.79 &   882.51    &  969.49  \\ 
%     GAT-1 & 2526.51 &  2115.72     &   2341.94 &  2202.73 & 2321.38 &  1863.86 \\
%     GAT-3 &  2547.01 &  2945.06  &  2325.61 &  3138.60  &   2312.89 &  2352.84 \\
% [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table-gnn-gpu} % is used to refer this table in the text
% \end{table*}


% \begin{table}[ht]
% \caption{Graph DL training time (in \textit{Milliseconds}) for PubMed dataset based on different graph DL models for 200 iterations. } % title of Table
% \centering % used for centering table
% % \setlength{\tabcolsep}{0.4mm}
% \begin{tabular}{l c r c c c} % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines
% Method & DGL  & {\graphpy} \\ [0.7ex] % inserts table
% %heading
% \hline % inserts single horizontal line
% GCN               &   4316.49  &  3060.49  \\ 
% GAT (single-head) &  8221.17   &   6604.11 \\
% GAT (multi-heads) &  16792.28   &  13896.02  \\
% [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table-gnn-pubmed} % is used to refer this table in the text
% \end{table}



% \begin{table}[ht]
% \caption{Graph DL training time (in \textit{Milliseconds}) for Citeseer dataset based on different graph DL models for 200 iterations. } % title of Table
% \centering % used for centering table
% % \setlength{\tabcolsep}{0.4mm}
% \begin{tabular}{l c r c c c} % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines
% Method & DGL  & {\graphpy} \\ [0.7ex] % inserts table
% %heading
% \hline % inserts single horizontal line
% GCN              &   3755.371    &  2108.99 \\ 
% GAT (single-head) &   4612.36 &  2766.27   \\
% GAT (multi-heads) &   6369.62 &  4704.58   \\
% [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table-gnn-citeseer} % is used to refer this table in the text
% \end{table}




% \begin{table}[ht]
% \caption{Graph DL training time on GPU (in \textit{Milliseconds}) for Cora dataset based on different graph DL models for 200 iterations. } % title of Table
% \centering % used for centering table
% % \setlength{\tabcolsep}{0.4mm}
% \begin{tabular}{l c r c c c} % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines
% Method & DGL  & {\graphpy} \\ [0.7ex] % inserts table
% %heading
% \hline % inserts single horizontal line
% GCN              &   900.00    &  1061.39 \\ 
% GAT (single-head) &   2526.51 &  2115.72   \\
% GAT (multi-heads) &   2547.01 &  2945.06   \\
% [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table-gnn-cora-gpu} % is used to refer this table in the text
% \end{table}

% \begin{table}[ht]
% \caption{Graph DL training time on GPU (in \textit{Milliseconds}) for PubMed dataset based on different graph DL models for 200 iterations. } % title of Table
% \centering % used for centering table
% % \setlength{\tabcolsep}{0.4mm}
% \begin{tabular}{l c r c c c} % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines
% Method & DGL  & {\graphpy} \\ [0.7ex] % inserts table
% %heading
% \hline % inserts single horizontal line
% GCN              &   883.42    &  1119.79 \\ 
% GAT (single-head) &   2341.94 &  2202.73   \\
% GAT (multi-heads) &   2325.61 &  3138.60   \\
% [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table-gnn-pubmed-gpu} % is used to refer this table in the text
% \end{table}



% \begin{table}[ht]
% \caption{Graph DL training time on GPU (in \textit{Milliseconds}) for Citeseer dataset based on different graph DL models for 200 iterations. } % title of Table
% \centering % used for centering table
% % \setlength{\tabcolsep}{0.4mm}
% \begin{tabular}{l c r c c c} % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines
% Method & DGL  & {\graphpy} \\ [0.7ex] % inserts table
% %heading
% \hline % inserts single horizontal line
% GCN              &   882.51    &  969.49 \\ 
% GAT (single-head) &   2321.38 &  1863.86   \\
% GAT (multi-heads) &   2312.89 &  2352.84   \\
% [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table-gnn-citeseer-gpu} % is used to refer this table in the text
% \end{table}

% \begin{table}[ht]
% \caption{Summary of evaluation results in terms of graph DL training time, for Cora dataset based on different graph DL modules. } % title of Table
% \centering % used for centering table
% \setlength{\tabcolsep}{0.4mm}
% \begin{tabular}{c c c c c c} % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines
% Method & DGL  & {\graphpy} & 4 threads & 8 threads\\ [0.7ex] % inserts table
% %heading
% \hline % inserts single horizontal line
% GCN & 4280.5194  &  3448.9654 &
% 2879.731 & 5736.927\\ % inserting body of the table
% GAT (single-head) & 6907.4924 & 3656.5170 & 3622.434
% & 12794.391\\
% GAT (multi-heads) & 8288.1600 & 4818.6416  & 4760.344
% & 6354.074\\
% [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table-gnn} % is used to refer this table in the text
% \end{table}

% \begin{figure}[b]
%   \includegraphics[scale= 0.76]{exp/gnn-cpu-crop.pdf}
%  \vspace{-6pt}
%   \caption{\small GNN training time comparison in CPU.}
%   \label{exp-gnn-cpu}
%  %\vspace{-12pt}
% \end{figure}

% \subsubsection{GNN Training on CPU}
% {\graphpy} achieves 1.30$\times$, and 2.29$\times$ speedup on average than DGL and PyG respectively for GCN  and GAT on smaller datasets on CPU as shown in Fig.~\ref{exp-gnn-cpu}. For Reddit, {\graphpy} achieves more than 2$\times$ speedup for GCN, and GIN. DGL shows OOM for GAT-1 and GAT-3, while {\graphpy} runs on GAT-1. PyG always shows OOM for Reddit on all the models. %Since, PyG relies on COO format, better performance of {\graphpy} was expected.
% DGL and {\graphpy} both use OpenMP for vertex-level parallelism in CPU.
% For DGL, the comparison simply enforces the observation, i.e., higher overhead is the main reason for better performance in smaller dataset.

% It should also be noted that preparing graph storage in this resource-constrained device is a bottleneck on Reddit, as it  could not finish preparation after more than an hour. Hence, systems that allow saving kernel graph and loading it back were able to avoid this bottleneck, as we can get the prepared graph from other machines. However, PyG does not have such APIs, and hence we had to write our own routine to save its graph storage, and load it back.
% Clearly, a system that takes care of such practical issues, such as {\graphpy} is very important for productivity.


% % \begin{table}[ht]
% % \caption{GraphPy topology analysis time (in \textit{Milliseconds}) for different datasets. } % title of Table
% % \centering % used for centering table
% % % \setlength{\tabcolsep}{0.4mm}
% % \begin{tabular}{l c r c c c} % centered columns (4 columns)
% % \hline\hline %inserts double horizontal lines
% % Dataset & BFS  & CC \\ [0.7ex] % inserts table
% % %heading
% % \hline % inserts single horizontal line
% % Cora &  0.2862  &  0.424  \\ 
% % PubMed &  10.706   &  22.640  \\
% % Amazon & 118.798  &  160.3046   \\
% % Patent Citation &  1102.865  & 3723.571  \\
% % [1ex] % [1ex] adds vertical space
% % \hline %inserts single line
% % \end{tabular}
% % \label{table-nxbfs} % is used to refer this table in the text
% % \end{table}

% \subsection{Graph Storage Preparation and Analytics}

% The Graph preparation performance is an important evaluation measure. 




==> tex/exp2.tex <==
\noindent \textbf{Traditional Graph Analytics}
In this test, we run two traditional graph analyses, namely breadth-first-search (BFS) and connected components (CC). We did not find a Python system with a high-performance back-end that can support arbitrary graph properties, so we choose NetworkX to show the advantage of choosing a high-performance back-end to perform the analysis. All the analyses are called from the Python environment.

Table~\ref{table-nx} shows the comparison. It is obvious that with a C++ backend, {\graphpy} will gain huge performance over pure Python-based NetworkX. 
%However, the aim of this experiment is slightly different: {\graphpy} is not just Python binding for an existing C++ back-end, but involves huge effort to
By enabling arbitrary edge properties using Numpy Dtype, {\graphpy} is as usable as the NetworkX or even more. So for users, NetworkX and {\graphpy} are the same but with better performance and scalability, which is purely achieved due to innovation in interface design.


\begin{table}[h]
\small
\caption{\small BFS and CC run-time of NetworkX and {\graphpy}. The run-time is in \textit{Milliseconds}. Speedup is shown inside the bracket.} % title of Table
\vspace{-6pt}
\centering % used for centering table
\setlength{\tabcolsep}{1mm}
\begin{tabular}{|l| r  r | r r| } % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
Dataset & \multicolumn{2}{|c|}{NetworkX} &  \multicolumn{2}{c|} {\graphpy}  \\ 
\cline{2-5}
 & BFS  & CC &  BFS  & CC \\
\hline % inserts single horizontal line
Cora & 13.05  &  0.86 & 0.29(45.00$\times$)  &  0.42(2.05$\times$)\\ 
PubMed &  449.49  & 42.72 & 10.71(41.97$\times$) &  22.64(1.89$\times$) \\
Amazon & 4152.54 &  594.10 & 118.80(34.95$\times$) &  160.30(3.71$\times$) \\
% Patent Citation &  OOM & OOM & 1102.86(-)  & 3723.57(-) \\
% [1ex] % [1ex] adds vertical space
\hline %inserts single line
\end{tabular}
\label{table-nx} % is used to refer this table in the text
\end{table}


%\vspace{2pt}
\noindent \textbf{Multi-Field Properties.}
%{\graphpy} provides users an option to store the edge properties when creating the graph. This option is important because some graph DL algorithms, such as GCN, do not need any edge property. Therefore, there is no need to create a graph with edge property in this case. DGL always creates edge IDs, while NetworkX has an option for specifying the optional weight. However, 
NetworkX allows specification on only a single weight field, while {\graphpy} allows specification of arbitrary multi-field custom weights using NumPy Dtype. 
% Though we limit our evaluation to simple graphs with option edge IDs. \td.
We use LANL dataset that has 9 properties for each edges to demonstrate this capability. Also, it does not have a numerical identifier in its raw data file. Thus, the vertex ID must be created from the string identifier. Hence, only {\graphpy} allows graph creation from this dataset. It achieves 2.247 Million Edges/Second of ingestion rate.

% \begin{table}[ht]
% \caption{Ingestion Rate (in \textit{Million Edges/Second}) for Kron-20 dataset. {\graphpy} allows parallel parsing of the dataset files, and leads to better performance.} % title of Table
% \centering % used for centering table
% \begin{tabular}{l r r } % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines
% System & Ingestion Rate & Speedup \\ [0.7ex] % inserts table heading
% \hline % inserts single horizontal line
% NetworkX               &    0.331 & 1.00$\times$ \\
% DGL                    &   0.869 &  2.62$\times$  \\
% {\graphpy} (1 thread ) &   3.767 & 11.37$\times$  \\
% {\graphpy} (2 threads) &   7.497 & 22.64 $\times$ \\
% {\graphpy} (4 threads) &   9.847 & 29.73$\times$  \\
% % {\graphpy} (8 threads) &   11.227 & 33.90 $\times$ \\
% [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table-parallel} % is used to refer this table in the text
% \end{table}


% \begin{table}[ht]
% \caption{\td result for parallel parsing Ingestion Rate (in \textit{just original time}) for  Patent-Citation. {\graphpy} allows parallel parsing of the dataset files, and leads to better performance.} % title of Table
% \centering % used for centering table
% \begin{tabular}{l r r } % centered columns (4 columns)
% \hline\hline %inserts double horizontal lines
% System & Ingestion Rate & Speedup \\ [0.7ex] % inserts table heading
% \hline % inserts single horizontal line
% NetworkX     &    0.318    & 1.00$\times$ \\
% DGL                    &  0.878   &  2.76 $\times$  \\
% {\graphpy} (1 thread ) &   3.777  & 11.89 $\times$  \\
% {\graphpy} (2 threads) &  6.684  &   21.04$\times$ \\
% {\graphpy} (4 threads) & 8.067   &  25.40$\times$  \\
% % {\graphpy} (8 threads) &   11.227 & 33.90 $\times$ \\
% [1ex] % [1ex] adds vertical space
% \hline %inserts single line
% \end{tabular}
% \label{table-parallel-patent} % is used to refer this table in the text
% \end{table}


% \vspace{1mm}
% \noindent \textbf{Parallel Parsing.}
% In the overall graph preparation pipeline, file parsing is the bottleneck as it is slow due to involvement of tokenization and other string operations. Hence, {\graphpy} provides parallel parsing when possible.  Users can choose the number of threads dedicated to this work.
% To test the system performance of this option, we use different number of threads and calculate the ingestion rate as the metric. 

% \begin{figure}[h]
%   \includegraphics[scale= 0.62]{exp/parallel-ingestion-crop.pdf}
%   \vspace{-6pt}
%   \caption{Ingestion Rate (in \textit{Million Edges/Second}) for Patent Citation dataset. {\graphpy} allows parallel parsing of the dataset files, and leads to better performance.}
%   \label{exp-parallel}
% %   \vspace{-12pt}
% \end{figure}

% We use Patent-Citation dataset that resides in multiple files. 
% We selected small size, because NetworkX runs out-of-memory for slightly bigger than this graph.
% Fig. \ref{exp-parallel} shows the average ingestion rate result, with different parsing thread count.  We find that as the number of threads increases, the system performance improves. The average graph creation time for {\graphpy} with 4 threads is over 25$\times$ and 9$\times$ faster than NetworkX and DGL respectively.
% % with 8 threads is 33$\times$ faster than NetworkX and 13$\times$ faster than DGL.
% The results around 4 threads are slightly sub-linear. This is because the system has only 4 physical cores. Hence, the graph creation starts saturating the resources as 4 threads are also dedicated to graph preparation from the buffered edges.


\subsection{Ingestion Rate of {\graphpy-SM}}
We use \textit{ingestion rate} as the metric to measure how many edges (from raw data files) can be processed per second to create the graph in CSR/CSC format. This ingestion rate is end-to-end, implying that it also includes the time of file parsing, which can only be done using a single thread if there is only one file. 
We evaluate the {\graphpy} against two existing graph systems DGL, and NetworkX, as both of them have Python interfaces.
Fig.~\ref{exp-ingestion} shows the ingestion rate in million edges/second for four datasets in a single socket 4-core Intel CPU up to 3.60GHz, and DRAM of 16GB loaded with Ubuntu 18.04.
% i7-4790 
We find that  {\graphpy} with edge ID is 6$\times$ and 11$\times$ faster than DGL and NetweorkX respectively. {\graphpy} is faster as it does the text file parsing in C++ which is faster than parsing in Python in DGL and NetworkX. 
%Second, the overlap of the parsing with CSR/CSC creation leads to a faster ingestion rate. 
If we create the graph without storing edge IDs, as in the GCN case, the ingestion rate can be improved by about 3\% but saves memory equivalent to $|E|$. It achieves over 4 million edges/second of ingestion rate on the Amazon dataset. 

%We did not create edge IDs in NetworkX as it is not a GNN framework.

 

\begin{figure}[h]
 \vspace{-6pt}
  \includegraphics[scale= 0.60]{exp/ingestion-crop.pdf}
%   \vspace{-6pt}
  \caption{\small Ingestion Rate: {\graphpy+} refers to creating the graph with edge IDs, while {\graphpy} refers without edge IDs. DGL always creates edge IDs. For NetworkX, we did not create edge IDs. OOM refers to out-of-memory condition.}
  \label{exp-ingestion}
  \vspace{-6pt}
\end{figure}


% \begin{table}[h]
% \caption{Ingestion Rate (in \textit{Million Edges/Second}): {\graphpy+} refers to creating the graph with edge IDs, while {\graphpy} refers to creating the graph without edge IDs. DGL always creates edge IDs. For NetworkX, we did not create edge IDs. OOM refers to out of memory condition that does not allow NetworkX to complete the ingestion on Patent Citation.} % title of Table
% \centering % used for centering table
% \setlength{\tabcolsep}{1.3mm}
% \begin{tabular}{l r r r r r} % centered columns (4 columns)
%     \hline
%     \hline %inserts double horizontal lines
%     System & Cora & PubMed & Amazon &    Patent-Citation & LANL \\ %[0.6ex] % inserts table
%     %  & & & & Citation \\
%     %heading
%     \hline % inserts single horizontal line
%     NetworkX & 0.201 & 0.364 & 0.400 & OOM & -\\
%     DGL & 0.611 & 0.833 & 0.787 & 0.752 & -\\
%     {\graphpy+} & 3.693 & 4.064 & 4.057 & 3.876 & NA\\
%     {\graphpy} & 3.850 & 4.167 & 4.252 & 4.081 & 2.247\\
    
%     % {\graphpy} (4THD) &   &   &   & 273.11 \\
    
%     % {\graphpy} (8THD) &   &   &    & 403.79 \\
% \hline %inserts single line
% \end{tabular}
% \label{table-ingestion} % is used to refer this table in the text
% \end{table}

\subsection{Sparse Tensor}
We choose the LeNet-300-100%~\cite{lecun1998gradient}, 
a fully connected neural network with 300 and 100 as the hidden layers. After weight pruning~\cite{han2016iclr}, all three fully connected layers become sparse with sparsity ratios of 4.46\%, 4.45\%, and 7.78\% respectively, i.e., keeping less than 10 connections for every 100 connections in the fully connected layer. We use the MNIST dataset which includes 60000 training and 10000 testing handwritten digits examples.  Each image in the dataset has 784 features, while the last fully connected layer produces predictions corresponding to 10 digits (0--9). 
%which are sent to the softmax layer. 
We set the retraining epochs as 100 and the batch sizes as 50. In other words, in each training epoch, the model will iterate 1200 times.
% and apply tensor-based operations for state-of-art model and the sparse layers computation for {\graphpy}.
{\graphpy} finishes the retraining in 16 minutes and 17 seconds, compared to 20 minutes and 1 second for the model that uses the bitmask matrix to achieve sparsity~\cite{{han2015learning,han2016iclr}}, achieving 17.5\% speedup, and huge memory saving.

%The reason for this speedup is the reduced computation which {\graphpy} could achieve due to its system-level support for sparsity. 
%On the other hand, prior works have used bit-mask matrix at the Python level for achieving sparsity where the underlying kernel still uses dense matrix for sparse layer computation. Again, 
The improvement is only 17.5\% as LeNet-300-100 is not a large neural network, as the bipartite graph has vertex counts in the range of 784 and 10. Hence, the sparse weight matrices are not as large as the graph data set we had above for the GNN case. However, it shows the possibility of the {\graphpy} framework for diverse research use cases.
%This affects the vertex-level parallelism for SpMM. With better technique, we expect better performance, as our implementation is only for reference. 

%Secondly, it is not just the performance improvement, but the huge memory saving that allows the compressed model to fully fit in the resource constrained devices. Hence, model inference can now be done fully in such devices.
% Also, the sparse layers computation procedures contain mostly random reads instead of sequential reads. 



==> tex/intro.tex <==
%{\color{red}


\section{Introduction} \label{sec.intro}
%Getting insights from data is very important, and hence 
Many applications have become data-driven today. 
%These applications are now popularly known as \textit{data science}. 
Within this ecosystem, a lot of real-world data can be stored as \textit{sparse matrices} or \textit{graphs}, such as social networks, chemistry, biology, recommendation system, scene description generation, knowledge bases, etc~\cite{fan2019graph, zitnik2018modeling, schlichtkrull2018modeling,hamilton2018embedding,ying2018graph,krahmer2003graph,perera2017recent,rgcn2018,wang2020entity}. 
%We call these data-driven use-cases as \textit{graph data science} 
To this end, many graph neural network (GNN) models, e.g., GCN~\cite{gcn17iclr}, graph attention network~\cite{gat18iclr}(GAT), GIN~\cite{xu2019powerful}, and others~\cite{gatedgraph2017,zhang18, graphsage17}, etc. have been proposed. 



% \noindent \textbf{Deep Learning on Sparse Data.}
% The neighborhood in graphs is different from other regular data, such as an image which has a fixed number of neighborhoods. To handle it, \textit{graph neural network}(GNN), has been proposed~\cite{gcn17iclr,gat18iclr,gatedgraph2017,gaan2018}. The GNN models can be trained efficiently if the graph can be used for storage. However, the current DL frameworks, such as PyTorch~\cite{pytorch2019} or TensorFlow~\cite{tensorflow2016} lack the same level of operational support for the sparse matrix that they have for dense matrix, as the original code-base of GCN~\cite{gcn17iclr}, GAT~\cite{gat18iclr} etc. have relied on bitmask at Python level to model sparsity on top of dense matrices that actually do not reduce computation or memory consumption. %because the underlying kernel still uses the dense matrix.


% traditional GNNs use the adjacency matrix to represent the graph structure and tensor operation to perform the forward and backward computations. 
% However, due to the sparsity, this will trigger the out-of-memory problem to represent a sizeable sparse graph and will cause computation inefficiency for tensor operation. 

% Since deep learning techniques can achieve excellent prediction, many graph neural network (GNN) works were proposed. Graph neural network (GNN) is about applying deep learning algorithms on the graph structure to do classification and prediction tasks, such as node classification, edge/link prediction, and graph classification. 
% The node classification denotes that given a graph structure and a subset of nodes with labels, the graph deep learning algorithm should predict the label of the remaining nodes. 
% In contrast, the link prediction tasks are predicting whether an edge exists between two given nodes or not, such as in auto-completing knowledge bases.


% \noindent \textbf{Deep Learning On Sparse Tensors.}
% DL Model compression techniques, such as weight pruning ~\cite{han2015learning,han2016iclr},  convert a dense model layer to a sparse layer by removing a lot of low-impact model parameters. 
% These techniques help to deploy large models on resource-constrained devices because the compressed models need less memory and CPU. Before deploying them, the compressed models undergo \textit{re-training}. This re-training step can be more efficient if the graph is used to model sparse layers. However, prior works~\cite{han2015learning} used bit-mask matrix in Python, and underlying dense matrix to achieve sparsity. Thereby, the \textit{re-training process did not really consume less memory}, hence we may not be able to use resource-constrained systems to do re-training, which are low on memory.

%These models also have inspired a number of systems optimizations~\cite{wang2021gnnadvisor,huang2021understanding,gespmmsc2020,fu2022tlpgnn,wu2021seastar,chen2020fusegnn}. However, our study finds that many of these design decisions indicate inadequate understanding because 

It should be noted that GNN is a special kind of deep learning (DL) model, and hence its training has a unique computation need. \textit{Forward computation} calls many \textit{kernels} (operations on data) from the input layer to the output layer to derive the prediction values which are compared with the ground truth to calculate the loss.
% and plug the loss into the backward procedure. 
Then, \textit{backward computation} uses the loss to derive the gradient by invoking kernels from the output layer to the input layer to update the model parameters.
%It uses the chain rule of gradient back-propagation to update the model parameter from it. 
Kindly note that the backward computation accesses results that are either accessed or produced in the forward computation and are called \textit{state tensors} (Fig.~\ref{fig-format}(a)). This computation paradigm differs from the prior forward-only related fields, e.g., graph analytics.
 
\noindent \textbf{Motivation: Missing End-to-End Focus.}
 Many prior GNN system optimization works~\cite{wang2021gnnadvisor,huang2021understanding,fu2022tlpgnn,wu2021seastar, chen2020fusegnn, kim2022analyzing,yan2020hygcn,liang2020engn,zhang2021boostgcn, geng2020awb} have established a clear trend of not measuring the GNN training accuracy, and many have only implemented forward computation.
%Many prior works either do not provide a full GNN model for training or do not measure training accuracy, 
Our analysis shows that it has led to significant practical issues, including questioning their proposed optimization techniques as presented next. %including the

Consider the case of the GAT model that calls 18 kernels in each layer~\cite{fu2022tlpgnn} in its forward computation. An obvious optimization technique is to fuse them into just one, as done by prior works~\cite{fu2022tlpgnn,huang2021understanding}. However, they have not implemented backward computation. The absence of end-to-end focus allowed them to avoid materializing the edge-level tensor($W_e$, a trainable GAT model parameter), and thereby not keeping edge ID(\cref{sec.background}) in their graph to access the same. 
Similarly, GNNAdvisor~\cite{wang2021gnnadvisor} does not measure the training accuracy. We point out that its codebase does not fuse the kernel correctly in the backward computation of GCN, and its model does not use bias, a vital model parameter, gaining performance unknowingly at the expense of accuracy. 

Hence all their demonstrated optimizations are not yet practical and require more investigation to implement backward computation to show training accuracy, which is likely to alter the very basic foundation of many proposed optimizations.
%Such additional steps would have enforced a brainstorming around the need for \textit{state tensors} and other GNN-specific requirements. 
%Fused kernels that avoid producing such tensors in the forward computation must implement backward computation to show that such fusion is feasible and justify them through training accuracy measurements.
%do not understand the system requirement from the GNN perspective. 
%Unfortunately,
%Hence, their optimization has no significance at this moment. We present various such observations in \cref{sec.obs}, however, the pressing question is whether such optimizations really advance the state-of-the-art. 
%and whether these mistakes are systematic.


%Further observations point us that many researchers do not understand GNN workflow exactly
%For example, 

%GE-SpMM~\cite{gespmmsc2020} forgets to consider the edge-level tensor when implementing the kernels. Section (\td) explains this analysis in detail. 



%\noindent \textbf{Systematic Lack}:
%We argue that these mistakes are systematic in nature. We present the following arguments to explain it. 

% No architecture papers \cite{yan2020hygcn,liang2020engn,zhang2021boostgcn}
%{\td  \cite{zhang2021boostgcn, geng2020awb, yan2020characterizing} only for inference and no accuracy}: Will see them later whether to include or not.
%\cite{baruah2021gnnmark} uses dgl and pyg, so not citing here.

%--------------
%(1) \textbf{No Training Accuracy Measurements and/or Missing Backward Computation.} 
% Indeed many prior works~\cite{wang2021gnnadvisor,huang2021understanding,fu2022tlpgnn,wu2021seastar, chen2020fusegnn, kim2022analyzing} do not measure the training accuracy either because they do not implement the backward computation or simply do not measure it despite having an end-to-end implementation.
% Hence, they may be totally unaware of the mistakes. 
% For example, GNNAdvisor~\cite{wang2021gnnadvisor}, and end-to-end GNN system does not fuse the normalization kernel correctly in the backward computation, while omitting the bias parameter from each GCN  layer (\cref{sec.obs}).
% %provides a more detailed analysis for this example). 
% Similarly, Huang et al~\cite{huang2021understanding}, and TLPGNN~\cite{fu2022tlpgnn} optimized the GAT model's forward computation without implementing its backward computation due to which they committed serious mistakes of wrongly fusing the kernels, including removal of edge-level tensors. Wrongly fused kernels can also alter the requirement significantly as they do not keep edge ID in their graph to access the attention score tensor in GAT(\cref{sec.obs}).


%Clearly, the research community has also not forced these works to measure training accuracy. 

%in form a natural boundary across which they cannot be blindly fused in the forward computation as they are needed in the backward 

% (2) \textbf{No Backward Computation.} Many prior works~\cite{huang2021understanding,fu2022tlpgnn}[\red{what about seastar and other works}] have not implemented a backward computation at all, and their optimizations focused on only the forward computation due to which they committed serious mistakes of wrongly fusing the kernels, including removal of edge-level tensors. We believe general awareness of GNN workflow and understanding is lacking, such as the need for \textit{state tensors}. Kernels producing such tensors form a natural boundary across which kernels cannot be fused in the forward computation. Wrongly fused kernels can also alter the requirement significantly. For example, Huang et al\cite{huang2021understanding}, and  TLPGNN\cite{fu2022tlpgnn} do not keep edge ID in their graph to access attention score tensor in GAT(\cref{sec.obs}). %(Section {\td} provides a more detailed analysis for this example). 
% %This mistake will be realized easily if these works implemented the backward kernel.
% % (3) One of the observations from such works is that they try to write GNN systems from scratch using current DL frameworks, such as PyTorch, TensorFlow, etc. 

% We explore the current methodology and find that it is very complex to write a GNN system from scratch because  passing the graph object and tensors to an independent module is very complex, and on top of this, users have to learn new build systems (Ninja), Python binding, memory management (due to delayed free of state tensors), etc. to integrate their code with a DL framework. We experienced the same issues ourselves when we tried to build a new baseline that resulted in exhaustion in just setting up the system. And, hence such exhaustion may force the researchers to not build an end-to-end system. 


%\noindent \textbf{End-to-End Systems Teaching.} 
%The academic community is also not encouraging end-to-end \textit{system} teaching. E.g., publicly listed assignments on DL/GNN {systems} courses offered by many universities~\cite{dlsCMU, cs15884CMU, cse599wWashington,cs231nStandford} \textit{focus only on the forward kernel} of an operator, and in Python without its integration in an end-to-end DL/GNN system. Hence, students cannot fully understand, appreciate, and gather complete requirements. Rather, industry partners have voiced concern about the availability of candidates with good systems and data science knowledge in an NSF workshop~\cite{storage2025NSF}.


%On the other hand, writing a GNN system from scratch gives the new system an immediate performance advantage, and we empirically show that prior work has been implicitly removed once other works develop a GNN system from scratch rather than integrating with DGL. can achieve performance improvement easily without any actual systems optimization. 

\begin{figure*}[t]
  \includegraphics[scale= 0.55]{result/edge_id_crop.pdf}
  \vspace{-12pt}
  \caption{\small (a) One GNN layer using GAS (gather-apply-scatter) to model the kernel: X and Y are intermediate features, and $W_e$ is the model parameter of the layer, e.g. attention score in case of GAT. X, Y, and $W_e$ tensors are \textit{state}, as they are used in backward. $A$ and $A^T$ are graph and its inverse respectively. (b) Sample graph (c and d) CSR and CSC representation along with edge ID indirection.}
  \label{fig-format}
 \vspace{-12pt}
\end{figure*}



\noindent \textbf{Contribution.}
This paper, called \textbf{\graphpy}, presents our observations that system optimizations based on a partial understanding of the GNN model may not lead to a practical system. {\graphpy} highlights the need for end-to-end model implementation to measure accuracy before showing the performance gain. 
To this end, {\graphpy} presents an ecosystem to perform it productively, and have following contributions. 

% focuses on two goals:
% (1) Writing a new GNN baseline by focusing on overhead reduction.
% (2) Explaining the critical pieces of the resultant architecture that has been extracted to develop an education and research tool to encourage the implementation of end-to-end DL/GNN systems. A detailed explanation of these contributions is below.


\noindent
\textbf{1. In-Depth Analysis (\cref{sec.obs} and \cref{sec.usecase}).}
We are the first ones to analyze existing GNN system optimizations, the current practices to integrate GNN systems to a DL framework, and the interfaces between GNN systems and the low-level GPU kernel implementation. A brief summary is provided here.

\noindent $\bullet$
\textbf{Accuracy and Performance Benchmarking.}
We observe many critical benchmarking issues due to missing end-to-end model implementation, and the absence of training accuracy measurements. 
{We also point out that relying exclusively on smaller datasets to show performance gain as done by prior GNN systems~\cite{wang2021gnnadvisor,gespmmsc2020} does not compare the impact of kernel performance but rather compares \textit{framework overhead}. To this end, we are the first to develop a  \textit{methodology} to measure the framework overhead. Overall, the investigation {questions the practical aspects of many proposed optimizations}.
%These issues also make DGL~\cite{dgl2019} the only end-to-end reliable \textit{baseline} that can be used to quantify the performance of future GNN systems. despite claims in several recent publications~\cite{wang2021gnnadvisor,huang2021understanding,fu2022tlpgnn,gespmmsc2020, wu2021seastar,chen2020fusegnn,featgraphsc20}. 
%These issues lead to two important use cases for which several interface-level limitations exist today as explained below.
%The full model implementation and accuracy measurement is needed to show the correctness of the developed kernel.  

% \red{\noindent $\bullet$
% \textbf{Framework Overhead Analysis and Methodology.}
% We are the first ones to state that the performance evaluation should rely on large data sets instead of the small data set because the overall training time in small data sets is dominated by the GNN system's framework overhead. Based on this observation, we also propose a methodology that can evaluate the framework overhead.}

\noindent $\bullet$
\textbf{DL Framework to GNN System (high-level) Interfaces.} End-to-end prototyping is needed to measure the accuracy to avoid the mentioned issues. But current DL frameworks do not allow passing any custom object, such as a graph to GNN systems, leading to reliance on workarounds for integration. This results in unstable system APIs whose signature changes for every custom graph storage. It deters innovation in graph storage and causes productivity and compatibility loss. %Hence, prior tools do not encourage end-to-end GNN system development.
%tensors to an independent module is very complex,
%out that a few GNN systems have critical issues in understanding system requirements, implementation 
%(a) The performance improvement stated in many prior works is not useful and prohibits their deployment to real-world GNN applications.
%{(b) Need of a Better GNN Baseline:}
%In this work, we observe (\cref{sec.obs}) many such issues in existing works, including an absence of end-to-end model implementation, avoiding training accuracy measurements, etc. 
%As we study code base of prior works and evaluate their work, we find that the optimization achieved by these works cannot be relied upon as they do not fully implement the GNN model correctly. Hence, 
%they would have benefited by following our recommendations such as enforcing GNN training accuracy, and using larger datasets for performance measurement.
%Similarly, assignments and tools should be developed to impart an end-to-end understanding of DL/GNN systems to future systems researchers and engineers.
%while the performance measurement should happen on larger datasets.


\noindent $\bullet$
\textbf{GNN Systems to CUDA kernel (low-level) Interfaces.}
CuSparse library defined general-purpose sparse kernels over a decade ago. However, it is not directly suited as kernels for GNN use cases. This low-level interface mismatch introduces extra memory allocation, additional kernel calls, and the materialization of intermediate results causing a slowdown and increased memory consumption in DGL. However, others~\cite{gespmmsc2020,featgraphsc20,huang2021understanding} continue to optimize the same kernel definitions and suffers from the cost of generality and mismatch.

\noindent
\textbf{2. Research Tool (\cref{sec.usecase} and \cref{sec.science}).}
To this end, {\graphpy} \textit{auto-generates codes to integrate GNN systems to DL frameworks} based on a simple domain-specific language. 
%users to write the kernel, called \textit{\graphpy-Kernel} independently without involving any DL frameworks, and have no version dependency whatsoever. {\graphpy} 
It relies on a proposed \textit{Half DLPack protocol} to offer DL framework-specific tensors to GNN systems using flat arrays. This achieves DL framework-independent GNN system, which in turn, removes all restrictions on passing graph objects to it. Further, {\graphpy} proposes \textit{graph storage management} module to prepare and export graphs to GNN systems as per GNN-specific graph edge property requirements. 

Through these mechanisms, {\graphpy} achieve \textit{productivity and re-usability} of GNN system across DL frameworks and their versions and also streamlines the interfaces for graph handling.
Further, we are unaware of any system that can support arbitrary multi-field edge properties. It also cannot be designed without significant innovations.

%The proposed tool also reduces the framework overhead due to its simplistic design. 

 
%\bullet$
%\noindent
%\textbf{3. Graph Storage Management (\cref{sec.engg}).}
% Analyzing different GNN models shows the need for graph storage with different edge properties. The current ad hoc approaches to handling graph storage present another productivity issue and a challenge to interface design and system integration. 
% We separate the graph storage management to another independent module to prepare graphs by specifying GNN specific edge properties succinctly using a single API. The API exports the prepared graph using \textit{zero-copy} arrays to the GNN system. 
% We are unaware of any system that can support arbitrary multi-field edge properties. It also cannot be designed without significant innovations.

%to satisfy the diverse storage needs of various classes of GNN, which cannot be supported by current tools.
%to achieve better performance in graph preparation and productivity in
%By relying on  Dtype, {\graphpy} makes sparse matrix (i.e., graph) same as dense matrix (e.g., image data) for storage specification and exchange purpose. 
%Interface design leaves enough room in {\graphpy-Kernel} to innovate on graph storage design without impacting {\graphpy-SM}.


% $\bullet$
\noindent
\textbf{3. GNN Inspired Kernels and an Optimized Baseline (\cref{sec.baseline}).}
We capture the system requirement using a new set of kernel definitions  that can directly be used inside GNN systems without any requirement mismatch and memory overhead. 
Based on these new kernels, we present a new GNN baseline 
%by removing the various overheads and fusing the kernels by carefully studying the GNN models
ensuring correct training accuracy and better performance amid low memory consumption. 


%presents much more than memory and performance optimization. It rather establishes a new  

% \noindent $\bullet$ 
% \textbf{Graph Data Management for DL.}
% We separate the graph storage management to another independent module, \textit{\graphpy-SM}, to handle multi-field graph properties using a single set of API by using \textit{NumPy Dtype}, while exporting the prepared graph storage to {\graphpy-Kernel} using \textit{zero-copy} NumPy arrays. 
% %and allow innovations in interface design
% By relying on  Dtype, {\graphpy} makes sparse matrix (i.e., graph) the same as a dense matrix (e.g., image data) for storage specification and exchange purposes. 
% Interface design leaves enough room in {\graphpy-Kernel} to innovate on graph storage design without impacting {\graphpy-SM}.
% We are unaware of any high-performance Python package that can support arbitrary multi-field graph properties. It also cannot be designed without significant innovations(\cref{sec.engg}).

%We demonstrate the usefulness of {\graphpy} with the implementation and evaluation (\cref{sec.exp}) of many GNN models. 
%on an average 1.64$\times$ and 1.42$\times$ speedup and 1.30$\times$ and 2.29$\times$ speedup over DGL, and PyTorch Geometric for various GNN models in GPU and CPU respectively. 
%Further, frequent out-of-memory conditions by DGL, Pytorch-Geometric, and GNNAdvisor force measurements to be performed on smaller dataset only. Measurements on smaller prevalent dataset do not show advantage of kernel optimization due to framework overhead.

Our evaluations (\cref{sec.exp}) show that {\graphpy} reduces memory consumption on average by 6.92$\times$ on GCN, 3.4$\times$ on GIN, and 1.96$\times$ on GAT-1 models in comparison to DGL, while DGL, Pytorch-Geometric~\cite{pytorchg2019} (PyG) have many out-of-memory conditions. 
Further, {\graphpy} achieves on average 1.38$\times$ 1.51$\times$, 1.58$\times$, 1.32$\times$ speedup for GCN, GIN, GAT-1, and GAT-3 compared to DGL on larger datasets. 
We also show that GNN-specific kernel definition alone without any workload balancing technique can perform much better (1.16$\times$ -- 2.95$\times$) than optimized and workload-balanced generic kernels of FeatGraph~\cite{featgraphsc20}, GE-SpMM~\cite{gespmmsc2020}, GNNAdvisor~\cite{wang2021gnnadvisor}, and Huang et al~\cite{huang2021understanding}, which can not be run end-to-end along with CuSparse and DGL.
Lastly, focus on interface design minimizes the framework overhead of {\graphpy} by 1.54$\times$, and 1.35$\times$ than DGL and PyG.
%to achieve better performance on smaller datasets. 

%To show the extensibility of {\graphpy}, we also demonstrate the implementation of sparse tensors (not sparse data) on LeNet-300-100.

%Therefore, future systems optimizations can benchmark their performance against our baseline to advance the state-of-the-art rather than comparing against various overheads.

%Empirical evaluations show that our optimized implementation achieves 1.62$\times$ and 1.35$\times$ over DGL and PyTorch for various GNN models on many datasets in GPU, and 1.55$\times$ and 1.88$\times$ on CPU respectively with similar accuracy readings.\td[end]
%\footnote{See \url{https://arxiv.org/pdf/1909.01315.pdf} for DGL overhead} 
%making {\graphpy} an excellent framework for research. 
%A better GNN performance using the reference implementation, less framework overhead, and low memory consumption make {\graphpy} an ideal baseline for performance benchmarking for future research. 


% The remainder of the paper is organized as follows. We present background on graphs and DL in \cref{sec.background}. 
% %The motivation, challenges, and overview of {\graphpy} are presented in \cref{sec.overview}. 
% The detailed use cases are presented in \cref{sec.after_observation}, technical challenges and prior works in \cref{sec.challenges}.  Implementation details are presented in \cref{sec.science} and \cref{sec.engg}, evaluations in \cref{sec.exp}, and we finally conclude in \cref{sec.conclusion}.


The paper specifies many practical issues with GNN systems and provides a practical yet powerful framework to overcome those issues. 
More importantly, the proposed baseline allows {\graphpy} to train GCN on a billion-edge graph on a single GPU due to memory saving while prior works cannot train even a 500 million-edge graph. 
The new baseline also offers  newer opportunities for practical optimizations. 
%where {\graphpy} offers researchers a powerful mechanism to design end-to-end systems productively. 
Indeed, there is an immediate scope for optimizing the proposed GNN-specific kernels through various format-specific and workload-balanced designs that can be compared against the proposed baseline to show the practical impact.
Lastly, the proposed tool and mechanisms may be used for end-to-end system education to train learners on system requirement gathering for GNN/DL models and implementation, which has been flagged as a major concern in an NSF workshop~\cite{storage2025NSF}. 


==> tex/intro2.tex <==
%{\color{red}


\section{Introduction} \label{sec.intro}
%Getting insights from data is very important, and hence 
Many applications have become data-driven today. 
%These applications are now popularly known as \textit{data science}. 
Within this ecosystem, a lot of real-world data can be stored as \textit{sparse matrices} or \textit{graphs}, such as social networks, chemistry, biology, recommendation system, scene description generation, knowledge bases, etc~\cite{fan2019graph, zitnik2018modeling,hamilton2018embedding,ying2018graph,krahmer2003graph,perera2017recent,rgcn2018,wang2020entity}. 
%We call these data-driven use-cases as \textit{graph data science} 
To this end, many graph neural network (GNN) models, e.g., GCN~\cite{gcn17iclr}, GAT~\cite{gat18iclr}, GIN~\cite{xu2019powerful}, and others~\cite{gatedgraph2017,zhang18, graphsage17}, etc. have been proposed. 



% \noindent \textbf{Deep Learning on Sparse Data.}
% The neighborhood in graphs is different from other regular data, such as an image which has a fixed number of neighborhoods. To handle it, \textit{graph neural network}(GNN), has been proposed~\cite{gcn17iclr,gat18iclr,gatedgraph2017,gaan2018}. The GNN models can be trained efficiently if the graph can be used for storage. However, the current DL frameworks, such as PyTorch~\cite{pytorch2019} or TensorFlow~\cite{tensorflow2016} lack the same level of operational support for the sparse matrix that they have for dense matrix, as the original code-base of GCN~\cite{gcn17iclr}, GAT~\cite{gat18iclr} etc. have relied on bitmask at Python level to model sparsity on top of dense matrices that actually do not reduce computation or memory consumption. %because the underlying kernel still uses the dense matrix.


% traditional GNNs use the adjacency matrix to represent the graph structure and tensor operation to perform the forward and backward computations. 
% However, due to the sparsity, this will trigger the out-of-memory problem to represent a sizeable sparse graph and will cause computation inefficiency for tensor operation. 

% Since deep learning techniques can achieve excellent prediction, many graph neural network (GNN) works were proposed. Graph neural network (GNN) is about applying deep learning algorithms on the graph structure to do classification and prediction tasks, such as node classification, edge/link prediction, and graph classification. 
% The node classification denotes that given a graph structure and a subset of nodes with labels, the graph deep learning algorithm should predict the label of the remaining nodes. 
% In contrast, the link prediction tasks are predicting whether an edge exists between two given nodes or not, such as in auto-completing knowledge bases.


% \noindent \textbf{Deep Learning On Sparse Tensors.}
% DL Model compression techniques, such as weight pruning ~\cite{han2015learning,han2016iclr},  convert a dense model layer to a sparse layer by removing a lot of low-impact model parameters. 
% These techniques help to deploy large models on resource-constrained devices because the compressed models need less memory and CPU. Before deploying them, the compressed models undergo \textit{re-training}. This re-training step can be more efficient if the graph is used to model sparse layers. However, prior works~\cite{han2015learning} used bit-mask matrix in Python, and underlying dense matrix to achieve sparsity. Thereby, the \textit{re-training process did not really consume less memory}, hence we may not be able to use resource-constrained systems to do re-training, which are low on memory.

%These models also have inspired a number of systems optimizations~\cite{wang2021gnnadvisor,huang2021understanding,gespmmsc2020,fu2022tlpgnn,wu2021seastar,chen2020fusegnn}. However, our study finds that many of these design decisions indicate inadequate understanding because 

It should be noted that GNN, like deep learning (DL), training has a unique computation need. \textit{Forward computation} calls many \textit{kernels} (operations on data) from the input layer to the output layer to derive the prediction values which are compared with the ground truth to calculate the loss.
% and plug the loss into the backward procedure. 
Then, \textit{backward computation} uses the loss to derive the gradient by invoking kernels from the output layer to the input layer to update the model parameters.
%It uses the chain rule of gradient back-propagation to update the model parameter from it. 
Kindly note that the backward computation accesses results that are either accessed or produced in the forward computation and are called \textit{state tensors} (Fig.~\ref{fig-format}(a)). This computation paradigm differs from the prior forward-only related fields, e.g., graph analytics.
 
\noindent \textbf{Motivation: Missing End-to-End Focus.}
 Many prior works either do not provide a full GNN model for training or do not measure training accuracy ~\cite{wang2021gnnadvisor,huang2021understanding,fu2022tlpgnn,wu2021seastar, chen2020fusegnn, kim2022analyzing,yan2020hygcn,liang2020engn,zhang2021boostgcn, geng2020awb}. 
 %have established a clear trend of not showing the training accuracy, while many have missing end-to-end implementation.
%Our analysis shows that 
This has led to significant practical issues. 
%including questioning  some of their proposed optimization techniques.
Consider the case of the GAT model that calls 18 kernels in each layer~\cite{fu2022tlpgnn} in its forward computation. An obvious optimization technique is to fuse them into just one~\cite{fu2022tlpgnn,huang2021understanding}. However, both of them have missing backward computation that allowed them to avoid materializing the trainable edge-level GAT model parameter ($W_e$) in their forward computation, and thereby not keeping edge ID(\cref{sec.background}) in their graph to access it. 
On the other hand, GNNAdvisor~\cite{wang2021gnnadvisor}, an end-to-end system, does not show training accuracy. Sadly, its codebase does not fuse the kernel correctly in the backward computation of GCN, and its model does not use bias, a vital model parameter. 

These works gain performance unknowingly at the expense of accuracy, so their demonstrated optimizations are not yet practical until training accuracy is shown by implementing the backward computation correctly. It is likely to alter the fundamental foundation of many proposed optimizations. % \red{which motivate this work.} 
In this paper, our \textit{contribution} is multi-fold. We first analyze the current GNN systems from various perspectives identifying many vital issues at different layers of the ecosystem and proposing a comprehensive platform to overcome them. 

\noindent
\textbf{I.} 
We summarize our in-depth analysis next.

\noindent %$\bullet$
%\textbf{Issues about Accuracy and Performance Benchmarking.}
\textbf{\#3.end-to-end real environment).}


\textbf{\#1. Independental kernel design).}



\textbf{\#2. auto generated intergated code design).}

\textbf{\#3. easily installed environment).}

%Such additional steps would have enforced a brainstorming around the need for \textit{state tensors} and other GNN-specific requirements. 
%Fused kernels that avoid producing such tensors in the forward computation must implement backward computation to show that such fusion is feasible and justify them through training accuracy measurements.
%do not understand the system requirement from the GNN perspective. 
%Unfortunately,
%Hence, their optimization has no significance at this moment. We present various such observations in \cref{sec.obs}, however, the pressing question is whether such optimizations really advance the state-of-the-art. 
%and whether these mistakes are systematic.


%Further observations point us that many researchers do not understand GNN workflow exactly
%For example, 

%GE-SpMM~\cite{gespmmsc2020} forgets to consider the edge-level tensor when implementing the kernels. Section (\td) explains this analysis in detail. 



%\noindent \textbf{Systematic Lack}:
%We argue that these mistakes are systematic in nature. We present the following arguments to explain it. 

% No architecture papers \cite{yan2020hygcn,liang2020engn,zhang2021boostgcn}
%{\td  \cite{zhang2021boostgcn, geng2020awb, yan2020characterizing} only for inference and no accuracy}: Will see them later whether to include or not.
%\cite{baruah2021gnnmark} uses dgl and pyg, so not citing here.

%--------------
%(1) \textbf{No Training Accuracy Measurements and/or Missing Backward Computation.} 
% Indeed many prior works~\cite{wang2021gnnadvisor,huang2021understanding,fu2022tlpgnn,wu2021seastar, chen2020fusegnn, kim2022analyzing} do not measure the training accuracy either because they do not implement the backward computation or simply do not measure it despite having an end-to-end implementation.
% Hence, they may be totally unaware of the mistakes. 
% For example, GNNAdvisor~\cite{wang2021gnnadvisor}, and end-to-end GNN system does not fuse the normalization kernel correctly in the backward computation, while omitting the bias parameter from each GCN  layer (\cref{sec.obs}).
% %provides a more detailed analysis for this example). 
% Similarly, Huang et al~\cite{huang2021understanding}, and TLPGNN~\cite{fu2022tlpgnn} optimized the GAT model's forward computation without implementing its backward computation due to which they committed serious mistakes of wrongly fusing the kernels, including removal of edge-level tensors. Wrongly fused kernels can also alter the requirement significantly as they do not keep edge ID in their graph to access the attention score tensor in GAT(\cref{sec.obs}).


%Clearly, the research community has also not forced these works to measure training accuracy. 

%in form a natural boundary across which they cannot be blindly fused in the forward computation as they are needed in the backward 

% (2) \textbf{No Backward Computation.} Many prior works~\cite{huang2021understanding,fu2022tlpgnn}[\red{what about seastar and other works}] have not implemented a backward computation at all, and their optimizations focused on only the forward computation due to which they committed serious mistakes of wrongly fusing the kernels, including removal of edge-level tensors. We believe general awareness of GNN workflow and understanding is lacking, such as the need for \textit{state tensors}. Kernels producing such tensors form a natural boundary across which kernels cannot be fused in the forward computation. Wrongly fused kernels can also alter the requirement significantly. For example, Huang et al\cite{huang2021understanding}, and  TLPGNN\cite{fu2022tlpgnn} do not keep edge ID in their graph to access attention score tensor in GAT(\cref{sec.obs}). %(Section {\td} provides a more detailed analysis for this example). 
% %This mistake will be realized easily if these works implemented the backward kernel.
% % (3) One of the observations from such works is that they try to write GNN systems from scratch using current DL frameworks, such as PyTorch, TensorFlow, etc. 

% We explore the current methodology and find that it is very complex to write a GNN system from scratch because  passing the graph object and tensors to an independent module is very complex, and on top of this, users have to learn new build systems (Ninja), Python binding, memory management (due to delayed free of state tensors), etc. to integrate their code with a DL framework. We experienced the same issues ourselves when we tried to build a new baseline that resulted in exhaustion in just setting up the system. And, hence such exhaustion may force the researchers to not build an end-to-end system. 


%\noindent \textbf{End-to-End Systems Teaching.} 
%The academic community is also not encouraging end-to-end \textit{system} teaching. E.g., publicly listed assignments on DL/GNN {systems} courses offered by many universities~\cite{dlsCMU, cs15884CMU, cse599wWashington,cs231nStandford} \textit{focus only on the forward kernel} of an operator, and in Python without its integration in an end-to-end DL/GNN system. Hence, students cannot fully understand, appreciate, and gather complete requirements. Rather, industry partners have voiced concern about the availability of candidates with good systems and data science knowledge in an NSF workshop~\cite{storage2025NSF}.


\begin{figure*}[t]
  \includegraphics[scale= 0.55]{result/edge_id_crop.pdf}
  \vspace{-12pt}
  \caption{\small (a) One GNN layer using GAS (gather-apply-scatter) to model the kernel: X and Y are intermediate features, and $W_e$ is the model parameter of the layer, e.g. attention score in case of GAT. X, Y, and $W_e$ tensors are \textit{state}, as they are used in backward computation. $A$ and $A^T$ are graph and its inverse respectively. (b) Sample graph (c and d) CSR and CSC representation along with edge ID indirection.}
  \label{fig-format}
 \vspace{-12pt}
\end{figure*}



\noindent %$\bullet$
%\textbf{Issues about Accuracy and Performance Benchmarking.}
\textbf{\#1. Questionable GNN System Optimizations(\cref{sec.obs}).}
We outline many critical system issues due to missing end-to-end model implementation and no measurement of training accuracy. 
Further, we point out that relying exclusively on smaller datasets to show performance gain as done previously~\cite{wang2021gnnadvisor,gespmmsc2020} does not compare the impact of kernel performance but rather compares \textit{framework overhead}. We are also the first to develop a  \textit{methodology} to measure the framework overhead to show this effect. Overall, the investigation {questions the practical aspects of many proposed optimizations}.
%These issues also make DGL~\cite{dgl2019} the only end-to-end reliable \textit{baseline} that can be used to quantify the performance of future GNN systems. despite claims in several recent publications~\cite{wang2021gnnadvisor,huang2021understanding,fu2022tlpgnn,gespmmsc2020, wu2021seastar,chen2020fusegnn,featgraphsc20}. 
%These issues lead to two important use cases for which several interface-level limitations exist today as explained below.
%The full model implementation and accuracy measurement is needed to show the correctness of the developed kernel.  

% \red{\noindent $\bullet$
% \textbf{Framework Overhead Analysis and Methodology.}
% We are the first ones to state that the performance evaluation should rely on large data sets instead of the small data set because the overall training time in small data sets is dominated by the GNN system's framework overhead. Based on this observation, we also propose a methodology that can evaluate the framework overhead.}

\noindent %$\bullet$
\textbf{\#2. Interface Limitation(\cref{sec.usecase}).} End-to-end prototyping is needed to measure the accuracy. But current DL frameworks do not allow passing custom objects, such as a graph to GNN systems, leading to workarounds for integration. This results in unstable system APIs whose signature changes for every custom graph storage. It deters innovation in graph storage, causes productivity loss, and leads to compatibility issues across various DL frameworks and their versions. 
%Hence, prior tools do not encourage end-to-end GNN system development.
%tensors to an independent module is very complex,
%out that a few GNN systems have critical issues in understanding system requirements, implementation 
%(a) The performance improvement stated in many prior works is not useful and prohibits their deployment to real-world GNN applications.
%{(b) Need of a Better GNN Baseline:}
%In this work, we observe (\cref{sec.obs}) many such issues in existing works, including an absence of end-to-end model implementation, avoiding training accuracy measurements, etc. 
%As we study the code base of prior works and evaluate their work, we find that the optimization achieved by these works cannot be relied upon as they do not fully implement the GNN model correctly. Hence, 
%they would have benefited by following our recommendations such as enforcing GNN training accuracy, and using larger datasets for performance measurement.
%Similarly, assignments and tools should be developed to impart an end-to-end understanding of DL/GNN systems to future systems researchers and engineers.
%while the performance measurement should happen on larger datasets.


\noindent %$\bullet$
\textbf{\#3. Requirement Mismatch (\cref{sec.usecase}).}
CuSparse library offers general-purpose sparse kernels for over a decade that has served well in many scientific computations. However, it is not directly suited as kernels for GNN use cases. This requirement mismatch introduces  additional kernel calls, extra memory allocation, and the materialization of intermediate results. DGL~\cite{dgl2019} and PyTorch~\cite{pytorch2019} which use CuSparse suffer a slowdown and increased memory consumption and hence do not allow training slightly larger datasets. However, others~\cite{gespmmsc2020,featgraphsc20,huang2021understanding} continue to optimize the same kernel definitions and suffers from the \textit{cost of generality}. 
%and \textit{requirement mismatch}.

%Based on the above-mentioned issues, it seems that DGL is the only system that can serve as an end-to-end GNN system baseline for diverse GNN model benchmarking. But due to requirement mismatch, DGL is not a competitive baseline. Hence, 

\noindent
\textbf{II.} 
Above mentioned issues lead to the identification of the following requirements and contributions.
%identify the following initiatives for GNN systems: 

\noindent $\bullet$
\textbf{Insights and Recommendation (\cref{sec.obs}).} This paper makes researchers and the community aware of these practical issues (\#1) and their vital impact on the progress of GNN system research. This will bring our recommendation in the right perspective so that researchers and the community together can enforce them to truly advance the state-of-the-art.

\noindent $\bullet$
\textbf{The Platform (\cref{sec.science}).} There is a need for an ecosystem to overcome the limitation of current DL frameworks (issue \#2) and let researchers prototype their system idea productively in an end-to-end fashion without compromising on innovation potential.
To this end, {\graphpy} \textit{auto-generates codes to integrate GNN systems to DL frameworks} based on a simple domain-specific language. 
It relies on a proposed \textit{Half DLPack protocol} to offer DL framework-specific tensors to GNN systems using flat arrays. This achieves a DL framework-independent GNN system, which in turn, removes all restrictions on passing graph objects, and ensures \textit{re-usability} of GNN system across DL frameworks and their versions saving potential cost in order to integrate the same idea across DL frameworks. 
Further, {\graphpy} proposes \textit{graph storage management} module to prepare and export graphs to GNN systems as per GNN-specific graph edge property requirements to streamline the interfaces for graph handling, and implements many types of GNN models.
We are unaware of any system that can support arbitrary multi-field edge properties. It also cannot be designed without significant innovations.

% Through these mechanisms, {\graphpy} allows researchers to plug their GNN system productively to achieve an end-to-end implementation so that it can be evaluated for accuracy to avoid these practical issues early during the prototype. 
% Moreover, {\graphpy}  ensures \textit{re-usability} of GNN system across DL frameworks and their versions saving potential cost in order to integrate the same idea across DL frameworks. 

%The proposed tool also reduces the framework overhead due to its simplistic design. 

 
%\bullet$
%\noindent
%\textbf{3. Graph Storage Management (\cref{sec.engg}).}
% Analyzing different GNN models shows the need for graph storage with different edge properties. The current ad hoc approaches to handling graph storage present another productivity issue and a challenge to interface design and system integration. 
% We separate the graph storage management to another independent module to prepare graphs by specifying GNN specific edge properties succinctly using a single API. The API exports the prepared graph using \textit{zero-copy} arrays to the GNN system. 
% We are unaware of any system that can support arbitrary multi-field edge properties. It also cannot be designed without significant innovations.

%to satisfy the diverse storage needs of various classes of GNN, which cannot be supported by current tools.
%to achieve better performance in graph preparation and productivity in
%By relying on  Dtype, {\graphpy} makes sparse matrix (i.e., graph) same as dense matrix (e.g., image data) for storage specification and exchange purpose. 
%Interface design leaves enough room in {\graphpy-Kernel} to innovate on graph storage design without impacting {\graphpy-SM}.



% \noindent $\bullet$
% \textbf{GNN Inspired Kernel.}
% That ecosystem should design kernels based on GNN use cases to provide an optimized GNN baseline (\cref{sec.baseline}) to show the performance improvement of doing things correctly and enable evaluations on larger datasets. This will allow future optimizations to compare system performance instead of the overhead or requirement mismatch.

% 
\noindent $\bullet$
\textbf{GNN Inspired Kernels (\cref{sec.baseline}).}
{\graphpy} captures the system requirement using a new set of kernel definitions  that can directly be used inside GNN systems without any requirement mismatch and memory overhead. 
Based on these new kernels, {\graphpy} presents a new GNN baseline 
%by removing the various overheads and fusing the kernels by carefully studying the GNN models
ensuring correct training accuracy and better performance amid low memory consumption. 
%This enables the evaluation of GNN training on larger datasets in a single GPU.


% {\td does the above words explain "What can \graphpy do to overcome these practical issues?"1. They can follow our advice to avoid the issues 2.use our GraphPy to avoid}

Our evaluations (\cref{sec.exp}) show that {\graphpy} reduces memory consumption on average by 6.92$\times$ on GCN, 3.4$\times$ on GIN, and 1.96$\times$ on GAT-1 models in comparison to DGL, while DGL, Pytorch-Geometric~\cite{pytorchg2019} (PyG) have many out-of-memory conditions. 
Further, {\graphpy} achieves on average 1.69$\times$ 1.22$\times$, 1.50$\times$, 1.27$\times$ speedup for GCN, GIN, GAT-1, and GAT-3 compared to DGL on larger datasets. 
We also show that GNN-specific kernel definition alone without any workload balancing technique can perform much better (1.16$\times$ -- 2.87$\times$) than optimized and workload-balanced generic kernels of FeatGraph~\cite{featgraphsc20}, GE-SpMM~\cite{gespmmsc2020}, GNNAdvisor~\cite{wang2021gnnadvisor}, and Huang et al~\cite{huang2021understanding}, which can not be run end-to-end along with CuSparse and DGL.
Lastly, focus on interface design minimizes the framework overhead of {\graphpy} by 1.54$\times$, and 1.35$\times$ than DGL and PyG.
%to achieve better performance on smaller datasets. 

%To show the extensibility of {\graphpy}, we also demonstrate the implementation of sparse tensors (not sparse data) on LeNet-300-100.

%Therefore, future systems optimizations can benchmark their performance against our baseline to advance the state-of-the-art rather than comparing against various overheads.

%Empirical evaluations show that our optimized implementation achieves 1.62$\times$ and 1.35$\times$ over DGL and PyTorch for various GNN models on many datasets in GPU, and 1.55$\times$ and 1.88$\times$ on CPU respectively with similar accuracy readings.\td[end]
%\footnote{See \url{https://arxiv.org/pdf/1909.01315.pdf} for DGL overhead} 
%making {\graphpy} an excellent framework for research. 
%A better GNN performance using the reference implementation, less framework overhead, and low memory consumption make {\graphpy} an ideal baseline for performance benchmarking for future research. 


% The remainder of the paper is organized as follows. We present background on graphs and DL in \cref{sec.background}. 
% %The motivation, challenges, and overview of {\graphpy} are presented in \cref{sec.overview}. 
% The detailed use cases are presented in \cref{sec.after_observation}, technical challenges and prior works in \cref{sec.challenges}.  Implementation details are presented in \cref{sec.science} and \cref{sec.engg}, evaluations in \cref{sec.exp}, and we finally conclude in \cref{sec.conclusion}.

%\red{The contributions of this paper are summarized below.}
%\noindent \textbf{Summary}
In summary, we are the first ones to specify many practical issues with GNN systems, provide useful recommendations, and offer a simple yet powerful framework to overcome many of those issues. 
% \red{2. We also state the reason why there is a need for an end-to-end platform which can help researchers  to avoid these practical issues before showing the performance gain.}
{More importantly, the proposed baseline can train GCN on a billion-edge graph on a single GPU due to memory saving while prior works cannot train even a 500 million-edge graph.} 
The new baseline also offers  newer opportunities for practical optimizations. 
%where {\graphpy} offers researchers a powerful mechanism to design end-to-end systems productively. 
%Indeed, there is an immediate scope for optimizing the proposed GNN-specific kernels through various format-specific and workload-balanced designs that can be compared against the proposed baseline to show the practical impact.
Lastly, the proposed tool and mechanisms may be used for end-to-end system education to train learners on system requirement gathering for GNN/DL models and implementation, which has been flagged as a major concern in an NSF workshop~\cite{storage2025NSF}. 

% \red{The contributions of this paper are summarized below.}

% \red{1. We are the first ones to analyze the existing GNN system optimizations, the current practices to integrate GNN systems to a DL framework, and the interfaces between GNN systems and the low-level GPU kernel implementation. 
% Based on the analysis, we observe that system optimizations based on a partial understanding of the GNN model may not lead to a practical system. 
% 2. We also state the reason why there is a need for an end-to-end platform which can help researchers  to avoid these practical issues before showing the performance gain.
% 3. We propose the {\graphpy} which can satisfy the need and let researchers implement their kernel prototype easily by the novel interface design. {\td no sure whether we should extend, such as we can run GAT on large datasets, which is important because researchers should not rely performance on small dataset}
% 4. {\graphpy} implements a set of GNN-inspired reference kernels after understanding of requirements of GNN systems and these kernels avoid requirement mismatch and other practical issues. Moreover, since these GNN-inspired kernels only apply traditional optimization techniques( feat-level parallelism) instead of specific techniques( such as workload balancing), {\graphpy} can be viewed as the practical baseline for future GNN system research. {\td maybe need a reason to define what is GNN specific problem}}



==> tex/kernel.tex <==
\section{{\myname-Kernel}: GNN Specific Kernel} \label{sec.baseline}

We now present kernels that are directly suited for Class A and B GNN use cases without incurring any requirement mismatch overhead. The proposed CUDA kernels have almost similar signatures as the system APIs of Table~\ref{table-api}. To recap, our investigation in \cref{sec.obs} and \cref{sec.usecase} pointed out that not just DGL (or CuSparse), but many others~\cite{gespmmsc2020,featgraphsc20,huang2021understanding} have continued developing CuSparse compliant-gSpMMve for GNN use-cases.  
%for at least class B GNN, namely gSpMMveid, while many still provide gSpMMve for class A GNN. 
%Also, APIs for CuSparse are not well-suited GNN use cases as discussed in \cref{sec.dgl}, which other works continue to optimize, such as gSpMMve, and not gSpMMveid which they should. 
%We define new signatures of \textit{gSpMMv} and \textit{gSpMMveid}. 


\noindent \textbf{gpk$\_$gSpMMveid.}
This {\myname} kernel is a weighted gSpMM that accepts vertex-level and an edge-level tensor. However, it accesses the edge-level tensor using edge ID which is part of the graph storage. We also support a vector feature for each edge, which is used by the multi-head GAT model.

 Memory saving and performance gains are achieved by {\myname} just because of the new API design compared to all prior systems. (1) It accesses the edge-level tensors directly using the edge ID, hence eShuffle kernel is completely avoided, and so is the need to materialize an additional tensor of size O($|E|$), thus saving memory. (2) This kernel is faster than even a workload-balanced gSpMMve plus a separate eShuffle kernel. (3) The multi-head gSpMMveid cannot be simulated by the CuSparse-compatible gSpMMve kernel.


\noindent \textbf{gpk$\_$gSpMMv.}
This kernel is unweighted gSpMM. Hence, it only accepts a vertex-level tensor as input along with reduction operation type, such as \textit{sum, min, max} but not any edge-level tensor. The API also accepts an optional boolean flag to indicate normalization by degree flag. When the flag is true, it only normalizes the result of gSpMM as part of the same kernel. Hence, in the backward computation, the flag should be set as false, and a separate normalization kernel should be called. This API is used by class B GNNs. 

This kernel definition, though very intuitive, differs from prior works. CuSparse, FeatGraph, Huang et al offer gSpMMve. GNNAdvisor does not make normalization optional and ends up with the wrong fusion during backward. GE-SpMM has mostly focused on gSpMMve, and silently implements gSpMMv without the normalization option. 
This vital change provides substantial memory saving to {\myname} on two accounts. (1) Compared to CuSparse compliant gSpMMve, {\myname-GNN} never need to allocate dummy edge-level tensor saving O($|E|$) memory. This also results in a substantial performance gain. 
(2) Even in the case of a separate normalization, {\myname} uses the same tensor as input and output both by using in-place normalization inside {\myname-GNN}. On the other hand, DGL performs normalization at Python level using  PyTorch's CUDA API that can only perform out-of-place normalization, Thus increasing the memory consumption by O($|V|$*feature-length). Hence, DGL-integrated systems, such as GE-SpMM and FeatGraph likely to consume additional memory as well.

\noindent \textbf{gpk$\_$gSDDMMve.}
We did not define gpk$\_$gSDDMMveid, as we generated COO in a way that can rely on an implicit edge ID equivalent of the position of each edge in the COO. %to use gpk$\_$gSDDMMve. 
%COO offers edge-parallel implementation, which achieves fully workload-balanced implementation. 

\noindent \textbf{gpk$\_$gSDDMMvv.}
It remains the same as discussed in \cref{sec.obs}.


We use CSR/CSC with vertex-level parallelism for gSpMM. We incorporated feature-level parallelism~\cite{yang2018design} when the features are vector, and used caching~\cite{gespmmsc2020}.
For reduction, we use a tree reduction~\cite{wang2016gunrock} wherever applicable. These techniques are used by most prior gSpMM works. We did not do any specific workload balancing.
We perform edge-level parallelism by using the COO format for gSDDMM variants, which by default have a workload-balanced design. We do not optimize the resultant kernels or fuse them any further.
\textit{This approach shows that devising the right kernels alone has the potential to speed up GNN training and lower memory consumption}.

% \noindent
% \textbf{1. Framework Overhead Reduction.}
% %\red{DGL has significant overhead for small datasets. To reduce the Framework overhead, }
% Prior works reduced framework overhead by moving the model layer to C++, which did not follow the guidelines property, as it could be complex to write those correctly. We left the model layer code in Python. However, we reduced the framework overhead by removing the system initialization steps of DGL which allocates many intermediate memory objects to bridge the requirement mismatch which takes a huge time (\cref{sec.exp-gnn}). 
% %dummy edge-level tensors, 
% Further, {\graphpy} uses code generation to define and implement interfaces. In doing so, it generates separate interfaces for each gSpMM and gSDDMM variant, thereby simplistic nature of {\graphpy} interfaces can invoke the right kernel variant quickly as we avoid having a message passing infrastructure and other overheads of DGL to locate the exact kernel variant to invoke. 
% %Further, for fused kernel design, {\graphpy} generates a new kernel from the DSL specification of the kernel. 
% Therefore, {\graphpy} optimized the training for small datasets.


% As we mention in \cref{sec.usecase}, DGL relies on CuSparse which creates requirement mismatch, hence DGL invokes additional kernels while materializing many intermediate results. We explain  how we remove these overheads.
% %class A type of GNN models use the unweighted sum for aggregation and use vertex-level tensor only. 
% %Class B type of GNN models touches both vertex level and edge level tensor. 
% %DGL uses gSpMMve kernel to handle  this. \red{ which involves extra unneeded computation. To optimize this situation, } {\graphpy} separates the gSpMM kernel into two specific designed kernels: gSpMMv designed for class A GNN which does not fetch the edge level tensor;  gSpMMve, designed for class B operates on vertex-level and edge-level tensors. \red{Since gSpMMv kernel does not fetch the unneeded edge-level weight anymore, the class A type of GNN models can achieve both better memory-saving and better time-saving. }
% (a) DGL uses a dummy edge-level tensor with each value as 1.0 to implement gSpMMv using CuSparse API, we directly implement gSpMMv without this dummy edge-level tensor. 
% (b) CuSparse does not offer edge-ID indirection, hence DGL first re-arranges the edge-level tensors using the edge ID, called \textbf{eShuffle}, for each gSpMMve kernel invocation. {\graphpy} supports merges eShuffle inside its new gSpMMve implementation using edge ID in its graph storage.  (c) DGL does \textbf{two additional transposes} using CuBLAS library because CuSparse API that DGL uses expects tensors in column-major layout. 
% %Here is a comment from its code base re-produced almost verbatim that explains the rationale: “\textit{We use CuSparse to perform the following operation: C = A x B, where A is a sparse matrix in CSR format, and B is the dense matrix for the node feature tensor. However, since CuSparse only supports column-major, while our tensor is stored in row-major, the actual computation is: C = trans(A x trans(B)). Currently, we use CuBLAS to implement transposition and allocate intermediate workspace memory for this.}''.
% (d) CuSparse API does not fuse normalization by degree array; hence, DGL calls normalization separately using PyTorch API in Python. {\graphpy} gSpMMv kernel is written using template meta-programming which uses normalization as a template parameter and hence can handle both cases efficiently. 

% \textbf{3. No Transpose and Shuffle Kernels.}
% \red{Unlike existing works, {\graphpy} removes the need for some computations by re-defining the computation kernel. For example, In both the class A and class B type of GNN models, {\graphpy} avoid the need to transpose on vertex-level features as our gSpMM variants support row-major operations directly.}
% % For both the GNN classes, we avoid the need to transpose on vertex-level features as our gSpMM variants support row-major operations directly.
% %For class A type of GNN, Without integrating with CuSparse, GraphPy can omit the requirement that the input should be column-based. Therefore, two additional transpose computations are not needed. 
% %By removing these additional computations, our end-to-end time does speed up. 
% For the class B type of GNN, GraphPy introduces an edge ID directly as an edge property in the graph using DType, and gSpMMve uses the edge ID directly in the computation. Hence, it also removes eShuffle kernel. By removing this kernel, we do not need to materialize the shuffle output.

% \textbf{4. Kernel Fusion with careful investigation}
% Although existing works fuse several kernels to improve the performance, they~\cite{wang2021gnnadvisor,huang2021understanding,fu2022tlpgnn} fuse the kernel wrongly. By realizing these issues, 
% {\graphpy} fuses the kernel carefully by understanding the requirement from an end-to-end systems perspective.  For example in GCN, {\graphpy} performs the aggregation first and then normalizes the result with the degree array in the forward direction. However, in backward, {\graphpy} normalizes the input tensor first and then performs the kernel computation. 
% Similarly, for gSpMMve, {\graphpy} implicitly fuses eShuffle and gSpMM computation.
% %Therefore, {\graphpy} can be viewed as the improved baseline. (\td measure our way is slow. Gnnadvisor is wrong but fast)



% \subsection{Optimizations}
% \label{sec.optimization}

% % \begin{figure}[h]
% %   \includegraphics[scale= 0.5]{result/mul_graph.pdf}
% %   \caption{Supporting sparse models need for multiple graphs. It can also be a bipartite graph, such as layer parameters of sparely connected layer.}
% %   \label{fig-mul_graph}
% % \end{figure}

% % It should be noted that this specific kernel is also a from of SPMM, but it is truly SPMM unlike the weighted aggregation that is used in GAT. Specifically, in GAT, the vector feature vector of each vertex is multiplied with a scalar attention score of each edge before aggregation (which is more like SpMV). But in sparse connected layer, it is truly SpMM where input dense matrix is multiplied with sparse tensor matrix.


% The focus of the paper is on the interface design, and abstraction of common tasks to independent modules, however we do implement some known parallelization strategy, which makes our kernel implementation different than DGL and Pytorch Geometric (\cref{sec.exp}). We also propose following new optimizations to demonstrate that new optimization can easily be implemented.

% \noindent \textbf{Edge ID Reordering.}
% We observe that sparse version of fully connected layer and GAT, both keep edge-level tensors or weights, which is used by forward computation, and accepts gradients during backward. This is different from traditional graph analysis where edge does not need to materialize the edge level messages. So, the performance is sensitive to how the edge IDs are allocated to the edges to avoid performing random read and write to edge level tensors. Current allocation scheme is to allocate edge IDs sequentially based on edge log, which results in random edge IDs in both the CSR and CSC, as both are involved in the computation.
% % However, we can only provide sequential edge ID in one of them. 
% We propose reordering the edge IDs in CSC to allocate them sequentially. That is, the in-neighbor list of vertex 0 was allocated edge IDs from 0 to N(0) (the length of in-neighbor list of vertex 0). Similarly, the in-neighbors of vertex 1 was assigned from N(0) to N(0)+N(1), and so on. 
% % Thus, edge IDs in CSR became random. 
% We were able to achieve this easily by writing a custom code inside $wrap\_graph()$ API of the kernel.

% We also have the option to regenerate COO format to provide it sequential edge IDs as per allocation in CSC. This was useful for SDDMM kernels to increase the parallelism. Hence, we are able to achieve sequential edge IDs in two of the graph formats, while prior works had sequential edge IDs only in COO, and not in CSR and CSC.

% \noindent \textbf{Kernel Fusion.}
% For GCN model, we observe that it performs tensor normalization by dividing the tensor elements with vertex degree. We fused this operation with the GCN's core kernel (gathering features of neighbors of a vertex to update the self). Kindly note that the order of normalization and gathering features changes in the backward computation compared to forward computation. Hence one must take care of this fact while fusing the kernel.

==> tex/new_added.tex <==
\section{New added sections} \label{sec.new}
\subsection{Research aspect}
Many existing works, [GNNadvisor, zhai, gespmm, ] mainly focus on optimizing the kernel implementation. (TODO GNNadvisor has a python model, zhai has a simulated GNN). However, based on our analysis, we are the first one to find that kernel implementation alone is not sufficient enough for system research to avoid mistakes and improve end-to-end DL training time.
The following sections will provide more details to support our findings. 
 
\subsubsection{End-to-end training is needed in GNN systems}


\textbf{Without end-to-end training, many implementation requirements are ignored by the researchers}
 
 
Different classes of GNN(GAT, GCN and GIN)
The GNN models can be classified into different classes based on their aggregation method. The GNN models which have unweighted sum aggregation are one class, such as GCN and GIN. The GNN models with the weighted sum aggregation method is another class, such as GAT, etc(todo we can cite more attention-based paper) Because of the aggregation difference, different types of GNN models have different system-level implementation requirements.  



Edge id indirection is needed, (Copy from 2d-snb)
As we mentioned in the background, Attention-based GNN models use attention(importance) scores to aggregate the neighbor values. Attention-based GNN models first generate the O(E) level attention score A. In the aggregation process, 

 Given a target node i, the model first fetches the attention score $A_{k}$ of its neighbors ($k \in N(v)$), then aggregate by sum$(A_{k} * H_{k})$ to updated the $H_{i}$. This process will be iterated until all nodes’ embedding is updated. This updated H will be used for the later computation. 

In the forward process, the kernel fetches the A by the normal graph order and performs the later computation, and saved it for the backward computation. 
In the backward process, the kernel needs to reload the saved A and fetch it again but in the reverser graph order. 
Here the problem comes, Since the graph is now reversed, the order of the edge list now is different than its order in the normal graph. If we still use the forward fetching order to fetch the A in the backward process, each attention score $W_{k}$ will be wrong. The incorrect fetched $W_{k}$ will cause a wrong backward computation, which corrupts the whole model training process.
While this  problem can also apply to compressed layers. E.g., in weight-pruned fully connected layers, as shown in Fig.~\ref{fig-prun}, the data is the dense matrix and the layers are sparse matrices.
To solve this problem, it is mandatory to maintain the edge indirection property so that  the kernel can fetch the correct $W_{k}$ in both the forward process and the backward process.

Zhai -- GAT problem
(copy from 2d-snb ended)
 
The corresponding DGL kernel of this computation is ‘gspmm’. To support this requirement, DGL provides an extra shuffle kernel to reorder the edge id list each time before fetching the edge score tensor. After that, DGL transposes the input tensor and uses the cusparse library to perform the computation. This extra shuffle kernel, transpose computation, and the system overhead time between them lead to extra time cost at the end-to-end training process. (todo find the line of code with shuffle + gspmm) 
If the requirement(above process) is not fully understood by researchers, even if they replaced the cusparse library with an optimized kernel, the overall end-to-end training process will not be optimized. 
Hardly do these previous papers discuss this edge id indirection requirement. Instead, Their kernel implementation can only support specific types of gspmm, such as GCN and GIN. 
 

Zhai’s work does not consider this requirement when implementing the kernel also. It fetches the edge tensor in sequence, this incorrect fetching will lead to the wrong aggregation result.
Although the integration between the kernel and the GNN model is correct, the overall simulated GNN has Some mistakes. (todo Not sure what this problem is: Input tensor and output send them as the same tensor)
Because of these mistakes, even if the simulated end-to-end training time shows improvement, this result is not trusted and cannot represent real-world GAT training. 
Gespmm forgets to consider edge id indirection also.

Therefore, if the researchers only focus on kernel implementation, it is likely for them to ignore some requirements and make some mistakes.
With an End-end training platform, it becomes easy to let researchers know that some extra requirements, such as edge id indirection property, needed to be taken care. With understanding this requirement, researchers are free to follow the DGL solution or propose their own solution. 


\textbf{Implement kernel only can cause end-end training accuracy problem}

Firstly, without end-to-end training, the kernel implementation may be incorrect.
One straightforward example is forgetting to meet some extra requirements we mentioned above(in the above section)
Secondly, even if the kernel implementation is correct, the overall training loop may be still wrong. For example, GNNadvisor implements it’s gspmm kernel alone correctly. But its experiment shows in (todo section ) show that it does not achieve correct accuracy. That is because it does not fuse the normalization computation with the gspmm kernel correctly for the backward process. In the backward process,  the fused kernel should do normalization first and then perform the aggregation.
(\todo zhai problem and gat)




To sum up, existing GNN system level optimization works, GNNadvisors, zhai, gespmm read the DGL code base to understand the requirement. ( need some reference email them) 
However, GNN model works, such as GCN, and GAT(these papers just provides the basic mechanism of the dense matrix) and GNN System works, such as DGL do not provide clear system-level requirement description. It is not guaranteed that all people can understand them correctly. Examples in the above section (todo list GNNadvisor, zhai, gespmm citation here) show that even researchers may ignore some requirements easily. 
 
Therefore, these requirements are very important in GNN systems but none of the Previous works explain them in the paper.  We are the first one to explain these requirements and illustrate their importance. We also state that with an end-to-end training platform to test the accuracy, these ignored requirements will be found. 

\subsubsection{A baseline is needed in GNN system area}


\textbf{End-to-end training time is controlled by overhead}

Our experiment in section (todo) shows that existing GNN systems, DGL, PyG have large overhead for the small data sets. To be more specific, the end-to-end training time is controlled by system overhead.
This large overhead has two negative effects. Firstly, since the work that implements most computation in cuda and c++ can avoid the system overhead and achieve huge end-to-end improvement, it is hard to measure the real effectiveness of performance improvement for these types of works. We do not know whether the improvement comes from the c++, cuda implementation, or the optimization techniques mentioned in these works(such as graph reordering, techniques to improve data locality, and better parallelism).

Secondly, the large overhead misleads the potential optimization directions for researchers.
That is because most researchers verify the effectiveness of their optimization techniques by performing an end-to-end training on small datasets.
In that case, the end-to-end training time will not change even if the kernel is optimized well, 
To solve this problem, GraphPy was optimized to achieve a small overhead so that the Kernel improvement can play more role in the end-to-end training. 

\textbf{Overhead neutralize the effectiveness of kernel improvement}
Besides the overhead on small datasets, framework overhead prohibits the improvement of the overall end-to-end training even if the kernel itself is well optimized. 
 
A straightforward example is DGL. DGL adopts the cusparse, an accelerated linear library optimized and provided by Nvidia over decades, as the core kernel for gspmm(mainly kernel used in GCN and GAT).
However, DGL’s gspmm kernel cannot achieve the same speed as cusparse. Instead, it has a 2 X, 3X slowdown compared with cusparse. (todo Test cuspare, and gspmm kernel in DGL to show the performace different in ogb dataset) 
That is because the gspmm in DGL is designed for both unweighted aggregation and weighted aggregation. It needs to apply one shuffle kernel each time before launching the cusparse to support edge id indirection(refer to next section). Moreover, since cusparse library can only accept column-level input, DGL needs to transpose the input tensor before using the cusparse library. These two more steps, shuffle, and transpose, cost some extra time. If the researchers just fuse these two steps together or remove the need for transpose for cusparese library and do not apply any optimization techniques, the end-to-end training time will improve a lot. 
 
But if the researchers do not understand these steps correctly, and design some optimized kernel to just replace the cusparse. Even if the optimized kernel is faster than cusparse, the end-to-end training time will not be improved. (todo not sure whether this DGL example is overhead or not)
 


(Todo Another example is the Gespmm, although its optimized kernel is faster than cusparse, after it integrated its kernel to DGL the overall training time does not have significant improvement. )



 
Our Experiment in section (todo), Figure (todo) also shows that even if our reference kernel gspmm is slower than cuspares, our GCN end-to-end training time achieves a (TODO) speedup compared to DGL among different datasets. 


(todo not sure Because of edge id indirection provided by our framework). Even if our kernel is slow alone, Our end to end training time still achieves huge speed up.
 
Therefore, Just focusing on the kernel implementation cannot lead to a good end-to-end performance. Moreover, since researchers study the kernels for more than 10 years, the new optimization mostly triggers an incremental improvement such as 10 percent - 15percent. From the above, we find that the end-to-end training time bottleneck comes from not only the kernel but also other parts.
 
Researchers need to understand not only just the kernel(The kernel here is different than the kernel in DGL, but not sure how to explain the difference) but also the other parts. This understanding can only be achieved by end-to-end testing. 

In that way, there is a need for an easily plugged-in platform to let researchers understand the roles of the kernels in the whole GNN training process. With a better understanding of the kernel role, researchers can implement the proper kernel which speeds up the overall training performance. 


\textbf{huge memory consumption causes problems}
As we know, DL needs to consume huge memory which will lead to a high energy cost. (citation to do takes 1-week energy of the whole city) Therefore, memory consumption becomes an important metric for DL systems. In this work, GraphPy provides a low memory consumption. It saves the number of E memory, which leads to 4 bits in GAT 1, and 12 bits in GAT3. For a graph with one billion edges, GraphPy saves 4 GB of memory. Moreover,  GraphPy can Save a number of vertex memory in features tensor compared to DG.L(todo add some details in interfaced design to explain).  In total, GraphPy can minimize 50% to 100 % memory consumption saving compared to DGL, which is a huge saving for energy costs. 
 
Another problem high memory consumption causes is graph splitting. For a large graph, the dataset cannot fit in a single GPU. Researchers need to split the large graph into multiple subgraphs and send them to multiple GPUs to do parallel training (todo citations). This multiple GPU setting makes the problem become more complex, and many concerns needed to be worried, such as how to synchronize the results, how to minimize the overhead, and how to optimize the communication between each split subgraph(Graph Partition is an NP-hard problem).
 
However, GraphPy provides low memory consumption to enable researchers to run GAT models on large datasets with a single GPU setting and avoid the complex multiple GPU problem settings. 


\textbf{Other problems with existing works}
Besides the overhead problem, there are other reasons that make the existing works cannot be used as a baseline.
As we mentioned in the above section, GNNadvisor has an accuracy problem in end-to-end training. It does not consider the edge id indirection at all so that it can only support a specific type of GNN model, such as GCN, GIN. It cannot work on another class of GNN, such as GAT.
Although zhai’s work supports GAT kernel, its kernel implementation is wrong because of the missing edge Id indirection. Moreover, Zhai’s work does not contain the end-to-end training loop. It is also impossible for researchers to implement a training loop by themselves because zhai’s work does not provide a backward process. 
Gespmm does not support edge indirection property either, which means that it cannot support GAT. 
PyG meets the OOM problem even for the median size data set. It also has a Large overhead for small datasets.
Therefore, none of the existing works can be treated as the baseline. 
There is a need for a Baseline in GNN systems, which is better than DGL in end-to-end training but does not include any novel opt techniques so that new optimization techniques can be added.

\textbf{Summary}
 
To sum up, wring the kernel alone is not enough. There is a need to provide a platform to let researchers really understand the kernel requirements and related topics.
 
To fix this gap, GraphPy focuses on interface design. By providing modular-based kernel, GraphPy
provides the opportunities and options system researchers can pursue which is not explored by the early framework.
 
To be more specific, the Kernel interface in GraphPy is not as simple as DGL expects. In the DGL, the core kernel for ‘gspmm’ is the cusparse kernel. To integrate with DGL, researchers can only implement new kernels to replace the cusparse. As we mentioned above, replacing cusparse cannot achieve end-to-end performance improvement.
However, GraphPy provides a more customized kernel interface so that researchers can decide whether they want to implement a new kernel that replaces all the above computations or just replace the cusparse. The optimized small overhead of GraphPy provides researchers the opportunity to check the effectiveness of the kernel in the end-to-end overall training.
(todo need to explain this part well. What is the difference between graphpy kernel and the DGL kernel? Not very precise What impact the overhead places here)


(todo Hardware evaluation. Or just kernel evaluation. (Possible for overhead analysis))



\subsection{Education aspect}
For education purposes, there are several educational attributes GraphPy provides.

\textbf{Just writing kernels in c++ or python is not enough}

The real-world GNN system[AWS, Azure, etc todo need citation] contains two aspects: c++/cuda based kernel implementation to provide fast speed computation and python-based wrapped kernel and GNN layers to let the data scientist customize their GNN models. 
 
 
 
 
 
 
The goal of the teaching is to let students understand both these two aspects.
 
Only teaching how to implement the kernel in c++/python is not enough. It is not just teaching students how to write the kernel and how to use pybind to wrap the kernel out in python.
Writing the kernel only cannot let students understand the exact requirement as we mentioned in the above research section. (todo cite the section number here) 
For example, GNNadvisor does not fuse the normalization and the computation kernel correctly in the backward process. But it is hard to explain this requirement to students on the kernel implementation. Only with an end-to-end system teaching, students will know this difficulty of kernel fusion. To be more specific, if we assign an assignment to let students fuse these kernels directly, students just implement the fused kernel without thinking of any requirement about this fusion process. 
But with an end-to-end system, the instructor can teach students these requirements and let them play with different kernel fusions and understand whether the requirement is satisfied or not from the accuracy. 
 
The existing platform does not provide an end-to-end system. They standford, berkely[need some citations] just provides pooling, softmax, batch normalization (not sure of convolutional layer) in the forward. Students still do not know how the backward process doing and how to use the wrapped kernel in an end-to-end training loop. 
 
It is hard for students to have a whole-picture view of how the GNN system works. With Graphpy, students can practice these steps and learn some practical tricky implementation techniques. And understand how each step works in an end-to-end training process.  This education training will help the students get a deep understanding of GNN systems, which will help them a lot in the future job market or academic research. 
 
Besides this, GraphPy also provides several educational attributes so that students can learn the GNN system easily.


\textbf{Easily plugged in kernel module}

In the GNN systems education teaching, there is a need to let the student write the kernel. However, this implementation process should be kernel focused only. That is because most students do not have enough background and time to explore the integration code and pybind wrapping technique.
GraphPy focuses on the interface design to provide the independent kernel module and auto-generated integration code to let students write the kernel easily and not need to learn the programming framework.


\textbf{Customized Python GNN layers}
Besides the kernel implementation, GraphPy wrappers the GAS kernel out in the python environment and provide the GNN model layers.
Students can modify them easily to learn the GNN models’ configurations and how the GNN model uses the GAS kernel.


\subsection{Graph system works cannot be extended to GNN}
Merril’s work handled the workload imbalance, which lead to a great performance improvement in spmv. However, it needs to preprocess the metadata first and use this metadata to do later things. These metadata structures cannot be passed to DL backends such as TF and Pytorch. (To do how to provide it cannot ). Many other works [citations] also rely on the preprocessed additional data structure.
 


\subsection{GraphPy can also work on unlabeled datasets}

For the unlabeled dataset, GraphPy can randomly generate the label for the training node id and test node id. With this synthetic label, these unlabeled datasets can be viewed as labeled dataset. 



==> tex/observation.tex <==
\section{Requirement Gathering/Design Goal analysis} \label{sec.obs}
In this section, we analyze the existing system level of work about GNN and discuss the several requirements for GNN framework that are suitable for both education and research. We first discuss many aspects a good educational/research framework should have and then introduce the motivation of our work. 


(\td  first section can come from the survey/ instructor and students)
\subsection{R1: required for end-to-end environment}
As an educational platform, it should have a clear top-down module end-to-end GNN environment. That is because the students/researchers need to fully understand the domain from many aspects. Especially when we consider the GNN ecosystem, it contains much more complex modules, such as GNN model workflow, HPC GNN kernel, etc, compared with traditional graph systems. Without the top-down view, it is hard to understand how each module works. 
For example, 
Students need to know the GNN model configurations before they dig down to the HPC backend. They also need to know the computation goals of each model layer.
Otherwise, it is hard to understand how to apply APIs based on the model configuration as well as understanding how SAG works in GNN system. 

Moreover, one paper mentioned(\td add graphpy) that many papers published on the top conference, such as OSDI, SC, PPoPP etc, misunderstood the HPC backend requirement during their kernel implementation without the end-to-end environment. Therefore, an end-to-end environment with an actual training loop and accuracy checking can help students/researchers a lot.


(\td add a survey about easy learning questions) 


\subsection{R2: easily plug in-out system architecture}
A second question for HPC backend implementation is: where to implement it?
Although modular-based system design is known by the community, many GNN systems, DGL, PyG, does not follow this requirement. Their library is complex and module-dependent, students need to modify many different files across many dependent modules when implementing the kernel. Moreover, it is normal for students/researchers to implement multiple versions of GNN kernels(eg, SpMM) based on different fundamental design trade-offs, such as thread scheduling, and data loading. The module-dependent design forbids productivity even more in this case. 




not torch c++, not easily for students to learn

\subsection{R3: auto-generated integration code}
Unlike traditional Graphpy analytic systems, an end-to-end GNN system is complex because it contains a couple of different models. Many corresponding integration codes are needed. However, it is unnecessary and hard to let students write such code. 



\subsection{R4: multiple purpose application use cases}
A good platform should not be limited to specific use cases. It should 
be extendable to other use-cases, such as compressed sparse models. 
The GNN-based system framework should not be a piece-by-piece work. 
(\td whether it is easy for the accelerator?)


\subsubsection{R5: extensible high-performance graph preparation}
Since Graphpy paper (\td cite graphpy paper) mentions that the GNN optimization techniques should be evaluated on large datasets because the evaluation time for small datasets represents the framework overhead instead of the kernel running time. However, existing works use the existing time-consuming package, such as scipy (\td not sure whether it is slow) to prepare the graph from raw text file. Other works, such as DGL even use its python-based (\td check not sure)graph creation module to create the graph structure. Those third-libraries graph creation module is time-consuming for large datasets, which slow down the kernel implementation and producibility since students verify its implementation. 


(\td not sure whether scipy fail(memory problem) for large dataset)
(\td we can also apply customer format for graph structure, but not know where to put)


\subsubsection{R5: version/DL backend independent}
The end-to-end GNN system needs to integrate with several existing third-party libraries, such as GPU toolkits, CUDA drivers,  and different DL backends.(TensorFlow, PyTorch, and Mxnet)
As a third-part library owned by industries, they are renewed, updated, and maintained periodly. Whether the newly released library affects the compilation of the end-to-end GNN systems becomes a problem. 
We realized many existing works(\td citations) have this version of conflict problems. For example, When we install and compile GNNadvisor code, we realize these GNN systems are pytorch version dependent. If the environment use the default newest pytorch or cuda toolkit, the compilation process will have errors. We need to roll back to some specific previous old versions, which is an easy job for students to handle.  

Moreover, these GNN systems GNN systems, such as Huang et al, GNNadviosr implement all their HPC backend and GNN-model integration code by fixed pytorch c++. This design limits their DL backend to pytorch only instead of other popular DL backends, such as Tensorflow and MxNet.
 

how to do tensor exachage, graph exchange, very detail but important,
memory management




==> tex/observation2.tex <==
%\section{GNN Training: Observation and Analysis} 
\section{Prior Works Analysis \& Recommendation} \label{sec.obs}
%Due to the involvement of edge-level tensors, the computations are more complex than the purely GCN model. 
%For graph storage, Class A does not require the presence of edge ID, while Class B does. For kernel computation, class A is simple and needs only gSpMMv, while class B needs gSpMMve, gSpMMe, and many variations of gSDDMM. 


\noindent \textbf{Taxonomy.}
Here we establish a taxonomy of classifying GNN models into broad categories. Each category is associated with two types of graph-related kernels~\cite{dgl2019} called \textit{gSpMM} (generalized sparse matrix dense matrix multiplication), and \textit{gSDDMM} (generalized sampled dense dense matrix multiplication).
%E.g., in weighted gSpMM kernel aggregates gathers all the received information a vertex and performs a specific \textit{reduce} function (e.g. sum, min, max, etc.) to aggregate them. 
gSpMM has many variations, including the weighted and unweighted versions, uses various reduction operations (e.g. sum, min, max, etc.).
% the same result as matrix operations, but provides option of many reduce operations in the gather phase. 
The gSDDMM kernel can be thought of as a derivation of edge-level tensors  either from vertex-level tensors or from a vertex-level tensor and an edge-level tensor. 
%E.g., summing the source and destination vertices features to derive edge-level tensor. 
It also has variations due to various operations (sum, division, etc.) that need to be performed.
%Despite the name similarity, gSpMM kernel is not truly SpMM, and so is the gSDDMM kernel. In SpMM (Y = AX), each row of A is multiplied with \textit{columns} of X, and is  summed;  while in gSPMM, the row values of A select the neighbor's feature (rows) of X, which are reduced (e.g., sum, min, max, etc.).

% We classify GNN models into different broader classes.
% We also classify main graph-related kernels in two categories~\cite{dgl2019}, called \textit{gSpMM} (generalized sparse matrix dense matrix multiplication), and \textit{gSDDMM} (generalized sampled dense dense matrix multiplication).



\noindent $\bullet$
\textbf{Class A: Vertex- + Edge- Level Tensors.}
The GNN models, such as GAT, RGAT, GaAN~\cite{gat18iclr, rgcn2018, zhang18}, etc.  use the weighted sum aggregation in its gSpMM, called \textbf{gSpMMve}, where the last two letters signify the input tensor types. The weight here represents the edge-level tensors that are trainable. We also need another gSpMM variant, called \textbf{gSpMMe}, and two variants of gSDDMM. In \textbf{gSDDMMvv}, the source and destination vertices' features are operated using the graph to generate edge-level tensors, while in \textbf{gSDDMMve}, vertex-level and edge-level tensors are accessed using the graph to arrive at the resultant edge-level tensor.
We use \textbf{gSpMMv\textit{eid}} in place of gSpMMv\textit{e} to emphasize explicit edge ID requirement. A similar convention is used for other kernels.

\noindent $\bullet$
\textbf{Class B: Only Vertex-Level Tensors.}
The GNN models such as GCN\cite{gcn17iclr} and GIN\cite{xu2019powerful}, use an unweighted sum to aggregate vertex-level neighbor features, Hence, it only needs vertex-level tensor, and not edge-level tensor, so no edge ID is needed in the graph storage. This kernel is called \textbf{gSpMMv}, a variant of gSpMM.
Another related kernel is \textit{normalization by degree} of vertex-level tensors, which is needed in GCN.
%A degree is the out-neighbor count of a vertex.


\noindent \textbf{Scope.}
Sampling-based GNN systems~\cite{kaler2022accelerating, yang2022gnnlab, waleffe2023mariusgnn, liu2021bgl,lin2020pagraph,song2022rethinking} 
remove the sparsity by sampling a fixed neighborhood count, such as only 10 neighbors per vertex. 
We do not consider them to have an in-depth discussion on graph (or sparse matrix) based kernels. We are rather inspired by this line of work, as papers have to show the impact of sampling by measuring overall accuracy.
%These works verify the correctness of their optimization by testing its accuracy among different datasets. We do not focus on this class, as measuring accuracy is a prerequisite that also avoids many issues that we discuss in the other two above classes. 
We also do not discuss distributed GNN systems~\cite{wang2021flexgraph,cai2021dgcl, md2021distgnn, zheng2020distdgl, p3gandhi2021,tripathy2020reducing, wang2021flexgraph} to focus on single GPU, whose performance and memory consumption is a very important factor for a distributed design.


The two GNN classes capture many variations of graph storage and kernel requirements. Hence we use them to analyze the GNN works and present some critical observations that motivate our work.
Datasets are discussed in \cref{sec.exp}, and experiments, if any, are run on an Nvidia A100 GPU.

\subsection{Training Accuracy Measurement} \label{sec.accuracy}
%We outline some issues that we have observed while studying a few works that have not measured accuracy  because either they do not have end-to-end model implementation or do not measure it.
% \noindent 
% \textbf{Missing Complete Model Implementation.}


%It's GCN model only has the 32.9\%, 14.2\%, 20.6\% test accuracy for cora, Pubmed and Citeseer datasets. However, the DGL achieve the 83.1\%. 76.5\%. 65.4\% for these datasets with the same model configuration. \td[Put it in a Table]. Table \ref{table-accu} shows this.
% \begin{table}[h]
% \small
% \vspace{-6pt}
% \caption{Accuracy between DGL and GNNAdvisor for GCN} % title of Table
% %\vspace{-6pt}
% \centering % used for centering table
% \begin{tabular}{|l| c cc|} 
%     \hline\hline 
%     Graph & Cora & PubMed & Citeseer\\ [0.5ex] % inserts table
%     %heading
%     \hline % inserts single horizontal line
%     GNNadvisor & 32.9\% &  14.2\% & 20.6\%    \\ 
%     DGL & 83.1\% & 76.5\% & 65.4\%    \\
%     % & 76.47 &  76.52 & & \\
%     \hline %inserts single line
% \end{tabular}
% \vspace{-6pt}
% \label{table-accu} % is used to refer this table in the text
% \end{table}

% Upon further code study, we notice various issues in prior works including the absence of complete code for their GNN model, such as missing backward computation and also suffering from some of the following critical issues.

%\noindent \textbf{Kernel Fusion Mistakes.}
%GNNAdvisor~\cite{wang2021gnnadvisor} does not fuse the normalization by degree kernel with the gSpMMv correctly in the backward computation. 
%\noindent \textbf{Invalid Kernel Fusion.}
%It is aptly clear that GNNadvisor trades off accuracy for performance gain without explicitly mentioning it.
We observe that many GNN systems targeting performance optimizations~\cite{huang2021understanding, wang2021gnnadvisor, fu2022tlpgnn, wu2021seastar, jangda2021accelerating, liang2020engn, zhang2021boostgcn, kim2022analyzing, yan2020hygcn} that implement their own GNN layers and kernel implementation have established a trend of not measuring training accuracy in their research papers, while many do not have an end-to-end model implementation. We analyze a few of them now. 
%Their prototype may be fine, but we argue that training accuracy measurements will avoid any such mistakes in the future.

Huang et al~\cite{huang2021understanding} and TLPGNN~\cite{fu2022tlpgnn} prototyped forward computation only, and hence we cannot measure their training accuracy. However, they keep one giant fused kernel for one GAT layer that avoids materializing the edge-level tensor which is a trainable model parameter. Their graphs do not keep edge ID which is needed for GAT training. 
Clearly, such optimizations require a feasibility study to derive backward computations, and whether they can avoid edge ID or any equivalent mechanism while achieving comparable accuracy without giving up the proposed optimization.

GNNAdvisor~\cite{wang2021gnnadvisor} implements a complete GCN model but does not mention the training accuracy in its paper; it drops by 14.8\% -- 24\% compared to DGL(see \cref{sec.exp}). The drop is attributed to two issues: (1) during backward, it calls normalization by degree after the gSpMMv in its fused kernel which must be called before the gSpMMv; 
%For GCN, the normalization by degree kernel is called after gSpMMv invocation in the forward computation. Hence during backward, the fused kernel should do normalization first and then the gSpMMv operation. While this error creates accuracy issues, the wrong kernel fusing results in performance gain, as we cannot fuse the backward normalization kernel in such an optimized way. 
(2) it used the model bias parameter in DGL evaluation but it has no bias support in its model layer, thus unknowingly trading off accuracy for performance without explicitly mentioning it.
%Unfortunately, GNNAdvisor~\cite{wang2021gnnadvisor} calls normalization after the gSpMMv during the backward computation. 
%\noindent \textbf{Missing Bias Parameter}.


% \begin{table}[t]
% \footnotesize
% \caption{Dataset showing accuracy for 2-layer Vanilla GCN that uses 16 as feature-length. \textbf{**}GNNAdvisor produced an invalid memory access error as observed by others~\cite{fu2022tlpgnn}.} % title of Table
% \vspace{-6pt}
% \centering % used for centering table
% \begin{tabular}{|l| r| r| r| r| r| } % centered columns (4 columns)
%     \hline\hline %inserts double horizontal lines
%       & Cora  & Citeseer  & PubMed & Reddit & OGB-Product\\ % inserts table
%     %heading
%     \hline % inserts single horizontal line
%     GNNAdvisor & 69.5\% & 40.9\% & 59.8\% & ** & **\\
%     DGL & 83.1\% &  65.4\% & 76.5\% &92.89\% & 69.75\%\\ 
%     \hline %inserts single line
% \end{tabular}
% \label{table-obs-accuracy} % is used to refer this table in the text
% % \vspace{-12pt}
% \end{table}

%From the above example, we find that by avoiding the measurements on accuracy, researchers commit errors in understanding the systems requirements by focusing on the forward computation only. Thus, it does not materialize the tensors that are needed as a state during back-propagation, while omitting crucial graph storage requirements. This off-course leads to wrong performance improvements.
 %some small mistakes such as misordering the kernel fusion step and forgetting to implement the bias corrupt the accuracy, but result in performance optimization. 


\noindent
 \textit{\textbf{Recommendation \#1}: Researchers and communities should enforce measuring training accuracy as it may help identify many issues during the prototyping phase and can be used to justify the proposed optimizations.} 
 %Focusing on the kernel fusion based on the forward computation alone, and then optimizing those kernels cannot advance the state-of-the-art in GNN system optimization unless we implement the complete GNN training and evaluate the accuracy.



%These works can be classified into two categories: (a) those that do not implement a complete model; and (b) others that do have complete model implementation but do not perform the training accuracy measurements. We present some examples of the mistakes that gain performance at the expense of accuracy. 

 
%There is a need for an end-to-end system that can verify the accuracy so that any system optimization can be evaluated correctly.

\subsection{Training Performance Measurement} \label{sec.performance}
%In \cref{sec.accuracy}, we noted above that performance improvement without accompanied accuracy measurements may lead us to justify some of the invalid optimizations. 
We now ignore whether accuracy is measured or not and focus on performance measurements to unearth more issues.
%of either complete GNN training, just one forward epoch, or only gSpMM kernel.
%We also ignore whether they do end-to-end training time measurements (e.g., by using 200 or more epochs that evaluate both the forward and backward computation) or just using just one epoch that focuses on forward computation.


\subsubsection{Smaller Dataset: Framework Overhead and Methodology}

% \noindent $\bullet$
% \textbf{Performance Measurement.}
%We now show the impact of exclusively using smaller datasets for GNN performance evaluation. 
%Many GNN systems that do have an end-to-end GNN workflow exclusively use the smaller datasets to test performance~\cite{wang2021gnnadvisor,gespmmsc2020} on top of two very popular existing GNN systems, DGL\cite{dgl2019}, and Pytorch-Geometric (PyG)~\cite{pytorchg2019}.
%\td discuss methodology.
We first present a new methodology to evaluate the framework overhead in GPU-based GNN systems. 

\vspace{-6pt}
\begin{equation}\label{eq-overhead}
\textit{Framework$\_$Overhead} = \sum_{k}\textit{$CPU$\_$Runtime$}
\end{equation}
\vspace{-6pt}

Eq.~\eqref{eq-overhead} defines the overall framework overhead, which is a sum of the time consumed by the CPU for each training epoch ($k$). %The $k$ represents the number of epochs in the training procedure. 
Kindly note that in the GNN system, GPU kernel invocation is asynchronous to the CPU, and it does not wait for the kernel execution to finish-- a practice followed by all GNN systems. Hence, measuring the time taken by each epoch without waiting for the kernels to finish execution roughly measures the time taken by all the Python and C++ code executed in the CPU. We can use this time to calculate the overhead. In this measurement, $k$ is set to [0, 200).
For smaller datasets, CUDA kernel run-time is in sub-milliseconds, hence the framework overhead masks the kernel run time as shown in 
Fig.~\ref{fig-obs-overhead} for many GNN models training in DGL and PyG.
%single-threaded CPU code (Python and C++) 

%DGL calls this \textit{framework overhead} when comparing against PyG. 
%in their paper.
%\footnote{\url{https://arxiv.org/pdf/1909.01315.pdf} accessed on 05 March, 2023} and calls it \textit{framework overhead}.
%Hence, the end-to-end training time is dominated by the single-threaded CPU code (Python and C++), and not by the kernel run-time on GPU as the kernels are executed asynchronously with respect to CPU code which masks the kernel run time. Therefore, exclusively relying on smaller datasets may not be sufficient to measure performance gain. 
%Without understanding this fact, some researchers have made mistakes in analyzing their performance benefits. 
%when they show better or equal performance than DGL and PyG.

%\textbf{Firstly},  
%e.g., GNNAdvisor~\cite{wang2021gnnadvisor}, TLPGNN~\cite{fu2022tlpgnn}, and Huang et al~\cite{huang2021understanding} keep the complete layer information in C++.
GNNAdvisor exclusively relied on smaller datasets for performance evaluations. But it uses the PyTorch plugin and moved GNN layer code from Python to C++, resulting in less overhead compared to DGL. 
%Thus, it avoids executing Python code and framework overhead of DGL. 
So, if it is really faster than DGL remains unknown.
%Similarly, many other GNN systems~\cite{wang2021gnnadvisor,huang2021understanding,wu2021seastar,fu2022tlpgnn} have been developed without using DGL or PyG, while also writing model layers in C++.
%\textbf{Secondly,} 
On the other hand, GE-SpMM~\cite{gespmmsc2020}, which is integrated into DGL, shows hardly any performance improvement for vanilla GCN (hidden feature length as 16) for smaller datasets on which it relied exclusively in its paper. But it wrongly attributes this observation to the number of prediction classes not being a multiple of 32.

%However, we argue that the observation is related to the framework overhead of DGL. %Therefore, they cannot perform better than DGL for smaller datasets. In that case, the end-to-end training time will not change even if the kernel is optimized well.

%Table~\ref{table-motivation-overhead} clearly identify that irrespective of the better kernel design, the system is simply performing better than DGL due to lower overhead. 
%since the work that implements most computation in cuda and C++ can avoid the system overhead and achieve huge end-to-end improvement, it is hard to measure the real effectiveness of performance improvement for these types of works. 

%Clearly, We cannot know whether the improvement is possible due to the proposed systems techniques, such as graph reordering, techniques to improve data locality, and better parallelism. 

% \begin{table}[t]
% \small
% %\vspace{-6pt}
% \caption{\small Framework overhead and training time (in Seconds) of both DGL and PyG for GCN model training for 200 epochs} % title of Table
% \vspace{-6pt}
% \centering % used for centering table
% \begin{tabular}{|l| r|r |r|r|r|r|} 
%     \hline\hline 
%     Graph  & \multicolumn{2}{|c|}{DGL} & \multicolumn{2}{c|}{PyG}\\ % inserts table
%     %heading
%     \cline{2-5}
%     Dataset & Traning & Overhead (\%) &  Training & Overhead (\%) \\
%  %           & Time     &              &     Time &  \\
%     \hline % inserts single horizontal line    
%  %   Cora & 1.35 & 1.34(99.48) &0.98 & 0.97(99.28) \\ 
%  %   Citeseer & 1.51 & 1.50(99.27) &1.05& 1.04(99.23)\\
%     PubMed& 1.48 & 1.47(99.32) &  1.20 & 1.19(99.33) \\   
%     % & 76.47 &  76.52 & & \\
%     \hline %inserts single line
% \end{tabular}
% %\vspace{-6pt}
% \label{table-obs-overhead} % is used to refer this table in the text
% \end{table}



\begin{figure}[t]
  \includegraphics[scale= 0.42]{exp/overhead_obs.pdf}
   \vspace{-18pt}
  \caption{\small Training time and framework overhead of both DGL and PyG for GNN models training for 200 epochs.}
  \label{fig-obs-overhead}
%\vspace{-8pt}
\end{figure}





% \begin{table}[h]
% \small
% \vspace{-6pt}
% \caption{Framework Overhead of DGL GCN model (in Seconds)} % title of Table
% \vspace{-6pt}
% \centering % used for centering table
% \begin{tabular}{|l| c cc|} 
%     \hline\hline 
%     Graph & Traning & Total & Percentage  \\ [0.5ex] % inserts table
%     Dataset & Time & Overhead  & (\%)  \\
%     %heading
%     \hline % inserts single horizontal line
% %    Cora & 1.347 &  1.340& 99.480  \\ 
% %    Citeseer & 1.510 & 1.499 & 99.272 \\
%     PubMed & 1.480 & 1.470 & 99.324  \\
%     % & 76.47 &  76.52 & & \\
%     \hline %inserts single line
% \end{tabular}
% \vspace{-6pt}
% \label{table-motivation-overhead} % is used to refer this table in the text
% \end{table}




\noindent
\textit{\textbf{Recommendation \#2:} 
%The large framework overhead misleads researchers when they verify the effectiveness of their optimization techniques on smaller datasets only. 
To negate the impact of overhead, end-to-end performance measurements should never be limited to smaller datasets only.} 
%Hence, any optimization technique may show up as better performing, without knowing whether the system techniques are really beneficial.




% \begin{table}[t]
% \small
% %\vspace{-6pt}
% \caption{\small Memory Consumption (in MB) when running GNN training. (Lower is better).} % title of Table
% \vspace{-6pt}
% \centering % used for centering table
% \begin{tabular}{|l| r|r |r|r|r|r|} 
%     \hline\hline 
%     Graph  & \multicolumn{2}{|c|}{GCN} & \multicolumn{2}{c|}{GAT-1} & \multicolumn{2}{c|}{GAT-3}\\ % inserts table
%     %heading
%     \cline{2-7}
%     Dataset & DGL & PyG & DGL & PyG & DGL & PyG\\
%     \hline % inserts single horizontal line
% %    Cora & 1,719 & 1,349   & 1,719 &1,375 &&\\ 
% %    PubMed & 1,767 & 1,395  &1809& 1,503 && \\
% %    Citeseer& 1,697&1,381   & 1,759 &1,409 &&\\ 
%     Reddit & 23,237&OOM & 30,395 & OOM  & OOM&OOM\\
%  %   OGB-Pr & 25,551 &OOM & 20,789 & OOM  &32,285& OOM\\
%     % & 76.47 &  76.52 & & \\
%     \hline %inserts single line
% \end{tabular}
% %\vspace{-6pt}
% \label{table-obs-memory} % is used to refer this table in the text
% \end{table}

\subsubsection{Larger Dataset}
We explain now that we have a limited choice (DGL) as an end-to-end baseline for performance comparison.  
For \textbf{ Class A}, Huang et al and TLPGNN both have focused on forward computation only (\cref{sec.accuracy}). We explain the issue with FeatGraph in \cref{sec.dgl}, while others have not focused on this class of GNN. 
%Due to frequent out-of-memory PyG is not a good baseline for larger dataset. 
For \textit{Class B GNN}, GNNAdvisor that evaluates exclusively using smaller datasets faced illegal CUDA memory access  on Reddit, which is also observed by others~\cite{fu2022tlpgnn}. 
%We were able to run its gSpMMv kernel (after commenting normalization and other codes). Table~\ref{table-kernel-time} shows that it performs worse than DGL for both datasets, which we explore in \cref{sec.exp}. Similarly, 
FuseGNN~\cite{chen2020fusegnn} reports that it is slower than DGL for its only larger dataset of Reddit. PCGCN~\cite{tian2020pcgcn} does provide an accuracy metric, but the authors have not open-sourced it.
We have explored many other systems (see \cref{sec.exp} for such systems), though we could not run them end-to-end due to issues mentioned in this section and in \cref{sec.dgl}.

This makes DGL and PyG only end-to-end baselines. However, PyG cannot run any GNN model on Reddit which is also shown by
prior works~\cite{chen2020fusegnn,huang2021understanding}. 
Kindly note that our result used its original design of using COO format and torch-scatter as its CUDA kernel that materializes message passing at edge-level resulting in out-of-memory. Its latest release
%\footnote{\url{https://pytorch-geometric.readthedocs.io/en/latest/notes/sparse_tensor.html}}  
uses CSR format and PyTorch for its back-end, which internally uses CuSparse ({https://github.com/pytorch/pytorch/issues/60854}), 
 which we evaluate extensively through DGL and separately.
%A natural question is whether we can test various GNN models end-to-end on larger datasets.
Further, DGL also consumes significantly higher memory as shown in 
Table~\ref{table-obs-memory} for Reddit. DGL cannot train a 3-head GAT model even in the A100 GPU with 40 GB of memory.
High memory consumption does not allow DGL to run Reddit at all on the older generation of GPUs, such as Nvidia GTX 1080 Ti, and Titan V. We explore the reasons behind its memory consumption in \cref{sec.dgl}.



%\footnote{\url{https://ogb.stanford.edu/docs/leader_nodeprop/##ogbn-products} shows that PyG can run on OGB-product, however, they use data sampling.}. 


\noindent
\textit{\textbf{Recommendation \#3:}}
\textit{Memory consumption is a very important factor in deep learning and should be analyzed with the same zeal as the performance, otherwise, we will continue to have limited choices for baseline systems to evaluate performance on larger datasets. }
%due to frequent out-of-memory, missing end-to-end systems, and other issues. For class A GNN models, we require access to the latest GPU, otherwise, have to rely on smaller datasets.}

\vspace{2pt}
\noindent \textbf{Clarification.}
The evaluation presented in this section is not related to the reproduction of the results of the prior works. 
% We indeed see similar results.
The points raised in this section (\cref{sec.obs}) are based on our interpretation of those results and our additional evaluations. 
%Our recommendation is to show training accuracy and measure performance on larger datasets.
%that show that these result are not practical to GNN systems, such as missing measuring the accuracy.

% The point we raise here is based on the interpretation of those and additional evaluations of closely related works while generalizing the observation of not measuring training accuracy.

\begin{table}[t]
\small
%\vspace{-6pt}
\caption{\small Memory Consumption (in MB) when running GNN training on DGL. PyG always runs out of memory (Lower is better).} % title of Table
\vspace{-6pt}
\centering % used for centering table
\begin{tabular}{|l| r|r |r|r|r|r|} 
    \hline\hline 
    %heading
  %  \cline{2-7}
    Graph Dataset & GCN & GIN & GAT-1 & GAT-3 \\
    \hline % inserts single horizontal line
%    Cora & 1,719 & 1,349   & 1,719 &1,375 &&\\ 
%    PubMed & 1,767 & 1,395  &1809& 1,503 && \\
%    Citeseer& 1,697&1,381   & 1,759 &1,409 &&\\ 
    Reddit & 23,237& 23,737 & 30,395 & OOM  \\
    %OGB-Pr & 25,551 &OOM & 20,789 & OOM  &32,285& OOM\\
    % & 76.47 &  76.52 & & \\
    \hline %inserts single line
\end{tabular}
%\vspace{-6pt}
\label{table-obs-memory} % is used to refer this table in the text
\end{table}


%The conclusion is that relying exclusively on smaller datasets misleads performance results. Further, the absence of training accuracy measurement or forward-only systems cannot fully justify the proposed system optimizations till training accuracy is shown. However, we have fewer baselines for future comparisons on larger datasets for Class A and B end-to-end GNN models. 


% \begin{table}[h]
% \footnotesize
% %\vspace{-6pt}
% \caption{\small Framework Overhead of both DGL and PyG for GCN model (in Seconds)} % title of Table
% \vspace{-6pt}
% \centering % used for centering table
% \begin{tabular}{|l| r|r |r|r|r|r|} 
%     \hline\hline 
%     Graph  & \multicolumn{3}{|c|}{DGL} & \multicolumn{3}{c|}{PyG} \\ % inserts table
%     %heading
%     \cline{2-7}    
%     Dataset & Traning & Total & Percentage & Traning & Total & Percentage\\
%       & Time & Overhead & (\%) & Time & Overhead & (\%)\\
%     \hline % inserts single horizontal line
% %    Cora & 1,719 & 1,349   & 1,719 &1,375 &&\\ 
% %    PubMed & 1,767 & 1,395  &1809& 1,503 && \\
% %    Citeseer& 1,697&1,381   & 1,759 &1,409 &&\\ 
%     Cora & 1.35 &0  & 99.48 & 0.98  & 0&99.28\\
%     Citeseer & 1.51 &0 & 99.27 & 1.05  &0& 99.23\\
%     PubMed & 1.48 &0 & 99.32 & 1.20  &0& 99.33\\
%     % & 76.47 &  76.52 & & \\
%     \hline %inserts single line
% \end{tabular}
% \vspace{-6pt}
% \label{table-overhead_merge} % is used to refer this table in the text
% \end{table}



% \begin{table}[h]
% \small
% \vspace{-6pt}
% \caption{Framework Overhead of PyG (in Seconds)} % title of Table
% \vspace{-6pt}
% \centering % used for centering table
% \begin{tabular}{|l| c cc|} 
%     \hline\hline 
%     Graph & Traning & Total & Percentage \\ [0.5ex] % inserts table
%     Dataset & Time & Overhead  & (\%)  \\
%     %heading
%     \hline % inserts single horizontal line
%     Cora & 0.976 &  0.969 & 99.283   \\ 
%     Citeseer & 1.046 & 1.038 & 99.235  \\
%     PubMed & 1.204 & 1.196 & 99.336  \\
%     % & 76.47 &  76.52 & & \\
%     \hline %inserts single line
% \end{tabular}
% \vspace{-6pt}
% \label{table-Pyg} % is used to refer this table in the text
% \end{table}

% Interestingly, the huge memory consumption for DGL is introduced due to the requirement mismatch handling (points \#1, \#2, and \#3) when using CuSparse kernels. The additional transpose (\#2) requires huge memory equal to $|V|*feature-length$, while eshuffle requires $|E|$ additional memory for each gSpMM kernel. These are huge memory requirements. 
% For PyG, it expects its graph in COO format, which materializes the intermediate  messages that are passed from one vertex to another. Hence, it consumes a huge amount of memory, and cannot run any large graphs.

% Moreover, large memory overhead may prohibit researchers to run the GNN training in large datasets or on complex models such as GAT. Such high memory overhead may discourage researchers to evaluate end-to-end GNN training on larger datasets on a single GPU, and hence likely to be misled by the performance gain on smaller datasets or through other means. 

%We believe that this is also one of the reasons that many researchers focused on smaller dataset evaluation only in a single GPU, which led to the wrong conclusion about performance benefits. However, huge memory consumption still discourages a lot of researchers that have access to slightly older GPUs,   and we need to encourage them as well for the advancement of systems research in this important field.

%If the researchers want to test the GNN models in large datasets, Researchers need to split the large graph into multiple subgraphs and send them to multiple GPUs to do parallel training (\td citations). This multiple GPU setting makes the problem become more complex, and many concerns needed to be worried, such as how to synchronize the results, how to minimize the overhead, and how to optimize the communication between each split subgraph(Graph Partition is an NP-hard problem).



% \subsection{Requirement Understanding Issues}
% It is clear from the examples presented earlier that system optimization becomes invalid if system requirements are not understood correctly. We now present some additional examples tailored toward missed optimization opportunities due to the absence of an in-depth analysis of the system requirements.

% \noindent \textbf{Requirement Mismatch and Its Overhead.}
% We take the example of DGL to demonstrate some overheads introduced due to the usage of CuSparse as the underlying library for kernel implementations. CuSparse has been developed more than a decade back when GNN was not known. So, it is obvious that it suffers from the requirement mismatch that we present next. 


% \noindent
% \textbf{\#1. Dummy Edge-Level Tensor (GCN Only):} GCN performs unweighted aggregation, and hence DGL has to pass a default edge-level tensor, whose value is 1.0 for each edge, to call gSpMM of CuSparse requiring additional memory and computation. 
% %\noindent
% \textbf{\#2. Two Additional Transpose}: The vertex-level tensor of CuSparse gSpMM expects a column-major layout whereas the PyTorch tensor is row-major. Hence, DGL invokes two additional transposes of the vertex-level tensors (\textit{implicit} kernels) for the input and output, which consumes additional memory and computation.

% \noindent
% \textbf{\#3. eShuffle (GAT Only):} The CuSparse gSpMMve does not support edge ID in its graph storage, therefore, the edge-level tensor is first shuffled by the edge ID that is stored in DGL before calling gSpMMve. 

% \noindent
% \textbf{\#4. No Support for edge-level vector features (Multi-head GAT Only).} In multi-head GAT,  the edge features are a vector for each edge, which is not supported by CuSparse gSpMMve. Further, it requires eShuffle support. 
% %hence DGL has to call gSpMMve kernel multiple times just to handle different dimensions of edge-level features, with same set of vertex-level tensors. 




% \noindent \textbf{Performance Implication.}
% Table~\ref{table-kernel-time} shows gSpMM run-time for DGL and CuSparse. DGL introduces a slowdown up to 1.64$\times$ over CuSparse due to requirement mismatch overhead. We also plot the eShuffle time for the scalar edge feature. For Reddit, which has a smaller vertex count and a much larger edge count, the eShuffle time is almost equal to gSpMMve time, as the transposition of vertex-level tensor (not measured) is small. For OGB-Product, the eShuffle time is significant.
 
% Interestingly, many new GNN systems are still focusing on optimizing CuSparse gSpMMve equivalent kernel in the garb of GNN use cases rather than designing new kernels that are appropriate for GNNs. This is specifically true for systems that integrate with DGL, such as GE-SpMM~\cite{featgraphsc20} and FeatGraph~\cite{featgraphsc20} whose gSpMMve implementations do not support edge ID inside their kernel, and hence eShuffle is still needed as a separate kernel that will materialize one additional edge-level tensor. Hence, optimizing gSpMMve alone will have a lesser impact on end-to-end training as the scope of gSpMMve improvements are small as this kernel has already been optimized by many works over the last many years.   

% Such works neither provide vector features for edges in their gSpMMve nor even talk about gSpMMe kernel. Off-course, such works have proposed a newer gSpMMv kernel and avoided transpose, but do not offer normalization by degree inside it.


% % \noindent
% % \textit{\textbf{Observation\#3:} It is clear that focusing on existing sparse kernels alone brings limited performance optimization, and hence end-to-end understanding is needed to fully optimize the system.}

% \noindent
% \textit{\textbf{Observation\#3:} It is clear that optimizing the sparse kernels based on CuSparse definition alone brings limited performance optimization because there is a large gap between the GNN requirements and the kernels offered by CuSparse. }


%Clearly, if the requirements are not understood exactly, then integration of better kernel design may not be the one contributing to the performance improvements. This is because researchers might just remove the need of mismatch of the requirement that may be the major performance contributing factor. 

%fuse these two steps together or remove the need for transpose for cusparese library and do not apply any optimization techniques, the end-to-end training time will improve a lot. But if the researchers do not understand these steps correctly, and design some optimized kernel to just replace the CuSparse. Even if the optimized kernel is faster than CuSparse, we lose many other opportunities for optimizations. the end-to-end training time will not be improved. (\td not sure whether this DGL example is overhead or not)


%The above observation is a general problem because GNN system researchers mainly focus on describing the systems technique for better kernel implementation, while accuracy evaluation as well as evaluation on diverse datasets, such as large datasets are not thoroughly evaluated and understood. This sometimes cannot lead to good end-to-end training performance or performance improvement can only be attributed to factors outside of the systems technique of the paper. 


% Besides the overhead problem, there are other reasons that make the existing works cannot be used as a baseline.
% As we mentioned in the above section, GNNadvisor has an accuracy problem in end-to-end training. It does not consider the edge id indirection at all so that it can only support a specific type of GNN model, such as GCN, GIN. It cannot work on another class of GNN, such as GAT.
% Although zhai’s work supports GAT kernel, its kernel implementation is wrong because of the missing edge Id indirection. Moreover, Zhai’s work does not contain the end-to-end training loop. It is also impossible for researchers to implement a training loop by themselves because zhai’s work does not provide a backward process. 
% Gespmm does not support edge indirection property either, which means that it cannot support GAT. 
% PyG meets the OOM problem even for the median size data set. It also has a Large overhead for small datasets.
% Therefore, none of the existing works can be treated as the baseline. 
% There is a need for a Baseline in GNN systems, which is better than DGL in end-to-end training but does not include any novel opt techniques so that new optimization techniques can be added.


% Our measurements in Table \ref{table-exp-memory} show that many current GNN systems show out-of-memory conditions frequently on even slightly larger dataset in  single GPU setup. 
% Reddit graph, which has less than 230 million edges, can not be trained on A100 GPU which has 40 GB memory by PyG, GNNadvisor on any of their supported models. DGL cannot run a slightly complex GAT model, while it still consumes way more than 16 GB memory for GCN, and a simple GAT model. Hence, it is unsuitable on low- and mid-grade GPUs that has small memory, such as Nvidia GTX 1080 Ti.
% Hence, many prior GNN systems have only demonstrated smaller dataset for performance, which then are affected due to framework overheads that we discuss shortly. 
% Moreover, many works that do evaluate larger dataset have only focused on kernel benchmarking, but has many issues. 

 
% We investigate if end-to-end training performance comparison on smaller dataset can really rank systems based on their kernel performance.
% Table~\ref{table-motivation-overhead} shows overhead for GCN on two smaller datasets of Cora and Pubmed in an A100 Nvidia GPU that includes the time taken by rest of the  Python and C++ code but not kernel time; as well as total training time. The methodology and dataset are described in \cref{sec.exp-gnn.time}. It is very clear from this table that the total training time for Pubmed actually does not depend on the kernel time, as total training time is almost equal to the overhead time. Hence, any optimization of the gSpMM kernel will not show up if using DGL to prototype kernels. However, many systems that use PyTorch's plugin approach to prototype GNN on this dataset shows huge performance improvement compared to DGL. Hence, how can we be sure if the performance improvement is purely due to better kernel implementation and not due to difference in the overhead, when we are not able to evaluate larger dataset. 


% \textbf{Summary}
 
% To sum up, wring the kernel alone is not enough. There is a need to provide a platform to let researchers really understand the kernel requirements and related topics.





   

==> tex/old_usecase.tex <==

\section{Old Use-Cases} \label{sec.extend}
There is always a need to write new layers and kernels either for research or education. 
%The focus on critical interfaces design, enabling plug-and-play architecture, 


\subsection{Research}
%keeping the {\graphpy-Kernel} independent of DL framework, light-weight due to available graph in CSR/CSC format, and 
% There are many factors that make {\graphpy} ideal for research prototype, specifically in graph domain. While \textit{productivity} remains an important factor that is achieved using generation of critical boilerplate code, and outsourcing of graph storage to {\graphpy-SM}; \textit{reusability} of Kernel code across many DL frameworks through automatic integration make {\graphpy} an ideal platform for developing re-usable kernel code.
%reusability of  research and education in graph data science. Further, the interfaces designed around tensor exchange are generic enough to use {\graphpy} in other DL use-cases and not just graphs. 
% Further, \textit{modularity} offerings of {\graphpy} ensures that unrelated use-cases can be housed in different modules, rather than following the monolithic approach of prior works,  yet  those modules can be combined with the benefit of flexibility and for variety of use-cases. Because of such reasons, {\graphpy} is able to support many isolated sparsity use-cases including sparse data for deep learning, sparse tensor for deep learning models which can be modeled using graph, as well as traditional graph data science use-cases. We have reference implementation for the same to demonstrate that it is possible.

% % Hence a third party module can easily implement those missing functionalities without writing the boilerplate code and use zero-copy data-sharing for graph and tensor both. 
% % %Anytime, there is a new release of DL framework, the plugin requires re-compilation. Worst, they are not distributed along with main binaries, but are highly depended on each version of their release.
% % Thus all the instances of {\graphpy-Kernel} module remains reasonably independent as far as development complexity is concerned. This makes it easy for learners to focus on system implementation to learn the system side of graph data science as the Python model code and interfaces remain same. 
% % On the other hand, advanced learners can write end-to-end model, including the logic to handle its backward computation, and kernel code utilizing the interfaces and DSL. This way, they can better understand the concept of model development, the role of backward computation and kernel in the overall DL workflow. 


% %Mobile app development has seen tremendous use-cases, because of well thought interfaces. 
% % Relying on DLPack tensor, and not asking for memory allocation/deallocation inside the GraphPY-Kernel makes the kernel development free from any limitation or additional works of third party tensor library. 



% %The novel design of {\graphpy} makes it becomes a general framework that can support multiple use cases easily. For the data level sparsity, although we highlight {\graphpy} can handle sparse data, it can handle dense data as well. Moreover, {\graphpy} also supports model level sparsity, which is not supported by existing works. 


%\subsubsection{Sparse Data}



\subsubsection{Sparse Data}  \label{sec.gnn-background}
Graph convolution network~\cite{gcn17iclr}(GCN), graph attention network~\cite{gat18iclr}(GAT), GIN~\cite{xu2019powerful}, GGNN~\cite{gatedgraph2017}, GaAN~\cite{zhang2018gaan} etc. are collectively called \textit{graph neural networks} (GNN) that specialize deep learning on graph data.
%The DL frameworks do not yet support sparse operations efficiently. Sensing the gap, a number of GNN frameworks were proposed recently, such as DGL~\cite{dgl2019}, NeuGraph~\cite{neugraph19atc}, AliGraph~\cite{yang2019aligraph}, Pytorch-Geomertric~\cite{pytorchg2019}, etc.
%GNNs ~\cite{gcn17iclr,gat18iclr, xu2019powerful,gatedgraph2017} are frameworks for representation learning on sparse data or graphs. 
%The forward computation uses a series of sSpMM and gSDDMM kernels. 
The trainable tensors in such GNNs can be at vertex-level ($X$ and $Y$); and edge-level ($W_e$ as attention score in GAT and GaAN. 
%and can be a vector as in case of multi-head attention. 
%In GAS forward, $W_e$ is calculated using a series of gSDDMM kernel, that takes various reduce operations of sum, min, max, etc in forward computation. Its one input tensor is a vertex-level, while the second input tensor can be either vertex-level or edge-level tensor. $W_e$ is used as edge weights (scalar or vector) in the gSpMM to calculate vertex-level tensor Y. In GCN, $W_{e}$ is absent in (unweighted) gSpMM. In its another variant, gSpMM only accepts an edge-level tensor to calcuate the output Y, and accepts various reduce operations.
Backward computation also invokes variations of gSpMM, and gSDDMM, and requires accessing the tensors produced during forward computation ($W_{e}$, $X$ and $Y$). Hence, they are saved as \textit{states}, as shown in Fig.~\ref{fig-forward}. 
Since, backward computation happens on the inverse graph (CSR), as opposed to using CSC during forward computation; the CSR and CSC  must share the same copy of the state tensors. This is handled by the vertex ID indirection for vertex-level tensors ($X$, $Y$), which is already present in the graph storage. However, for edge-level tensors ($W_{e}$), graph storage needs to introduce \textit{edge ID indirection} (Fig.~\ref{fig-format}). 
%For completeness, some gSDDMM kernel during backward does not need inverse graph.

\begin{figure}[t]
  \includegraphics[scale= 0.64]{result/gnn-crop.pdf}
 \vspace{-12pt}
  \caption{\small GNN Forward and backward mode: X and Y are intermediate features, and $W_e$ is the model parameter of the layer, e.g. attention score in case of GAT. X, Y and $W_e$ tensors are \textit{state}, as it is used in forward and backward both. $A$ and $A^T$ are graph and its inverse.}
  \label{fig-forward}
%   \vspace{-12pt}
\end{figure}





\noindent \textbf{Why end-to-end GNN system needed?}
This edge ID requirement for attention-based GNNs differentiates DL sparse kernels from prior works in sparse linear algebra and graph analytics.
Hence, if one only focuses on kernel optimizations without thinking of evaluating accuracy on an end-to-end training loop, it is very likely to omit edge ID requirements~\cite{huang2021understanding}. 
%Rather, we have noticed that a GNN performance improvement work~\cite{huang2021understanding} does not store edge ID in their graph storage for GAT. 
Such errors could have been easily found if the work integrated their kernel in a training loop, and measured the accuracy. Similarly, another GCN work~\cite{GNNAdvisor} did not use bias in its model. Both of these works are likely to over state the performance benefits in the absence of accuracy measurements due to omission of crucial requirements.

Therefore, instead of focusing on kernel optimization only, measuring training accuracy is needed, that can act as a feedback to researchers about correct implementation. 
%Further, such a framework will also show the true impact of better kernel design on the end-to-end training performance. 
%To satisfy this need, We propose an end-end system {\graphpy} that let researchers write the new kernel easily. The Independent and Auto-Integrated Kernel (\cref{sec.science.auto}) and graph storage GraphPy-SM (\cref{sec.engg}) make {\graphpy} becomes \textit{productivity}, \textit{reusability} and \textit{modularity}. which is an ideal end-end prototype for GNN system research.
Rather many techniques proposed by graph analytics systems~\cite{kyrola2012graphchi,roy2013x,nguyen2013lightweight,liu2017graphene,powerlyra2015eurosys,gstore, zheng2015flashgraph,mosiacEuroSys17, roy2015chaos, han2013turbograph, kumar2017falcon, zhu2015gridgraph,hong2012green, wu2015g, ai2017squeezing, zhu2016gemini,liu2015enterprise}, such as using specifically tailored data layout~\cite{zhang2015numa,gstore,libgraplus15DB}, graph-aware compression~\cite{libgraplus15DB,gstore}, fine-grained and workload-aware parallelism~\cite{liu2015enterprise,wang2015gunrock}, graph re-ordering~\cite{gorder16sigmod,rabbit16ipdps}, graph partitioning, etc. for CPUs and GPUs, could also be evaluated easily for GNN use-cases, if a platform can offer easier integration of system works to DL workflow.

\subsubsection{Support for Sparse Tensors}
Recent work on model compression, such as weight pruning~\cite{han2015learning,han2016iclr}, removes significant number of parameters from specific layers (e.g. fully connected layer) to achieve model/layer compression as shown in Fig.~\ref{fig-pruning}. Such techniques have enabled a number of large models to be deployed in resource-constrained devices. However, before their deployment, re-training is required to fine-tune their parameters. 

%\noindent \textbf{Different Sparsity.}
The sparsity in the model layers is \textit{different} from data sparsity. E.g., the sparse connectivity here requires bipartite graph, where the number of source and destination vertices sets are different. Further, multiple layers can be sparse in this case with each layer having its own bipartite graph. Also, the graph object is part of sparse tensor, and not sparse data. Finally, the computation in this case is more like traditional sparse linear algebra, i.e. SpMM and SDDMM. On a different note, edge ID is still needed, if it involves edge-level tensors as in sparsely connected layers (Fig.~\ref{fig-pruning}).

% Fig.~\ref{fig-pruning} shows the weight pruning~\cite{han2015learning,han2016iclr} intuition for a fully connected layer, where the resultant layer becomes sparsely connected, can easily be represented as graph. 
Re-training, like training process, is mostly done using in-memory system today. Hence prior works that have used ad hoc methods to re-train such models, such as using a bitmask matrix 
% the punned layer is now a combination of a dense parameter matrix and a bitmask matrix.  it 
will still use the dense linear algebra of DL frameworks to perform re-training, and uses the bitmask to only filter out the computation results on pruned weights. Clearly, this re-training still uses same memory consumption, and performs almost the same number of computation that would have been done using the original model.

\begin{figure}[t]
  \includegraphics[scale= 0.5]{result/pruning-crop.pdf}
 \vspace{-6pt}
  \caption{\small Model compression here converted two fully connected layers to sparsely connected layers after weight pruning, and can now be represented using bipartite graphs.}
  \label{fig-pruning}
 \vspace{-6pt}
\end{figure}




However, if we can model the sparse tensors using graphs, we can provide huge memory saving for tensor storage where sparsity level is high, and achieve reduced computation. Thus, we can enable their re-training and deployment in resource constrained devices.
% while sparsity is achieved using bitmask on the computed results.


%To fix this gap, {\graphpy} supports bipartite graph and sparse tensor easily by its novel design. 


% While the support for GNN is an important use-case that we support, we would like to highlight the support for sparse tensors to store model parameters using graph as an out-of-box feature of {\graphpy}. Support of sparse tensors are needed during re-training phase of compressed layers, such as a fully connected layer after weight pruning. The primary vision behind model compression is to enable re-training and deployment in resource constrained devices. Since, deep learning training and re-training process are mostly done in-memory today, Hence if the sparsity level of the sparse tensors are high, using graphs can provide huge memory saving for tensor storage. Thereby, {\graphpy} enables the usage of resource-constrained devices or simply reduces the hardware requirement. Further, decades of research in sparse linear algebra is likely to improve the re-training time when using graph to compute sparse kernels.
%The sparse model uses the weight pruning technique (Fig.~\ref{fig-pruning} in \cref{sec.background}) to convert the fully connected layers to sparsely connected layers.

% To support the re-training procedure of sparsely connected layers, we implemented biparatite graph, the sparse kernel, and the layer, and rely on generated code similar to Listing \ref{list-spmm} to handle bipartite graph and call sparse layer spmm() and sddmm() kernels implemented in the {\graphpy-Kernel}. 
%It should be noted that the graph is this case models the sparse tensors for which no support exists in any prior DL frameworks.

%On the other hand, DGL/PyG does not provide support for sparse tensors. Since, supporting it require two new kernels and corresponding interfaces (apart from supporting bipartite graph), we have to learn details of interfaces and internals of DGL/PyG, and still have to work-around the limitations. Such internal system details are missing from their documentation. Hence, it is likely to take huge effort to implement.
%So, interfaces are important, and we think that no prior work has paid attention to interface design to make the kernel development independent. 


\subsubsection{Graph Data Science Eco-System}
A few deep learning applications
require some of traditional and ad hoc graph analysis. E.g. when
preparing the dataset for deep learning, GraphSage~\cite{graphsage17} first does sampling or community analysis to downsize the graph. Additionally,
it performs connected component analysis, and then does union of a few
components before performing the training on it. Today, such pre-processing is done using NetworkX~\cite{networkx08}, a purely Python Package. Clearly, this approach will not scale when the dataset size is larger, as evident in our measurements in ~\cref{sec.exp}.

We observe that isolated approach of solving different parts of a common problem requires huge efforts. We envision a new graph data science eco-system, that can bring high-performance to every part of such use-cases. Such eco-system should not only provide better performance, but must also allow modular design so that other system researchers can take advantage to develop other functionalities, and plug back their contributions easily. 


\subsection{Education}
There is a need to introduce system-level classes for DL education, as has been voiced in an NSF workshop~\cite{storage2025NSF} by industry partners. 
%Preparing the lectures to explain kernels, and GPU properties are easy. However, It is indeed hard to design kernel assignment that can be used in  end-to-end training without involving additional efforts. 
There exists several courses~\cite{dlsCMU, cs15884CMU, cse599wWashington,cs231nStandford} that teach deep learning. Their coding assignments that have a training loop do not have a system components. While, assignments that have system components allow Python implementation, such as pooling, softmax, batch normalization, etc., and are not evaluated in a training loop. 
%Others~\cite{dlsCMU, cs15884CMU, cse599wWashington} focus on the deep learning system, however, their code assignment is piece-wise (not an end-to-end approach like pacman), mainly focusing on individual components in Python and not in C++ without using them in an end-to-end training. 
%implementing computational graphs or gradient updates in a Python environment. \td 
%Therefore, there do not exist any education assignments which can provide potential c++/CUDA kernel implementation for DL systems.

We strongly believe that the learning remains incomplete, if students cannot see the impact of kernel developed as part of an assignment or semester long project in a training loop.
%Due to fixed duration of any coursework, students needs a software infrastructure to quickly do the assigned tasks. 
Further, we cannot expect students to write this integration task from scratch, as integration problem solving or taking care of storage management is not aligned with the teaching goal of every assignment. 
Moreover, the limited duration of coursework is likely to be a challenge in completing those parts.

%We see many other challenges in offering such infrastructure today. \textit{Firstly}, it is also difficult for students to design graph and tensor exchange between the environment and kernel.
%%That is because this procedure is not important for  systems teaching, but it 
%which is very important in GNN systems implementation because it links the Python environment with the C++/CUDA kernel. Without this link, the GNN system cannot work even if the remaining parts are correct.  However, as we explain in \cref{sec.science.challenges}, passing graph and tensor to a kernel is very different and challenging than passing data between Python and C++. \textit{Secondly},  %Students do not know where to start and how to design the infrastructure.
%Students may not learn deep learning when preparing the dataset and create the corresponding graph storage, which varies based on the type of GNN model, as well as based on one's conviction about which storage will result in better performance. Although there exists some third-party library that can generate the graph object, this graph object cannot be used to implement the GNN kernel. \cref{sec.science.challenges} explains the reason in detail. \textit{Lastly}, ideally GNN assignment platform should be a real-time assignment protocol to match the GNN systems. In other words, the ideally platform should be separated to different tasks(functionalities) easily. However, existing works are very complex and it is impossible to use them to teach students about GNN kernel as well as some CPU, and GPU optimization strategies. \red{not clear.}
 
%Our novel design (section 4) makes {\graphpy}  become an ideal education platform for the GNN system. To prove it, the {\graphpy} was introduced to a graduate-level course that we taught recently. Students were able to implement CPU and GPU versions of GCN in 4 weeks, and each student independently implemented another GNN in the semester-long project. We plan to introduce {\graphpy} in the undergraduate courses also.

% By devising tensor exchange method independent of DL framework, and allowing passing of any custom objects in Kernel APIs, {\graphpy} offers application in any deep learning domain. 

% By focusing on graph data science use-cases, {\graphpy} has made it very productive to educate learners in graph domain with a focus on Systems education. Since, {\graphpy} touches the very basic building block of end-to-end deep learning procedure, classroom assignments can be tuned to target different functionalities. 

% This novel design of {\graphpy} 
% let learners remained focused to complete DL programming assignments, as evident in a graduate level course that we taught recently. 
% Students were able to implement CPU and GPU version of GCN in 4 weeks, and each student independently implemented another GNN in the semester long project. We plan to introduce {\graphpy} in the undergraduate courses, and share it with wider audiences to fulfill the demand of the industry~\cite{storage2025NSF}.

% \noindent \textbf{Minimizing the Framework Overhead.}
% Avoid introducing overhead is an necessary requirement for a system so that the later optimization techniques will not try to minimize that overhead, and rather should focus exclusively on actual system optimization tasks. In other words, when compared against small overhead systems, it is not likely to get misleading benefits. However, in the traditional graph data science domain, Mcsherry et al~\cite{mcsherry2015scalability} point out that many systems introduce large system overhead, which is then also optimized as part of analytics performance optimization. Hence, actual performance improvement remains less.

% Our experiment measurements (\cref{sec.exp}) show that DGL introduces huge system overheads in the form of a one-time start up cost, and run-time overhead, which is also identified by DGL. And because of these two costs, DGL performs poorly (more than 2$\times$)  compared to reference implementation (not optimized) of {\graphpy} for GNNs on several dataset, despite DGL kernels performing better than {\graphpy} kernels. Since DGL has a large overhead, it is not surprising that many prior GNN systems~\cite{GNNAdvisor,huang2021understanding}, which do not use DGL for their integration, have a huge speedup.

% To this end, {\graphpy} through its lightweight design minimizes both the overheads, and hence is well-suited not only for future systems research prototypes, but also as a baseline to understand the true impact of prior system optimizations.

% %On the other hand, DGL/PyG takes only COO arrays as input in their initialization API. 
% %Further, the generation of critical boiler-plate code, makes integration effortless. 
% \noindent \textbf{Sparse Data.}
% We also implemented {\graphpy-Kernel} for GNN as proof of concept and reference. We mostly focused on CSR/CSC format for reference and comparison, 
% It includes an unweighted gSpMM kernel to support GCN and GIN; a weighted gSpMM kernel, and two versions of gSDDMM kernel for GAT as mentioned in Table~\ref{table-kernel}. 
% %Both of these are sufficient for a graph-specific softmax layer, and for edge-level attention score from vertex-level features.
% We use pull-style computation that avoids usage of atomic instructions: so CSC for forward and CSR for backward computation or wherever inverse graph is needed.
% We used OpenMP for vertex-level parallelism in CPU. % and use vertex-centric computation.
% To support GPUs, we implemented kernels in CUDA. The same {\graphpy-Workflow} works except that the model requires to be converted to GPU, which is achieved using $model.to(cuda)$, where cuda is the device context. Similarly, the adapter of {\graphpy-Workflow} allocates tensors directly on GPU.

% We also implemented another format borrowed from prior graph analytics work~\cite{gstore}, which is very different from CSR/CSC format to demonstrate that an entirely different format can be implemented with same ease, using the same set of Kernel APIs. We used the same {\graphpy-Workflow} code, including the GNN model, graph convolution layers. We do not use that format for comparison.
% % \noindent 
% % $\bullet$ \textbf{GPU Support.} 
% % The specialized kernel is also implemented in GPUs by using the same boiler-plate code. The same {$wrap\_graph$()} API instead of simply wrapping the CPU version of Numpy arrays, it copies them to GPU memory, and then wraps them up in $g$ object. Thus, the rest of the kernel APIs (Table~\ref{table-kernel}) get the GPU version of the graph, and Python binding code of the kernel invokes the GPU kernels. Thus, the same piece of {\graphpy-Workflow} works except that the model requires to be converted to GPU, which is achieved easily using $model.to(cuda)$, where cuda is the device context. Similarly, the {\graphpy-Workflow} allocates tensors directly on cuda or device memory.

\noindent \textbf{Observation \#1.}
General purpose DL frameworks' plugin development environment have interface  limitations that only allow their captive tensor data-structure and built-in scalar type but not a graph object to be used as kernel arguments. Due to such limitations, many works~\cite{pytorchg2019,spektral,graphnets,GNNAdvisor,gespmmsc2020,huang2021understanding} have devoted huge efforts due to critical thinking (\cref{sec.science.challenges}) in designing workarounds to pass graph storage to kernels. Clearly, such efforts have no research outcome, and are merely done to integrate the kernel. Some~\cite{pytorchg2019,spektral,graphnets} even chose inefficient COO format, as it can easily be passed as a pair of tensors, despite it being inferior to CSR/CSC format.

%(see \cref{sec.background.graph} for definition) 
%discarding the decades of research works on sparsity~\cite{zhang2015numa,gstore,libgraplus15DB,liu2015enterprise,wang2015gunrock,gorder16sigmod,rabbit16ipdps}.
%such as using specifically tailored data layout~\cite{zhang2015numa,gstore,libgraplus15DB}, graph-aware compression~\cite{libgraplus15DB,gstore}, fine-grained and workload-aware parallelism~\cite{liu2015enterprise,wang2015gunrock}, graph re-ordering~\cite{gorder16sigmod,rabbit16ipdps}, graph partitioning, etc. for CPUs and GPUs. 
%The limitation has clear implication in terms of critical thinking efforts about designing workarounds (\cref{sec.science.challenges}) on how to pass the CSR/CSC graph storage to kernel prototype as evident in~\cite{GNNAdvisor,gespmmsc2020,huang2021understanding}. 
%that could have been devoted to actual research. 
%while a few excellent DL system research did not show the impact on the end-to-end training
%or requires development of new tensor library along with its memory management.
%Sparsity has recently been handled for traditional graph data science use-cases ~\cite{malewicz2010pregel,gonzalez2012powergraph,roy2013x}, such as Breadth-First Search, PageRank, or unsupervised machine learning. 
% Due to its similarities with GNN (\cref{sec.gnn-background}), it is natural to use these techniques to handle the sparsity in DL.
%However, to use these code-bases in an end-to-end DL benchmarking, we need DL framework's crucial features, such as \textit{computation graph}, \textit{tensor management}~\cite{dgl2019}, and \textit{gradient back-propagation} (\cref{sec.background.dl}). 

%\noindent \textbf{Observation \#2.}
%It is insufficient to implement the new GNN kernels either on top of prior graph analytics code-bases or from scratch in isolation without integrating them in an end-to-end DL model training loop. The reason is that 
To bypass the integration, many system works focus on isolated approach of kernel implementation and evaluation. However, 
In DL, forward computation, and gradient back-propagation generate requirements for different graph storage and computation. E.g., GAT~\cite{gat18iclr}, the edge-level tensor should only be accessed using edge IDs that should be part of the graph storage (\cref{sec.background.dl}), and may be missed by such approach. %Unfortunately, an evaluation that only focuses on kernel optimization in isolation without evaluating the training accuracy is likely to skip such finer details of edge ID requirement, resulting in misleading performance comparison. 
We point out that performance benchmarking without evaluating the accuracy have resulted in errors in performance measurement in prior works~\cite{GNNAdvisor,huang2021understanding} (\cref{sec.gnn-background}). 
%Such observation outline the need to integrate the kernel optimization in an end-to-end training loop for accuracy evaluation, before performance evaluation can be performed.  
%Rather, we observe that a few prior works that still focuses on  
%As we explain in \cref{sec.science}, integration is a complex task, and requires work-around instead of being straight-forward. 


%Systems frameworks such as MPI, OpenMP, PGAS etc.
% \td maybe we talk a little bit more about GAS,(GAS can achieve the same performance as original algorithm?)
% While some difference does exist  between graph analytics and GNN, which we explain shortly, 
% Because of the similarity between graph analytics and GNNs, it becomes a natural desire to adapt the system designs from the success of the graph analytics to the GNN workloads to take advantage of the decades of system research work.
% It is imperative that the research community should be able to test the efficiency and applicability of the systems aspects that targeted graph analytics to the GNN workloads quickly, instead of repeating the decades of research work. This exercise is desired because, 

\noindent \textbf{Observation \#2.} Our measurements show that many prior works frequently show out-of-memory error on slightly larger dataset that has less than 230 million edges in a single GPU setup. Due to this, prior works have only evaluated smaller dataset. Our investigation finds that any performance improvement in training smaller dataset is purely due to framework overhead, and not because of better kernel performance. Hence, we hardly have any baseline system which allows training on larger dataset so that it can be used to authoritatively show performance benefit of better kernel design on end-to-end DL training tasks in a single GPU setup.

\noindent \textbf{Observation \#3.} 
Existing works handle the sparsity for data science use-cases in a piece-meal way. (a) GNN systems handle only sparse data, but not sparse tensors that can use graphs. (b) There is no support for many common tasks, e.g. graph storage preparation from raw data.
For different GNN models, graph storage differ a lot in terms of graph direction, edge ID, etc., thereby same tasks need to be repeated for different GNNs by users in ad hoc way. 

%Hence, a new abstraction is needed that can unify the support for diverse graph storage need to an independent module, and makes exchange of graph storage simple and standard without repeating the mundane tasks. 
%Hence, many GNN systems~\cite{GNNAdvisor,neugraph19atc} have chosen to demonstrate only simple GNNs, where graph is undirected and unweighted, ignoring the attention based GNNs such as GAT or sparse models. 
% (c) NetworkX ~\cite{networkx08}, a purely Python graph data science package, remains popular due to its ease of use by data scientists, but remains very slow due to absence of system languages like C++/CUDA. 
% Therefore, there is a gap between systems (C++/CUDA) research deployment for traditional graph data science (Python) use-cases.

%To fix this gap, we see an opportunity in unifying different use-cases under a single platform with open interfaces where independent high-performance back-end modules can be plugged easily including abstracting the common tasks to a single module. 
%and can exchange data using zero-copies.
% We argue that providing Python binding on top of such optimized systems will bring the performance advantage to data scientists, while it can help in abstracting away many mundane tasks in variety of data science use-cases.
% despite being an order of magnitude slower. 



% \noindent \textbf{Observation \#3.} Traditional graph analysis did achieve an incredible system performance, but NetworkX~\cite{networkx08}, which is purely a Python package, is still very popular and is maintained actively due to the ease of use of Python programming environment over system languages like C/C++/CUDA. We argue that providing Python binding on top such optimized systems will bring the performance advantage to data scientists.
% despite being an order of magnitude slower. 
% However, bridging the gap between systems researcher (C/C++/CUDA) and data-scientist (Python) is not possible without significant research and design effort (\cref{sec.multi}.



% Lets us talk about GraphOne in problem statement.
%Although there exists some graph analytics systems which includes the graph data engineering, such as GraphOne~\cite{kumar2017graphone} NetworkX~\cite{networkx08}, these works cannot be used in the graph data science directly. But GraphOne, A, B are mainly written in c++. These implementation incompatible also increase the difficulty for users to deploy the mechanism to re-use these graph representations. 
%Firstly, Graphone, A, B, NetworkX do create the graph representation structure, but if the user wants to use it, they need to figure out the graph structure details, which is not an easy job.

% \noindent \textbf{Observation \#3.}
% Existing GNN systems such as DGL, featgraph, GNNAdviosr  (need citation TODO)
% implement their kernel by using the c++/CUDA plugin of a specific DL framework backend. (Not sure whether DGL satisfies this or not TODO) This system design makes their kernel highly dependent on not only the DL framework backend but also the specific version of the DL framework backend.
% The DL framework backend dependency limits their kernel codebase to a specific DL backend, which makes their codebase cannot be re-used across different DL framework backends.
% The DL framework backend version dependency increases the manual effort to maintain the GNN systems because of the periodic update of DL framework backend versions.
% Moreover, the DL framework backend version dependency increases the difficulties and complexities of usage because there may exist package version conflicts when configuring the environment and compilation.
% Therefore, there is a need to provide a unified GNN system that is independent of backend versions and their codebase can be reused across different backends.


\noindent \textbf{Observation \#4.}
Industry partners have voiced concern on availability of candidates with good systems and data science knowledge~\cite{storage2025NSF}.
%However, DL frameworks limitations do not allow them to be used as educational platform for DL system learning. 
%There exists a void in terms of education tools to introduce deep learning system research to our future system engineers and researchers. 
In Operating Systems (OS), XV6~\cite{xv6} has become a popular tool for undergraduate teaching allowing OS kernel modification for learning. 
%Similarly, the Pac-Man~\cite{denero2010teaching}, Open AI gym~\cite{brockman2016openai}  and RLcard~\cite{zha2019rlcard}, etc. provide sufficient environment for evaluating reinforcement learning algorithms.
However, limitation in DL frameworks' plugin interfaces, that disallow passing custom objects, limits their usage. 
We observe that many deep learning system courses~\cite{cs224w,cse599wWashington,cs231nStandford,cs15884CMU,dlsCMU} in universities actually allow Python to prototype the kernel assignments without focus on its integration in a DL workflow. 
Hence, they not necessarily train students in data science and systems both.  
%Therefore, we believe a lightweight platform is the need of the hour to train students in data science and systems together. 
%Other approaches need huge efforts just to integrate kernels to deep learning training, while being severely limited the way data can which may not be suited for assignments in semester long courses.

% and it is not modular enough to easily implement them as explained in \cref{sec.background}.

% \vspace{1mm}
%\noindent \textbf{Proposition.} Evaluation of the system techniques proposed by traditional graph analysis for the DL use-cases, offering high performance to data scientists, and speeding up the systems research in graph data science are all related problems, and have a number of overlapping steps. While general-purpose DL frameworks are definitely not suited for such purpose due to poor support for sparse data and sparse tensors, even the current GNN frameworks are not ready yet, as they still lack the support for sparse tensors/layers. Moreover, it even does not handle a graph different from a plain homogeneous graph. Thus, sparse layers and ad hoc analysis cannot even be supported (\cref{sec.motivation}). Finally, only few are open-sourced, they are monolithic, lack design documentation for back-end and are frequently changing, and do not preclude writing many mundane tasks. Hence, modifying such monolithic and frequently changing code-base for prototyping system ideas is hard and time-consuming, and the resultant system will become even more complex.

% and it is not modular enough to easily implement them as explained in \cref{sec.background}.
%A platform is desired for quickly prototyping any new or old system idea without getting bogged down by the sheer complexity of learning undocumented code-bases or with dated documentations. Rather, a platform is also desired to introduce deep learning to our future systems engineers and researchers, which has been flagged as a concern in various forums[\td]. Modifying the back-end of general-purpose DL framework for educational or even research purpose is too time consuming. Following a restricted programming in the form of plugin development and their build system (e.g. in Pytorch) will result in a loss of general learning specifically how the interfaces work in such a large system. Further, these all method involves repeating many mundane steps that provide no value to research or learning. 
%At the same time, offering data-scientist high-performance APIs is needed. 


% A good platform for graph data science should clearly identify the boundary between different tasks, should provide all the mundane task for graph data science and offer boiler-plate code to integrate the third party kernels, and let the system programmer continue with their choice of tool-set and programming language. 




\noindent \textbf{Contribution.}
We present {\graphpy}, a modular and interface oriented lightweight platform to enable implementation of various graph data science use-cases for both research and educational purpose. Fig.~\ref{fig-arch} shows a high-level overview of {\graphpy}. Contributions are summarized as follows:

\noindent $\bullet$ \textbf{Tensor and Graph Exchange.} The innovations in interface design enables tensors to be passed to kernels as array-like structure, and allowing graphs or any custom objects to be passed to kernels directly, thereby avoiding the need of critical thinking that we discussed in observation \#1.
%same way that any dense data (such as images) are passed, thereby achieving uniformity without any limitations. Further, any arbitrary objects could be passed as well. 
Compared to current practices, {\graphpy} interfaces have no issues in passing any data-types in kernel invocation, and enable {\graphpy-Kernel} to gain full independence from any DL framework code, thereby
%and offer easier research prototyping and effortless deployment. 
introducing \textit{re-usability} of kernel code across many DL frameworks and their versions. 

\noindent $\bullet$ \textbf{Automatic Integration.}
{\graphpy} \textit{generates} critical boilerplate code to handle interfaces, memory management, and Python binding of kernels.  This results in zero effort in integration. 
%

\noindent $\bullet$ \textbf{Separation of Graph Storage, and standardization of its Exchange.} 
%to an independent high-performance {\graphpy-SM} module is achieved using \textit{Numpy dtype} that can supports specification of \textit{arbitrary multi-field graph properties}. The module exports the graph storage using \textit{zero-copy} Numpy arrays to other modules to free the data scientists and systems researchers from graph storage tasks. 
By separating the graph storage management, we allow innovation in interface design that let {\graphpy-SM} to handle multi-field graph properties using a single set of API by using \textit{NumPy Dtype}, while exporting the prepared graph storage to {\graphpy-Kernel} using \textit{zero-copy} NumPy arrays. 
By relying on  Dtype, {\graphpy} makes sparse matrix (i.e., graph) same as dense matrix (e.g., image data) for storage specification and exchange purpose. Interface design leaves enough room in {\graphpy-Kernel} to innovate on graph storage design without impacting {\graphpy-SM}.
We are unaware of any high-performance Python package that can support arbitrary multi-field graph properties. It also cannot be designed without significant innovations(\cref{sec.engg}). 






% NetworkX~\cite{networkx08} is the closest one, but is a pure python package, and hence lacks scalability, performance, and cannot handle big graphs. 
% It also supports the arbitrary edge features which is important in knowledge bases graph GNNs. Besides this, the graph creation module also provides flexible choice for users to determine whether create the edge ID or whether procedure(forward/backward) the edge should be created. 

% Furthermore, it generates boiler-plate code to integrate independent kernels of different data science use-cases to keep the efforts minimal while integrating them to Python and provides an extensible architecture to support various computations that makes it easy to implement new system idea. 



% {\graphpy-Kernel} module is an independent plug-and-play module responsible for kernel implementation in CPU/GPU by using the above prepared graph, while {\graphpy-Workflow} uses general-purpose DL frameworks to offer computation graph, and gradient back-propagation, and uses Python APIs of {\graphpy-Kernel}.
% To integrate these without much dependency, {\graphpy} generates the required critical boiler-plate code for Python binding of kernels, and tensor handling code in {\graphpy-Workflow} using our proposed domain-specific language (DSL). The generated code does the memory management of tensors and passes them as flat arrays to {\graphpy-Kernel}. Hence, this separation and generated code reduces the end to end development cost of any DL layer and corresponding kernels. 

% 3.{\graphpy} supports dynamic graph by incrementally update the graph representation. Some optimizations techniques are also adopted so that it can support large graph. 





% 7. {\graphpy}support extensible wrapped python APIs. {\graphpy}is optimized to only use c++ as the bottom implementation language in kernel module and graph creation module and wrapped them out to python to interact with remaining modules. In other words, we use python for modules without high performance requirement instead of implementing all modules in c++ but provides some high level python APIs. This implementation strategy can let graph neural network researchers extend or add new customized graph DL framework easily. 

% The contributions of our work are summarized as:
% \begin{itemize}
% %\item Unifying the graph data engineering with graph DL leads to one integrated graph neural network system, and provides end-to-end control over data engineering and machine learning operations resulting into greater synergy and performance.
% \item {\graphpy} supports graph creation with arbitrary vertex and edge properties, which make it more flexible for multiple types of graphs, and GNN models. It is mainly written in c++, but provide python user interface, which make it possible to use more cores and distributed systems to handle larger graphs.

% \td do we also need to mention that graphPy is a end-to-end work that users do not need to worry about how to read raw data?
% \noindent $\bullet$
% {\graphpy} unifies the GNN system research by its novel memory management design and framework design. 
% Unlike existing systems, {\graphpy} does not limit to a specific DL framework version or a specific DL framework backend.  Therefore, System researchers only need to focus on kernel implementation and optimization instead of worrying about environment configuration.
 

%Further, combination of two entirely different languages: compilation oriented C++/CUDA with interpretation oriented Python, creates further challenges. 
\noindent $\bullet$
\textbf{Modular and Lightweight.} {\graphpy} is inspired from the Unix Philosophy~\cite{mcilroy1978unix} as opposed to monolithic design.
Hence, custom use-cases for handling sparsity can easily be developed, optimized and deployed independently.
%By using graphs to model the sparsity, {\graphpy} opens a new research direction where the plethora of work done in graph analytics can be extended to GNN, and to support sparse tensors that can be modeled using graphs.
%Further, focus on interface design minimizes the framework overhead that other systems~\cite{dgl2019} often encounter
%\footnote{See \url{https://arxiv.org/pdf/1909.01315.pdf} for DGL overhead} 
%making {\graphpy} an excellent framework for research.
Bare minimum code-base, and support for graph storage make {\graphpy} an excellent tool for deep learning system education, 
%as system learners only need to focus on kernel implementation and optimization, 
while automatic integration allows system code evaluation in actual graph data science use-cases, that we believe is a strong motivation for learners to stay invested. 
%Further, the lightweight design leads to less framework overhead, while our reference implementation consumes less memory that makes {\graphpy} an ideal baseline system. 



% {\graphpy} helps in easy prototyping any DL layer as well as performing systems research where the plethora of work done in graph analytics or new systems ideas can easily be tried for deep learning.
% Due to such flexibility, we are able to offer a high-performance implementation for GNNs, sparse models, and traditional graph analysis that all are usable from Python. 
% For evaluation, we use our reference vanilla implementation, and leave the evaluation of optimizations as future work. 




% \noindent $\bullet$
% From the view of the flexibility of sparsity use-cases, {\graphpy}  can be used in multiple levels of sparsity situations due to its novel design. For example, existing DL frameworks, such as DGL and PyTorch Geometric, can only support data level of sparsity (e.g., Sparse data, the data itself is sparse). However, {\graphpy} not only supports data level sparsity but also can support model level sparsity (e.g., the Sparse model, the compressed deep learning model itself is sparse, which means many model weights are set to 0).


We demonstrate the usefulness of {\graphpy} with the implementation of at least two different storage format for many GNN kernels as well as support sparse tensors that can be modeled using graphs, and using {\graphpy} in a graduate-level course. Empirical evaluations show that our \textit{reference implementation} achieves 1.62$\times$ and 1.35$\times$ over DGL and PyTorch for various GNN models on many datasets in GPU, and 1.55$\times$ and 1.88$\times$ on CPU respectively with similar accuracy readings.
%on an average 1.64$\times$ and 1.42$\times$ speedup and 1.30$\times$ and 2.29$\times$ speedup over DGL, and PyTorch Geometric for various GNN models in GPU and CPU respectively. 
Investigation of accuracy and speedup together brings several critical observations, which question some of the measurement practices of prior works: focusing purely on performance gain without measuring accuracy is a recipe of disaster for this new area of GNN research for which we do not have complete system understanding, including graph storage requirement, role of framework overhead, etc.  
%Further, frequent out-of-memory condition by DGL, Pytorch-Geometric, and GNNAdvisor forces measurements to be performed on smaller dataset only. Measurements on smaller prevalent dataset do not show advantage of kernel optimization due to framework overhead.
To this end, our measurements show that focus on interface design minimizes the framework overhead of {\graphpy} by 1.46$\times$, and 1.28$\times$ than DGL and PyG.
Low memory consumption allows {\graphpy} to run GCN, GIN, and two versions of GAT on all the datasets, while DGL, PyG, GNNadvisor all have many out-of-memory conditions.
%\footnote{See \url{https://arxiv.org/pdf/1909.01315.pdf} for DGL overhead} 
%making {\graphpy} an excellent framework for research. 
A better GNN performance using the reference implementation, less framework overhead, low memory consumption make {\graphpy} an ideal baseline for performance benchmarking for future research. 
%as prior works show out-of-memory conditions even on a moderate sized dataset on which evaluation is mandatory, as measurements on smaller prevalent dataset do not show advantage of kernel optimization. 


\begin{figure}[t]
  \includegraphics[scale= 0.5]{result/overview-crop.pdf}
 \vspace{-6pt}
  \caption{ \small {\graphpy} Platform: {\graphpy-Kernel} is plug-and-play, which can be customized to implement any novel system design to handle sparse data and model. {\graphpy-Workflow} provides the DL support including tensor management and computation graph.} 
  %{\graphpy-SM} prepares graph.}
  \label{fig-arch}
%   \vspace{-12pt}
\end{figure}

%We show that the speedup with respect to DGL is the result of less framework start up and run-time overhead, as DGL kernel performs better than the {\graphpy} reference kernels. We also show the implication of DGL's framework overhead on evaluations of prior works, and why its design and overhead discourage researchers to use DGL for research prototyping. 
%This result confirms that latest GNN works have benefitted from while proposing new system optimizations have not compared against well-known but simple parallelization techniques. Hence, we establish new baseline for GNNs that can be used for evaluating impact of future optimizations.

Moreover, we show that using graphs for re-training compressed LeNet-300-100 (sparse model) on MNIST dataset leads to 17.5\% speedup in CPU, while minimizing the memory need of the compressed layers.
For the graph creation procedure, {\graphpy} is more than 5$\times$ and 10$\times$ faster than DGL and NetworkX respectively on various datasets. 
For traditional graph analysis from Python programming environment, {\graphpy} is up to an order of magnitude faster than NetworkX.



%}
% system with a high-performance graph creation module and pluggable, neural kernels modular as well as the transparent, extensible python Graph DL APIs. It also outlines the steps to keep the efforts minimal while integrating the techniques of prior graph analytics systems to {\graphpy}.
% \td figure one words is not the same as we discussed below, do we need to modify it?

% \textit{{\graphpy-DE}} is a high-performance graph data engineering module which will create the graph representation directly from the raw graph data from Python programming environment, and exports it to be used by any module. % It also uses zero-copy mechanism to export the prepared graph out to any other module in the CSR, or COO format.
% \textit{{\graphpy-Kernel}} is a \textit{plug-and-play} high-performance module, where each instance is is responsible for implementing kernels using the prepared graph and boiler-plate code for a specific use-case. 
% \textit{{\graphpy-Workflow}} provides all the support for DL workflow. It uses the DL framework to provide computation graph creation, tensor management, and gradient computation, and allows the specialized version of {\graphpy-Kernel} to be called during forward and backward computation both without doing any single tensor related operations inside the kernel.


% (b) between graph analytics and DL. We present {\graphpy}, that provides a ready to use python package for data engineering efficiently, but also outlines the steps and provides solutions to keep the efforts minimal while integrating the prior graph analytics systems. 
%this gap by presenting an end to end pipeline to support graph data science and graph data engineering. 

\noindent $\bullet$
\textbf{Support Sparse Tensors.}
{\td add the sparse tensor in background}
Except for the GNN, many model compression works involve a different level of sparsity. (Our section \td ) These sparsity differences prohibit the existing works to apply to this problem anymore. In this work, Our modular-based design lets us be the first one to provide memory saving and performance speed-up for this type of sparsity, which can deploy them to the limited-source device.
\subsection{Sparse Model Retraining Performance}

We choose the LeNet-300-100 \cite{lecun1998gradient}, a fully connected neural network with 300 and 100 as the hidden layers as the DL architecture. After weight pruning, all three fully connected layers become sparse with sparsity ratio of 4.46\%, 4.45\% and 7.78\% respectively, i.e., keeping less than 10 connections for every 100 connections in the fully connected layer. We use MNIST dataset which includes 60000 training and 10000 testing handwritten digits examples.  Each image in the dataset has 784 features, while the last fully connected layer produces prediction corresponding to 10 digits (0--9), which are sent to the softmax layer. 
We set the retraining epochs as 100 and the batch sizes as 50. In other words, in each training epoch, the model will iterate 1200 times.
% and apply tensor-based operations for state-of-art model and the sparse layers computation for {\graphpy}.
{\graphpy} finishes the retraining in 16 minutes and 17 seconds, compared to 20 minutes and 1 second for the state-of-the-art model that uses the bitmask matrix to achieve sparsity, achieving 17.5\% speedup, and huge memory saving.

%The reason for this speedup is the reduced computation which {\graphpy} could achieve due to its system-level support for sparsity. 
On the other hand, prior works have used bit-mask matrix at the Python level for achieving sparsity where the underlying kernel still uses dense matrix for sparse layer computation. Again, the improvement is only 17.5\% as LeNet-300-100 is not a large neural network, as the bipartite graph has vertex counts in the range of 784 and 10. Hence, the sparse weight matrices are not as large as the graph data set we had above for GNN case. This affects the vertex-level parallelism for SpMM. With better technique, we expect better performance, as our implementation is only for reference. 

Secondly, it is not just the performance improvement, but the huge memory saving that allows the compressed model to fully fit in the resource constrained devices. Hence, model inference can now be done fully in such devices.
% Also, the sparse layers computation procedures contain mostly random reads instead of sequential reads. 


==> tex/others.tex <==
\vspace{1mm}
\noindent \textbf{Proposition.}
However, these graph deep learning system cannot directly read the graph structure from the raw data, instead, they rely on some pre-implemented python graph structure, NetworkX ~\cite{networkx08}, or a list of python objects. This design will make the users need to do more graph preprocessing jobs and lack scalability, performance, and cannot handle big graphs. Moreover, NetworkX cannot support dynamic graph representation, which means even if the graph is updated by a small number of edges, the NetworkX needs to re-create the whole graph representation instead of increment updating. This triggered us to design an end-to-end graph deep learning system with a high-performance graph creation modular which can support dynamic graph. 
 
As we mentioned in the introduction, the GNN research area is young, which means many new GNN frameworks with different variant tensor operations or some customized message-passing paradigms maybe proposed in the future. Therefore, the extensibility of graph deep learning systems become important. A good graph deep learning system should be flexible enough to extend to new GNN operations and should be able to add in new customized message passing kernels easily without worry about the code dependency. 
 
Although DGL does provide some extensibility by providing 4 scatter choice ‘sum, sub, multiple, divide’ and 3 gather options ‘max and min, sum’ for users to choose, the message passing paradigms is fixed. If users want to apply a customized message passing paradigms, they need to modify the whole message-passing paradigms as well as the dependent codes in other submodules. This design pattern may limit its usage because graph neural networks are more familiar with machine learning operations and it is hard for them to handle system code dependency.  From the above observation, we put all message-passing paradigms in a pluggable, neural kernels modular and minimize code dependency between different modular. 
 
For some knowledge bases graph GNNs[NEED ADD SOME CITATIONS], the edge information is also captured when applying the graph deep learning. Unlike the traditional edge information which normally treated as the edge weight or a float number, the edge information in the knowledge bases graph can be extended to a vector.[Not sure whether  I understand it correctly or not] Therefore, there is a need for a graph deep learning system to support the customized edge. 


Moreover, different GNNs have different aggregations. GCN uses the unweighted sum as the aggregation. But GAT uses the weighted sum version to assign a weight for each corresponding edge. In other words, edge ID is not necessary for GCN but necessary for GAT. It is unnecessary to always create the edge ID for GNNs. Moreover, the backward procedure of message passing paradigm need to integrate more computation than the forward. If the edge Id can be stored based on the backward procedure, the performance will be improved. Therefore, it is necessary for a graph deep learning system to provide flexible edge choice to users, such as whether creating the edge ID and which procedure the edge ID should be stored. 




\noindent 
$\bullet$ \textbf{New Sparse Formats and Data Sharing}
While we discussed that Numpy arrays will be used to allow zero-copy sharing of graph structured data, and hence it becomes very easy to share CSR/CSC format. However, once a system researcher comes up with an entirely different format~\cite{gstore,mosiacEuroSys17,hicoosc18}, one can think that {\graphpy-DE} as well as the data sharing APIs become non-usable. 
It should be noted that G-Store~\cite{gstore} calls the format Smallest-number-of-bits (SNB), and Mosaic~\cite{mosiacEuroSys17} calls it tile format. HiCoo~\cite{hicoosc18} reduces to the same format when dealing with sparse matrices, but it also extends this to higher dimension sparse data. We use SNB format as it was published first, and explain how the same set of API can be used for graph preparation and data exchange.

\begin{figure}[h]
  \includegraphics[scale= 0.22]{result/zero_tile.pdf}
  \caption{{\graphpy} SNB format.}
  \label{fig-snb}
\end{figure}

 \textbf{Solution: CSR as an Indexing Structure.}
To solve it, we came up with a generalized theory about graph data preparation and sharing that can capture graph in various formats. 
Fig.\td shows the SNB format, which we have re-arranged to make it look like CSR structure. This established the fact that CSR can be used as a general purpose indexing structure, wherever we have one-to-many relationship. 
Clearly, all the data exchange format remains same as it is, e.g. we can still use the 4 Numpy arrays with slightly different dtype to share the graph between {\graphpy-DE}, and {\graphpy-Kernel}, as shown in Listing \ref{list-snb}. It only required one cosmetic change at both the line number 6 and 10. 
%We also needed to modify the $get\_graph$() API that also returned vertex count as we cannot rely on offset array for the vertex count. This also require that we pass vertex count in the $init\_graph$() API. However, all these changes are cosmetic from the user point of view as we provide different version of $prep\_graph$() API.


%Python code highlighting
\begin{lstlisting}[language=Python, caption= Illustration of graph creation in SNB format, label={list-snb}]
import numpy as np
import graphpy as gp
def prep_graph():
  edge_dt=np.dtype([('src', np.int32), ('dst', np.int32), ('wt1', np.float), ('wt2', np.int32)]
  #Directed and SNB graph. 
  G=gp.create_graph(gp.eDdir|gp.eSNB, edge_dt) #Changed code 
  #space is delimiter
  G.add_edges_from_dir('./input_dir/', ' ')
  #Get graph as numpy array using SNB dtype.
  snb_dt=np.dtype([('src', np.int16), ('src', np.int16), ('wt1', np.float), ('wt2', np.int32)]) #Changed code
  csr_offset, csr_neighbor, csc_offset, csc_neighbor = G.get_graph(csr_dt)
\end{lstlisting}

To implement it in {\graphpy-DE}, we still utilized the same infrastructure, but had to adjust the \textit{CSR creation routine} in Fig.~\ref{fig-parallel_pa} to offer graph in SNB formats without changing its APIs.

Off-course, {\graphpy-Kernel} has to implement all the GNN kernel code, but it can still utilize the boiler-plate code. For the proof-of-concept, we integrated G-Store code which also had in-memory processing routine. We also implemented the spmm kernel for GCN. It should be noted that we did not require any changes to the {\graphpy-Workflow}.
%Should this format result into better GNN performance, but we leave it to the respective authors to implement the kernel and find out the details.





\subsubsection{\#2: Integrating Graph Analytics System Research with GNN}

Since existing graph analytics systems usually include optimized high-performance graph computation engine. A straightforward way to test their innovating ideas is to integrate these graph analytics systems with Graph neural networks by simply implementing the new GNN kernels on top of them.

\noindent \textbf{Gap between Kernel and DL Framework.}
One approach to integrate newly written kernel code to current DL framework is to port them to DL Frameworks. However, current DL frameworks does not have support for sparse linear algebra, and hence it is not easy to integrate these system enhancements to improve GNN performance, as it will involve huge efforts not only in integrating into the back-end but also require python binding as per the limitation of these frameworks. Such frameworks allow python binding of limited types.

%To this, end, we list down some basic building blocks, that can guide researchers from graph analytics field to quickly prototype additional functionality on top of the existing code base to test whether those techniques are beneficial or not, before we jump to brand new implementation.
One can try to integrate those code-bases to existing GNN frameworks by porting the existing design and code to them. However, such porting generally requires huge effort to understand the existing development environment and framework. Moreover, their code-base is still nascent, does not have documentation on how one can integrate the code in the back-end, and their code base is constantly changing. Without active involvement of the system maintainer, it seems not possible to integrate new ideas to current GNN frameworks~\cite{featgraphsc20}.
%and as well as  E.g. \td. what are the problems if we integrate in C++ way with Pytorch?  

Hence a more lightweight approach is required, where the job of system researcher should remain limited to implement the required kernels using their design without being restricted to follow a specific development style or any changes to the framework. Yet, it should immediately become part of the whole deep learning workflow. 
This will lead us to a flexible and generic infrastructure that will allow an independently developed pluggable modules, yet taking care of managing computation graph and tensors.


\subsection{Opportunities and Challenges}

The forgone decade saw incredible performance improvement to graph analytics tasks, such as Breadth First Search (BFS) or Page Rank due to various novel system designs, such as better data layout, improved utilization of hardware caches, NUMA-aware data partitioning, structure-aware compression, re-ordering to introduce data locality, integration with various hardware platforms, such as GPUs, FPGAs, customized hardware, etc. 
They improved the performance of graph analytics by orders of magnitude. Many of the techniques are highly graph-aware to take care of its irregularity in the structure and computation both.

On the other hand, GNN computations are very new with the first system level framework appearing recently~\cite{dgl2019}. So, there are plenty of opportunities to improve the performance, and is already being tried~\cite{featgraphsc20}. This is now even more important as deep learning training procedures are  more compute intensive than the tradition graph analysis. So, we are likely to see a number of research direction to optimize the GNN training time including using the techniques mentioned above.

% not all the techniques are possibly applicable to GNN eco-systems due to differences in the requirement between graph analysis and GNN.Graph analytics system researchers were highly influenced by Graph500~\cite{graph500} ranking, which benchmarked BFS or other graph traverse algorithms only. Each iteration of graph traverse algorithms operates on an active vertex set only and contains scalar vertex-level metadata only. However, 

However, trying system system techniques in the context of deep learning is not so easy.
These graph traverse algorithm workloads are very different from the GNNs as GNN have 2 procedures, \textit{forward procedure}, \textit{backward procedure} in each epoch of the training. 
Further, the GNN kernel uses vector metadata and trainable parameters for each vertex and edge in forward procedure and calculate the loss based on the prediction result. In backward procedure, GNN kernel computes the gradient and updated the training parameters based on the loss we calculated before. 
In other words, we can view traditional Graph Analytic works as performing the forward procedure only.
% but do not need the backward procedure.
% \td maybe backward also need to store the gradient information? 
As we discussed in Figure~\ref{fig-forward}, backward procedure has additional requirements, including saving and operating on the tensors produced by forward computation, referred as tensor \textit{states}, and many times operating on the inverse of the graph.

%Nonetheless, considering the variety of work it is natural that  we must test the efficacy of such techniques before putting the verdict out. 

So, if one wants to develop GNN on top of prior graph analytics systems, he or she has to take care of data engineering tasks, implementation of GNN kernels on top of their GAS framework, and the deep learning specific workflow including computation graph and gradient calculations. These tasks have system challenges and involves huge efforts as we discuss next.

% Specifically, many of the techniques focused purely on optimizing the BFS due to benchmarking established by Graph500. BFS is very different than GNN kernels. The former is very compute light, and only a few vertices participate in each iteration. Apart from that the computation only happens in the forward direction in graph analytics as it does not involve gradient computation.



%system which can support graph deep learning features. To be more specific, given the raw input data, such as the CSV, Jason, text or binary data, the graph deep learning system should build the dynamic graph representation data structure automatically and also provides python APIs for users to perform traditional graph topology analysis as well as the graph deep learning operations. 
 
%All the previous works cannot support these requirements, this trigger our work {\graphpy}, which unify the graph data engineering with graph deep learning leads to one integrated graph neural network system and provides end-to-end control over data engineering and machine learning operations resulting in greater synergy and performance.





\subsubsection{Traditional Graph Data Science}


With the advent of data-science as a field, people from many fields are attracted to it. One of the important reason of is easy to program using Python programming language, and the ease with which DL frameworks can be programmed at least in a single node/GPU setup.




==> tex/related.tex <==
\section{Related Work} \label{sec.related}

DNN-related benchmark platforms~\cite{mlperf, TBD, dnnmark, Fathom, DAWNBenchA} have been proposed recently, but the presence of the graph makes them unusable for GNNs.
%Additionally, our experiments, along with several other papers, have shown that PyG is significantly slower than DGL for GNN training and inference tasks.
GNN benchmarking has remained an understudied problem. We are not aware of any systems that have focused on this problem. GNNMark~\cite{baruah2021gnnmark} 
%is a benchmark designed to characterize GNN training properties on GPUs. However, its GNN implementation solely relies on code from existing frameworks, DGL and Pytorch-Geometric(PyG). This approach is deemed inappropriate as a baseline for GNN comparisons, as discussed in previous sections. The use of DGL and PyG makes GNNMark become a system-to-system comparison rather than a standardized GNN benchmark which leads to many issues as we showed in Section \td.
%Furthermore, GNNMark itself 
is not designed as a standardized framework to integrate system kernels, making it impossible to integrate with any system-level GNN optimizations.


DGL suffers from framework overhead for runtime and memory consumption. Hence systems integrated into it also have the same issues. The system integration process is also unclear or documented, and each researcher has to first learn its internal for the integration. Hence prior works have followed different approaches. 
%and we could run two popular works of GE-spMM~\cite{gespmmsc2020} and FeatGraph~\cite{featgraphsc20} end-to-end.
GE-SpMM~\cite{gespmmsc2020} provides the source code files to replace the same-named DGL source files. However, those named files are now missing in DGL due to its complete code re-organization, a trait of a monolithic system. %Further, the DGL code-base has included one such file\footnote{\scriptsize \url{https://github.com/dmlc/dgl/blob/master/src/array/cuda/ge_spmm.cuh}} but did not integrate it. Our evaluation revealed functionality bugs with this code. Hence we did not proceed with it.
We also could not run FeatGraph~\cite{featgraphsc20} end-to-end despite trying many GitHub branches as suggested by their authors (see appendix for our communication), though it is officially integrated by DGL using a compile-time flag. So, questions remain on the modality of integration. 
%However, both of them relied on the same storage format as DGL. But 

Supporting a custom graph storage needs to change almost the whole DGL backend including many public system APIs of DGL, such as \textit{successors()} and \textit{predecessors()}, which are not even used by GNN systems. 
%the way we understood advanced features of PyTorch to pass graphs as a custom object using the smart pointer approach\footref{foot.time}.  
%Then, they can prototype a custom kernel and can support custom graph storage.
Hence, spending additional effort may be useless if the whole backend and system APIs need to be replaced. History indicates that such types of optimization works~\cite{huang2021understanding,wang2021gnnadvisor,fu2022tlpgnn,spektral} have rather relied on plugin environment, developed their own model code, system APIs, and system code despite the interface-level limitation.
%We reached to the authors of a few GNN papers to understand why they did not use DGL. 
One of the authors of a prior GNN system aptly described the limitations of working with DGL: \textit{``We didn't use DGL, because some of its design is inefficient but is also embedded in the system design in a complex way''} %\footnote{Personal communication using email}, 
confirming our observation on using DGL. 

Pytorch-Geometric(PyG)~\cite{pytorchg2019}, relying on the Pytorch plugin, and suffers from the limitations that a plugin system suffers.

% offers the CSR and COO graph storage formats based on the input data. 
% %However, PyG's foundation on PyTorch limits its extension to TensorFlow and increases its complexity for future integrations. In other words, 
% PyG was not designed to be a standardized GNN benchmark, resulting in a lack of support for custom graph formats commonly used in current system-level GNN optimizations.



% \subsubsection{DGL: Unsuitable as a Benchmarking Platform} \label{sec.dgl}
% DGL is a widely used open-source GNN system. Many systems researchers have modified it to show the system advances~\cite{gespmmsc2020,featgraphsc20}. However, it is not well-suited to be used as a benchmarking suite as we explain next.
% %\textbf{Custom Kernel and Requirement Mismatch.} 
% %Most systems~\cite{gespmmsc2020,featgraphsc20}\td[more citation] that integrate their system works to DGL have not performed any kernel fusion. 

% \noindent 
% $\bullet$ \textbf{Huge Framework-related Memory Overhead.}
% Our measurements show that the DGL framework suffers from huge memory consumption. The source of this huge memory consumption remains unknown to us.
% While a few prior works blame the extra storage needed for storing CSR, CSC, and COO by DGL\footnote{One DGL researcher also hinted the same during discussion.}, while other GNN systems may only need one or two storage formats.
% However, graph storage is not majorly responsible for such memory consumption. For example, on OGB-Product, the GPU memory consumption due to graph storage is only XX GB, while running a 2-layer GCN consumes a total of YY GB memory. Thus an additional ZZ GB memory consumed as part of training seems very high based on our estimate (and later confirmed in \cref{sec.exp}). \td.

% This result indicates that DGL introduces a huge framework-related memory overhead, thus DGL is unsuitable for the GNN benchmarking framework. 
% It is also important to establish a baseline memory consumption to truly advance the research in memory-saving techniques, an important research direction considering deep learning is known to consume huge amounts of memory.


% \noindent 
% $\bullet$ \textbf{Unclear Integration Process.}
% While DGL has very good documentation on using the platform and developing new GNN models, it has no documentation on system integration. 
% Hence prior works have followed different approaches. 
% %and we could run two popular works of GE-spMM~\cite{gespmmsc2020} and FeatGraph~\cite{featgraphsc20} end-to-end.
% GE-SpMM~\cite{gespmmsc2020} provides the source code files to replace the same-named DGL source files. However, those named files are now missing in DGL due to its complete code re-organization, a trait of a monolithic system. %Further, the DGL code-base has included one such file\footnote{\scriptsize \url{https://github.com/dmlc/dgl/blob/master/src/array/cuda/ge_spmm.cuh}} but did not integrate it. Our evaluation revealed functionality bugs with this code. Hence we did not proceed with it.
% We also could not run FeatGraph~\cite{featgraphsc20} end-to-end despite trying many GitHub branches as suggested by their authors (see appendix for our communication), though it is officially integrated by DGL using a compile-time flag. So, questions remain on the modality of integration.

% %though they claimed that the proposed techniques have been integrated into DGL's own kernels.
% %while we have not encountered any prior work that has written a custom interface in DGL. 
% %\noindent \textbf{Massive Effort are Needed for Integration.}

% %Further, DGL offers one generic system API each for gSpMM and gSDDMM interface to the DL framework. So any attempt at kernel fusion needs a \textit{custom system API}, and almost full re-write of the DGL backend including the new fused kernels. 

% \noindent
% $\bullet$ \textbf{No Support for Custom Graph Storage.}
% The current trend in Graph Neural Network (GNN) optimization involves enhancing performance through graph decomposition techniques such as tiling and blocking(\td cite). For example, a common approach is to propose different techniques to build customized graph storage formats to achieve workload balancing.
% To facilitate the integration of these optimization techniques, there is a need for an easily abstracted graph storage format object. However, DGL currently lacks support for such customizable graph storage formats.

% %However, both of them relied on the same storage format as DGL. But 
% Supporting a custom graph storage needs to change almost the whole backend including many public system APIs of DGL, such as \textit{successors()} and \textit{predecessors()}, which are not even used by GNN systems. 
% %the way we understood advanced features of PyTorch to pass graphs as a custom object using the smart pointer approach\footref{foot.time}.  
% %Then, they can prototype a custom kernel and can support custom graph storage.
% Hence, spending additional effort may be of no use if the whole backend and system APIs need to be replaced. History indicates that such types of optimization works~\cite{huang2021understanding,wang2021gnnadvisor,fu2022tlpgnn,spektral} have rather relied on plugin environment, developed their own model code, system APIs, and system code despite the interface-level limitation.
% We reached out to some authors of GNN papers to understand why they did not use DGL. 
% One of the authors of a prior GNN system aptly described the limitations of working with DGL: \textit{``We didn't use DGL, because some of its design is inefficient but is also embedded in the system design in a complex way''} %\footnote{Personal communication using email}, 
% confirming our observation on using DGL. 

% %An advanced system researcher may be able to understand and modify the internals and APIs completely despite the absence of integration-related and backend documentation. However, DGL integrated systems~\cite{gespmmsc2020,featgraphsc20} have not even fused obvious kernels of gSpMMv and normalization by degree. 



% %It should be noted that DGL suffers from large framework overhead and huge memory consumption, hence using it is not good for benchmarking as any system can develop its own benchmark and can easily outperform the DGL-based benchmarking suite for run-time and memory consumption.

% %for GNN system optimizations. 
% %This response points towards the complex monolithic design that does not encourage innovations in custom storage format or kernel fusion. 

% % allows prototyping of the system idea easily.
% %We now study if DGL can be used productively to support system integration of GNN optimizations, and presents the following challenges.
% %It has neither advertised that is a tool for \textit{systems} research and education nor has any documentation to aid in integrating systems work to it. Clearly, integration with DGL requires additional effort in understanding its back-end system design and code base. 
% %Additionally, DGL suffers from two critical limitations if it is used for performing system research.
% %In absence of documentation on integrating different systems to DGL, researchers have taken an approach based on its code-study, and success do have been reported~\cite{gespmmsc2020,featgraphsc20} \td[more citation]. However, 
% %DGL is a monolithic system,   
% % The official DGL integrated code of FeatGraph~\cite{featgraphsc20} (hosted by DGL) has not implemented graph partitioning as described in the original paper.
% % %is not exactly a framework designed with systems research and education in mind.
% % %DGL internally prepares CSR/CSC format with an edge ID as its fixed edge property irrespective of whether needed or not, and 
% % DGL is a monolithic system that supports a variety of APIs on graph objects, such as \textit{successors()} and \textit{predecessors()}, whose implementation will involve  additional effort if a custom graph storage is implemented which is not useful when the aim is just kernel optimization through a better storage format.
% % %Hence DGL integrated systems either use or force to use vanilla CSR/CSC format for integration purposes unless all the APIs are correctly implemented.
% % Not implementing these APIs will leave the whole DGL code in a broken state due to its monolithic nature.
% %implying that the monolithic nature may reject merging other past and future research if it involves storage format change.
% % Similarly, GE-SpMM~\cite{gespmmsc2020} is CSR/CSC based GNN system to be integrated into DGL.


% DLPack tensor is very simple structure, and does not require huge effort for its Python binding.

%The core ‘scatter-gather’ function implemented based on c++ arrays, which is incompatible with the tensor operations used in graph DL. To solve this challenge, {\graphpy} use the DLPack tensor to fix this gap between tensor operations and the array-based c++ computation.
%As we mentioned above, {\graphpy} uses the c++ array to implement the message-passing schema. However, Python-based tensor operations are widely used in the graph DL area. There is a need for users to figure out how to integrate the Python tensor operation with the C++ array-based computation kernel. 




%{\color{red}
%For graph handling, {\graphpy} allows multiple methods to handle the graph exchange.(\cref{sec.multi}) As we mentioned before, {\graphpy} makes the{\graphpy-GNN} module truly independent, which avoids any limitation of any no-tensor data exchange between how Kernel and Workflow. Therefore, {\graphpy} can use any python binding or any object to handle the graph exchange between Kernel and Workflow. 
%}


%Developing a third-party tensor library inside the Kernel module requires huge learning curve as well as introduces an additional burden in terms on memory management for which no guidelines exist. 
% While the tensor inside Kernel needs to be allocated when producing the kernel output, the tensor deallocation path is complex.
% Recall the need of state tensors during back-propagation, and can be freed only after that in each epoch. 
% This requires understanding of the protocol of computation graph including when the DGL tensor can be safely deallocated, and how. 
% Unfortunately, how this deallocation process works, how to implement the compatibility among tensors are not documented by the owners of intermediate compatible tensor~\cite{dlpack}, leave alone how one would implement their own tensor library-- even a bigger problem.
% %Therefore, the goal of integrating the {Kernel} module is still complex. 



%Our limited survey of other works that modified DGL to demonstrate better performance, also relied on CSR/CSC format. We suspect that such researchers may have found that modifying whole DGL Kernel a tedious process when format changes are involved. \td.

%Hence, the lightweight Kernel module in the plug-and-play eco-system of {\graphpy} provides enough space for innovations without the need to spend efforts on graph preparation or in supporting the APIs that are not applicable for deep learning purpose.

%Writing interfaces for a new kernel in DGL is still a complex problem due to involvement of tensor library and memory management. Therefore, in our opinion, DGL is a system, and not necessarily a productive framework suited for systems research and education.


%Avoid introducing overhead is an necessary requirement for a system so that the later optimization techniques will not try to minimize that overhead, and rather should focus exclusively on actual system optimization tasks. In other words, when compared against small overhead systems, it is not likely to get misleading benefits. However, 
%In the traditional graph data science domain, Mcsherry et al~\cite{mcsherry2015scalability} point out the introduction of large system overhead, which is then also optimized as part of analytics performance optimization.  Hence, actual performance improvement solely due to better algorithmic implementation remains less. Our experiment measurements (\cref{sec.exp}) show that DGL introduces huge system overheads in the form of a one-time start up cost, and run-time overhead, which is also identified by DGL. Hence, any system that does not use DGL to implement GNNs 




  


% \noindent \textbf{Integration with DL Framework}
%Further, the DL model layer development follows the usual step of the DL framework to implement the layer in Python. Thus, {\graphpy} uses this framework's computation graph automatically.
%It should also be noted that the kernels that are invoked in the backward computation are related to the kernels called in the forward computation. E.g., if an unweighted SpMM kernel is invoked in the forward direction, the backward computation also invokes this unweighted SpMM kernel but on the inverse graph. 
% So, it is the job of  {\graphpy-Workflow} to implement this workflow and call the right set of kernels in forward and backward with the right set of input and output tensors. 
%Each {\graphpy-GNN} also offers $flag$ as part of their APIs (e.g. Table~\ref{table-kernel}) through which {\graphpy-Workflow} can specify if the computation should be done in forward or inverse of the graph. The corresponding implementations are handled in {\graphpy-GNN}. 

% It should be noted that we are able to fully share the Kernel code, while at this moment Workflow code must be rewritten for every DL framework excluding the adapter. Hence, {\graphpy-GNN} becomes fully plug-and-play, and can easily be replaced by a better-optimized Kernel by others.
%We are looking at possible extension of DSL to automatically generate complete Workflow code as well.







% \subsubsection{\graphpy-GNN} \label{sec.kernel}

% % Our aim for this component is to provide the boilerplate code so that it is easy to implement any kernel now or in future with any novel system ideas without spending time on how to write those boilerplate code. 
% Table \ref{table-kernel} shows how {$wrap\_graph$()} API accepts the Numpy arrays for the graph exported from {\graphpy-SM}. It wraps them up in a $g$ structure.
% Hence, all kernel APIs then accept this $g$ object, apart from DLPack tensors for input and output tensors, and other inputs.
% This module contains the boilerplate code for Python binding of the APIs (Listing \ref{list-pybind}), that converts the input and output DLPack tensor to native arrays by extracting the pointer, and finally calls the actual C++ kernel implementation in the back-end.
% Thus remaining job then is to simply implement those kernels without worrying about tensor. 
% For the GPUs, there are a few more steps, that we discuss next in  \cref{sec.extend}, that still follow the similar philosophy.
% % Hence, all kernel APIs then accept this $g$ object, DLPack tensors for input and output tensors, and other inputs, and uses the boilerplate code to call the actual C++/CUDA kernel implementation in the back-end. 
% Also, the boiler-plate code is automatically generated when a system researcher specifies a new kernel that is not supported out-of-the-box from {\graphpy}. 


% The {\graphpy-GNN} provides all the GAS APIs for GNN use-cases using three set of APIs as listed in Table~\ref{table-kernel}. We also provide a choice of reduce function using $eFn$ enumeration type, which may contains values SUM, MIN, MAX, DIV etc. Further, we also provide kernels for sparse layers, which implements traditional sparse linear algebra as we discuss shortly. We also provide other traditional GAS APIs and Kernels such as BFS. 




% The only duplicated effort is on writing the Python code for model, i.e. the data scientists' job. We do not think that data scientists will need to write model code for many frameworks, as they  will write their model code using  their preferred framework.

%There are other ways to build {\graphpy-SM} but they have not been tried yet. E.g., 
% \noindent
% {A database table} 
% %supports edge properties through table columns and can make data exchange free of compilation. However, they are 
% is  an examples of captive solutions where we need to send the computations (e.g., queries) to the database module. If we need to get the whole graph in CSR/CSC format,
% %Similarly, one can use binary JSON structure as a way to store the properties, and thus enable data transfer easily, however, we need to convert it back to CSR/CSC first. 
% the \textit{dtype} like mechanism is still needed. Hence, just a python package of existing databases is not enough to get the graph storage to {\graphpy-GNN}. %without the support of \textit{dtype} like mechanism.


% \noindent \textbf{Static Graph Analytics System.}
% Traditional graph analytics systems focus on creating graph representation and performing traditional graph analysis. Some works \cite{roy2013x} \cite{liu2017graphene,powerlyra2015eurosys,gstore, nguyen2013lightweight,
% zheng2015flashgraph,mosiacEuroSys17, roy2015chaos, han2013turbograph, kumar2017falcon, zhu2015gridgraph,hong2012green, wu2015g, ai2017squeezing, zhu2016gemini,liu2015enterprise} 
% can only support the graph topology analysis on the static graph. These works pre-process the raw input data to create the graph representation and then perform the graph topology analysis. None of them, are able to support arbitrary edge properties. They allow at max one additional field for edge weights.

% \vspace{1mm}
% \noindent \textbf{Dynamic Graph Analytics System.}
% Grace~\cite{grace12atc}, LLAMA~\cite{macko2015llama}, Stinger~\cite{ediger2012stinger}, Graphone~\cite{kumar2017graphone,kumar2020graphone}, Aspen~\cite{dhulipala2019low} can support dynamic graph but it is implemented mainly in C++ and did not provide any wrapped python APIs. Further, except GraphOne, others does not provide arbitrary edge properties. Moreover, GraphOne uses template meta-programming to support arbitrary edge properties, however it is almost impossible to enable python binding for arbitrary edge properties. {\graphpy-DE} fixed this gap between C++ and Python, and also took advantage of the fact that it has to support only static graphs. Hence, provides many new optimization that does not require the data consistency support.

% \vspace{1mm}
% \noindent \textbf{Python based Graph Analytics System}. NetworkX~\cite{networkx08} is a popular python based graph system. However, it is very slow due to its purely python based implementation. We believe that {\graphpy-DE} can become a back-end to take advantage of the huge analysis code-base of NetworkX.

% \noindent \textbf{Graph Neural Network (GNN)} system, such as DGL~\cite{dgl2019}, NeuGraph~\cite{neugraph19atc}, Pytorch-Geometric~\cite{pytorchg2019} perform deep learning on graph data. DGL \cite{dgl2019} is an open-source,  DGL is a monolithic GNN framework, and, and supports only a limited set of graph preparation, and does not export the graph representation to third party module, so it is hard to quickly prototype any new system idea. It also does not support bipartite graphs, hence it cannot support sparse models.
% % purely c++ implemented graph deep learning system. 
% NeuGraph is a not open-sourced, and does not support attention based models such GAT. Pytorch-Geometric is tightly integrated with Pytorch~\cite{pytorch2019}. Hence, integrating new system design involves huge efforts.

% Although these works support graph deep learning features, data scientists need to pre-process the raw input data themselves. It is not clear how will they convert the raw string identifier to a numeric vertex ID in such cases. Possibly, they force the data-scientist to do more ad hoc processing.  
% % to create the graph representation themselves. 

% % On the other hand, {\graphpy} is a full-fledged systems for complete data-science need on graph like data, including graph preparation from raw-data in parallel and high-performance way, traditional graph analysis, and graph deep learning. Moreover, it export the internal graph data as numpy arrays, on which any ad hoc graph analysis including graph deep learning can be performed.  
